Towards Scalable Dataframe Systems

Dataframes are a popular abstraction to represent, prepare, and analyze data. Despite the remarkable success of dataframe libraries in Rand Python, dataframes face performance issues even on moderately large datasets. Moreover, there is significant ambiguity regarding dataframe semantics. In this paper we lay out a vision and roadmap for scalable dataframe systems. To demonstrate the potential in this area, we report on our experience building MODIN, a scaled-up implementation of the most widely-used and complex dataframe API today, Python's pandas. With pandas as a reference, we propose a simple data model and algebra for dataframes to ground discussion in the field. Given this foundation, we lay out an agenda of open research opportunities where the distinct features of dataframes will require extending the state of the art in many dimensions of data management. We discuss the implications of signature data-frame features including flexible schemas, ordering, row/column equivalence, and data/metadata fluidity, as well as the piecemeal, trial-and-error-based approach to interacting with dataframes.

==> algebra_challenges.tex <==
% \subsection{New Algebra Challenges}\label{sec:algebra-challenges}
% \rebuttal{
% Existing APIs for dataframe implementations like pandas have ballooned
% to hundreds, making them difficult to maintain and even more difficult
% to optimize. It would not be feasible to declare a comprehensive set of
% rewrite rules on all combinations of the 240 APIs pandas supports. It is,
% however, much more feasible to define rewrite rules on the algebra
% we presented in Section~\ref{sec:df-algebra}. Armed with this algebra,
% we can start to rethink the existing 
% query languages to maintain some expressiveness without duplication.
% This new algebra will present a host of new challenges that prevent
% us from using some best-practices in query processing and
% optimization from relational literature.
% In this section we discuss in detail 
% the new challenges in supporting the dataframe
% algebra and potential opportunities.}

% \rebuttal{
% \stitle{Transpose.}
% }

% \todo{
% Interesting rewrite rules
% \squishlist
% \item select transpose = project
% \item pivot transpose = other pivot
% \squishend
% }

% \todo{
% Metadata manipulation vs. physical manipulation when it makes sense e.g. matrix multiplication
% }

% % \rebuttal{
% % \stitle{Schematic asymmetry.}
% % }

% % \rebuttal{
% % This schematic asymmetry presents some new challenges that
% % are specific to the dataframe with how
% % queries are optimized.
% % }

% \rebuttal{
% \stitle{Map}
% }
% \moved{
% Extended relational algebra supports map via the use of functions
% in the subscript of projection operators (i.e., in the \code{SELECT}
% clause of SQL). However, this
% % For example, in a relational system,
% % the equivalent of a \code{fillna} operation would
% % likely require code refactoring after a schema change introduces an
% % additional column (wherein the new column is explicitly named in the
% % \code{fillna} equivalent), but no such refactoring is necessary if
% % an additional column is added to a dataframe.
% projection
% syntax is linear in the arity of the relation, which is cumbersome 
% for very wide schemas (e.g., after a \code{TRANSPOSE}).
% In this definition, \code{MAP} is passed an entire
% row as an argument so it can reason across columns
% in a generic fashion without enumerating them, whereas 
% SQL expressions (including UDFs) typically require specific fields
% from the row as scalar arguments. For example, 
% consider a transformation that needs to ensure the values in 
% all \textbf{float}-domain columns 
% in a given row sum to 1.0; a generic, reusable \code{MAP} function can 
% normalize the value in each \textbf{float} 
% field by the sum of the \textbf{float} 
% fields in that row;
% instead, a SQL expression
% would have to be crafted specially for each schema. 
% }

% \rebuttal{
% % \stitle{Query optimization.}
% Since \code{MAP} is applied to each row individually, the
% user defined function may need access to any number of columns.
% In the naive case, this places a difficult constraint on the query plan, where
% all columns of a given must be fully materialized before the function
% can be applied, which limits the amount of query planning possible.
% This is true even in cases where the \code{MAP} function only
% requires access to one column.
% Another query optimization challenge with \code{MAP} is that the
% user's function may change the schema. This makes it difficult to
% apply global optimizations, and it can render any existing columnar
% data layout optimizations useless.
% }

% \todo{constraint maps: explosion of APIs}



% \rebuttal{
% \stitle{TOLABELS and FROMLABLES}
% }


==> challenges.tex <==
\section{Optimizing for Execution}\label{sec:datamodel}

\techreport{In this section we discuss several directions of future work to support optimized execution of dataframes. 
We divide these optimizations along several directions including physical data layout, query planning, improved support for interactive data exploration, and multi-query optimization.}

Dataframes combine functionality from relational and linear algebra, so there are opportunities to leverage, combine, and extend advances in physical data layout pioneered in both the database and scientific computing communities.  
Over the last two decades, the database community has explored many directions for table
storage, including both row- and column-oriented storage as well as various hybrids at
both the disk and in-memory level (as surveyed by Abadi, et al. \cite{abadi2013design}).
Principally, from this work the fundamental concepts of data independence, has the opportunity to play a major role in future dataframe systems.  
Today's dataframe systems already share common physical storage of data across multiple derived dataframes to reduce the memory requirements.
However, future dataframe technologies might also explore view based representations where computation is used in place of storage. For example, the Vaex project \cite{vaex}, which is a dataframe-like system
that allows querying on HDF5 files, implements virtual columns. With virtual columns,
the column is not actually materialized until required for output, printing, or for a query. 
In cases where the computation that creates a column is expensive, virtual columns will
need to be paired with intelligent caching mechanisms that prioritize caching
columns that were expensive to generate. 

Traditional work on dataframes has largely focused on modest-size datasets that fit in RAM
on a single machine. Scaleup in this domain can be achieved in two standard ways: exploting
the aggregate RAM across many machines using data partitionining (``sharding''), and/or
exploiting a memory hierarchy, e.g. by spilling data to secondary storage in bulk algorithms,
or using a paginated buffer cache for random accesses. These techniques are natural aspects
of the design space for a scalable dataframe library, though once again the diversity of
potential access patterns may complicate the story beyond the prior work in databases,
scientific computing and dataframes. This design space is further complicated by technology
trends including the desire to shuttle data to/from GPU memory for matrix operations,
multi-level storage hierarchies both in new hardware and in cloud storage services, and
the ability to autoscale cloud resources including RAM for bursts of memory- and
compute-intensive work.
Given that the dataframe model is a hybrid of both the relational and
matrix-oriented representations,
there must be many considerations about how to store and retrieve a dataframe using both
memory and secondary storage. Like a matrix, a dataframe might be scanned in either
row- or column-major order, and must support retrieval along either axis (or both) by
index, or positional notation. 
Vectorization of
execution is important for certain dataframe operations and depends heavily on the physical data layout.
% Both in the columnwise relational style \cite{abadi2013design} and in terms of linear algebra on matrices, especially using GPUs [cite what?]. 
Compression can be important for minimizing memory footprint and
improving I/O bandwidth as in columnar databases, but may be a bad fit to certain access
patterns.

\stitle{Apache Arrow.}
Apache Arrow\cite{pyarrow} is an in-memory column store targeted at setting a cross-language
standard for flat and hierarchical tabular data. \modin uses Apache Arrow for serialization
of dataframe partitions when they being communicated or shuffled between processes. Apache
Arrow has an in-memory tabular format called Arrow Tables and several high-performance
compute kernels that can be used to operate on Arrow Tables. Arrow is not designed to be
a user-facing dataframe library, but does aim to be the in-memory storage format
for tabular data computation. Arrow Tables do not directly conform to the dataframe data model
presented in Section~\ref{sec:dataframedef} primarily because there is no vector of row labels
$R_m$ in an Arrow Table. Arrow Tables also do not yet support \code{TRANSPOSE}, and it is not
clear what the new column labels of a \code{TRANSPOSE} would be without explicit row labels.

Aside from optimizing the physical plan and data layout,
dataframes will need new query rewriting rules due to the new algebra.
Existing dataframe systems execute queries in a strictly imperative way
and do not perform any query rewriting~\cite{mckinney2010data, R, dask}.
Some systems that market themselves as dataframes (e.g. Spark, Dask) are declarative but do not support operations
beyond the traditional relational table operations~\cite{Armbrust:2015:SSR:2723372.2742797, dask}.
The \code{TRANSPOSE} operation presents some particularly interesting opportunities and challenges, and in some cases can be avoided using clever rewrite rules.
For example, the query \code{TRANSPOSE}, \code{SORT}, \code{TRANSPOSE} to reorder columns can be 
rewritten as a \code{MAP} and \code{RENAME}. 
The challenge of supporting declarative query processing across a wide range of dataframe operators is that
the cost of extending rewrite rules beyond relational operations, 
to support spreadsheet and linear algebra operations, requires a significant development effort.
As a result, dataframe users either have to sacrifice performance, 
operate on a feasible subset of their data, 
or manually construct and profile various possible rewrite to determine the optimal approach to execute the query~\cite{optimizing-pandas}. 
When creating rewrite rules for dataframes, we have to consider (i) how to group the dataframe operations into queries and (ii) when to rewrite the queries.
Manual query optimization on the part of the developer can be a daunting task due to the large number of possible ways to perform an operation~\cite{wu2019diel}.
In addition to the numerous ways of writing any given query at the API level,
the problem is further exacerbated by the fact that
there is a large and diverse set of operations beyond relational operators to consider when creating rewrite rules. \eat{An important area of future
work in \modin will be in defining rewrite rules to efficiently
handle cases that traditional systems cannot.}

There is a very wide physical design space for dataframes, 
which spans ideas from the literature in databases, scientific computing and recent machine learning systems. It will be important to validate
the research with real-world workloads and new benchmarks that
evaluates how dataframes are used and interacted with in practice.

\techreport{
\subsection{Data Layout and Indexing}\label{sec:datalayout}

\smacke{Professor suggestions: highlight that there are many
existing layout strategies and corresponding optimizations and
the interesting part is hybridizing these for dataframes.}

\jeg{The following was a quick brainstorming session of "ideas" for research directions we want to cover in physical data layout.}

\begin{itemize}
    \item Block oriented storage and the connection between advances in column stores and compressed sparse block representations (eg https://people.eecs.berkeley.edu/~aydin/csb2009.pdf)
    \item referential or view based storage: store data as a reference to other dataframes or store data as a function of other data rather than by value.
    \item Advances in indexing: 
    \begin{itemize}
        \item extending to columns and rows
        \item Automatic index generation for intermediate queries (must have already been done?)
    \end{itemize}
    \item Better support for vectorized operations (hardware accelerator aware data layout)
    \item Automatic repartitioning to improve operator performance (must have already been done?)
    \item Discussion on NULL value
    
\end{itemize}


Because dataframes combine functionality from relational and linear algebra there are opportunities to leverage, combine, and extend advances in physical data layout pioneered in both the database and scientific computing communities.  
In the following, we provide a high-level overview of a few of the key advances from each community and how they can be incorporated and extended to support efficient computation on dataframes.




% Given the unique aspects of the dataframe data model and algebra, 
% there are a number of natural open questions regarding both storage and processing
% of dataframes, as opposed to traditional relational tables or scientific matrices.

% \subsection{Ordered Data Model}
% The ordered data model of the dataframe presents challenges
% to the existing optimizations used in relational databases.
% It is possible to add dataframe-style order semantics
% to a relational table by maintaining
% the order rank of each row in a special immutable column, represented
% in Figure~\ref{fig:datamodel} as part of the row metadata. After
% every query, the system can perform an \code{ORDER BY} on
% the order rank column to preserve the user's order through
% operations. This would also preserve the relational model's
% unordered data model in that the \code{ORDER BY} operation
% would reorder the data after every query so that the
% system is free to have an arbitrary physical order.
% This presents new optimization problems that can leverage
% prior work in the database community. Order in the dataframe
% data model serves two purposes: 
% consistent presentation of user's view of the data
% and \code{WINDOW} operations.

% Dataframe users often build their query incrementally through trial-and-error. 
% As illustrated in Section~\ref{sec:usecase},
% the trial and error style involves printing some subset
% of the rows and columns through the 
% \code{head}, \code{tail}, or \code{print} operation.
% The \code{head} and \code{tail} commands print the first
% or last \code{n} rows (5 by default), respectively and
% printing a dataframe
% shows both the first and last 5 rows. 
% When a user prints
% the first \code{n} rows, they expect to see the first
% \code{n} rows from the actual data that was ingested,
% and they expect that the system will print the same
% \code{n} rows each time. The latency of displaying these first and last
% \code{n} rows is important as users rely on these operations to verify the
% correctness of their data and query and subsequently make decisions about what to do next.

% While it is possible to use strategies similar to those that
% optimize for the \code{LIMIT} clause in RDBMSs \cite{kim2018optimally}, additional
% consideration must be made for the \code{ORDER BY} clause to ensure that
% the order is the same every time
% time the user prints the dataframe, as in \cite{SOMETHING}. 
% To avoid computing the \code{ORDER BY}
% on every computation, the first and
% last \code{n} rows can be logically removed as separate tables, 
% and perform computation on those
% tables to print the results faster. The remaining data can 
% computed separately following the lazy evaluation paradigm,
% enabling query planning on the remaining data. In the case
% that the query modifies the order of the data, the
% printed rows will have to wait until the \code{ORDER BY} to 
% ensure that the user sees the data in the order they have
% specified. In these cases, there is a limit to the amount of
% query planning that can be applied because the print forces
% the \code{ORDER BY}. We will further discuss the challenges
% in mutliquery optimization in Section~\ref{sec:challenge-inter}.


% \subsection{Data Layouts}

% \begin{figure}
% %\includegraphics[width=0.4\textwidth]{clean_slate_block.png}
% \includegraphics[width=0.475\textwidth]{modin-composability.png}
% \caption{Factoring out views from the dataframe physical layout.}
% \label{fig:composability}
% \end{figure}


\subsubsection{Databases}
Over the last two decades, the database community has explored many directions for table
storage, including both row- and column-oriented storage as well as various hybrids at
both the disk and in-memory level (as surveyed by Abadi, et al. \cite{abadi2013design}).
Principally, from this work the fundamental concepts of data independence, has the opportunity to play a major role in future dataframe systems.  
Today's dataframe systems already share common physical storage of data across multiple derived dataframes to reduce the memory requirements.
However, future dataframe technologies might also explore view based representations where computation is used in place of storage. For example, the Vaex project \cite{vaex}, which is a dataframe-like system
that allows querying on HDF5 files, implements virtual columns. With virtual columns,
the column is not actually materialized until required for output, printing, or for a query. 
In cases where the computation that creates a column is expensive, virtual columns will
need to be paired with intelligent caching mechanisms that prioritize caching
columns that were expensive to generate. 


\jeg{paragraph on indexing techniques.}
To improve efficient data access the database community has developed sophisticated indexing strategies.  
\jeg{Additional transition ... we believe these techniques will play a role in advancing performance of dataframes ...}
Like a relation, the rows of a dataframe may also be
retrieved by name, or named notation, and hence require
value-based indexing. The columns of a dataframe may also be retrieved by name, and given
the potential for massive arity on the order of billions, this also requires value-based indexing.


\jeg{paragraph on array based}
In addition, there has been work on supporting array-based data in databases, for both
``multidimensional'' OLAP workloads in the traditional relational model, e.g.
\cite{deshpande1997cubing, otoo2007optimal}, and for database-backed scientific computing
(e.g. last surveyed by \cite{rusu2013survey}).

\subsubsection{Scientific Computing}

Much of the focus on large scale scientific computing has been on efficient storage and execution of basic linear algebra subroutines.  
There is extensive work in the
scientific community on matrix representations for parallel computation (e.g.
\cite{choi1992scalapack}). \jeg{merge first two sentences.}


\subsection{Partitioning and Memory Hierarchies}
\smacke{JMH: maybe all this can be talked about in the data layout section,
dividing that into single vs multi node}
\smacke{AGP: prepartitioning to optimize for stream of subsequent operations is sensible}
\smacke{AGP and Anthony: Maybe merge with Section~\ref{sec:datalayout}}

Traditional work on dataframes has largely focused on modest-size datasets that fit in RAM
on a single machine. Scaleup in this domain can be achieved in two standard ways: exploting
the aggregate RAM across many machines using data partitionining (``sharding''), and/or
exploiting a memory hierarchy, e.g. by spilling data to secondary storage in bulk algorithms,
or using a paginated buffer cache for random accesses. These techniques are natural aspects
of the design space for a scalable dataframe library, though once again the diversity of
potential access patterns may complicate the story beyond the prior work in databases,
scientific computing and dataframes. This design space is further complicated by technology
trends including the desire to shuttle data to/from GPU memory for matrix operations,
multi-level storage hierarchies both in new hardware and in cloud storage services, and
the ability to autoscale cloud resources including RAM for bursts of memory- and
compute-intensive work.


Given that the dataframe model is a hybrid of both the relational and
matrix-oriented representations,
there must be many considerations about how to store and retrieve a dataframe using both
memory and secondary storage. Like a matrix, a dataframe might be scanned in either
row- or column-major order, and must support retrieval along either axis (or both) by
index, or positional notation. 
Vectorization of
execution is important for certain dataframe operations and depends heavily on the physical data layout.
% Both in the columnwise relational style \cite{abadi2013design} and in terms of linear algebra on matrices, especially using GPUs [cite what?]. 
Compression can be important for minimizing memory footprint and
improving I/O bandwidth as in columnar databases, but may be a bad fit to certain access
patterns.



Apache Arrow\cite{pyarrow} is an in-memory column store targeted at setting a cross-language
standard for flat and hierarchical tabular data. \modin uses Apache Arrow for serialization
of dataframe partitions when they being communicated or shuffled between processes. Apache
Arrow has an in-memory tabular format called Arrow Tables and several high-performance
compute kernels that can be used to operate on Arrow Tables. Arrow is not designed to be
a user-facing dataframe library, but does aim to be the in-memory storage format
for tabular data computation. Arrow Tables do not directly conform to the dataframe data model
presented in Section~\ref{sec:dataframedef} primarily because there is no vector of row labels
$R_m$ in an Arrow Table. Arrow Tables also do not yet support \code{TRANSPOSE}, and it is not
clear what the new column labels of a \code{TRANSPOSE} would be without explicit row labels.


\jeg{I don't know what this is saying:}
There is a very wide physical design space for dataframes, which spans ideas
from the literature in databases, scientific computing and recent machine learning
systems. Real-world workloads and benchmarks will be important issues in this space.


\subsection{Statement Optimization}
\devin{Fill in with reference to prior sections and introduction}
\devin{Rewrite rules}
% \devin{Map is too powerful - Lara}
\smacke{JMH: grab bag of potential optimizations}

% \stitle{User Views.} These views are the views that a user would
% see. These could be the result of a query, or they could be identical
% to the baseline Ordered View. Each of these views is free to have its
% own order, but it shares a baseline order, logical schema, and
% physical model with all other user views.

% \stitle{Ordered View.} The ordered view is a view on the data
% that presents the data in the order requested. This is the initial
% order of the data, as it was ingested, and must be maintained as a
% baseline for the other views.

% \stitle{Logical Schema.} The logical schema contains metadata
% about the table. Because of the equivalence of rows and columns
% in the dataframe system, additional metadata will need to be
% maintained above that of a typical relational DBMS.

% \stitle{Physical Model.} The physical model is similar to a
% typical relational DBMS physical model, outside of requiring
% additional optimizations for the dataframe algebra primitives
% not expressed in relational algebra.

% \subsection{Memory and Storage}
% Despite the fact that large memory machines are becoming more
% accessible, it is not reasonable to expect all dataframe workflows to
% fit in memory. Many dataframe systems are strictly in-memory,
% following the matrix model. This
% limitation has been addressed in some systems\cite{sparksql-func, dask} by
% enabling memory ``spillover'' to disk, but
% these systems sacrifice semantics in the interest of optimization. we
% discuss the deviations of these systems in detail in Section~\ref{sec:ext}.
% In order to preserve the semantics
% of dataframes, new systems will need to have an optimized storage layer. No
% existing dataframe system allows users to directly query data stored
% on disk, instead requiring users to load the data from a file
% and materialize the data in memory. \modin will bring relational
% database-like direct storage querying to dataframes by enabling
% memory spillover and buffer-pooling.

% Memory spillover is the first step in enabling direct storage querying.
% \modin has preliminary support for spillover, or ``out of core'', which
% allows a session to exceed the memory of the machine it is on and spill
% to disk. In this model, memory is still the primary storage for the
% workflow, but can page data to disk. Data is still read from disk into memory in
% its before querying can begin, so there is less of an opportunity to pushdown
% predicates to the storage layer. Additionally, many of the file formats
% that are commonly used in dataframe workflows do not follow a
% query-friendly standard. Parquet~\cite{parquet} offers the capability
% to do predicate pushdown, and is supported by pandas, but is far less
% commonly used than CSV or text files. This may be because pandas does not
% do predicate pushdown and text-based file formats allow users to directly
% inspect them from the command line or a text editor. Memory spillover
% will not be sufficient if \modin is to enable relational database-style 
% querying to dataframes. Buffer-pooling will enable \modin to deliver
% fast performance on data staged on-disk without requiring the data
% to be loaded into memory.

% \agp{This section is quite weak. From the storage standpoint, you need to talk about row vs. col storage and its interaction with transpose. Compression may be beneficial. Block storage may also be beneficial to allow for quick inspection, especially for wide and deep tables. Say that the order that things are stored may not be the one that is actual order. Can postpone ordering if user doesn't inspect most expensive operations: easier to treat labels as data for the purpose of optimization...}
}

==> challenges_agp_5-25-bkp.tex <==
%!TEX root = modin-vision.tex

\section{data model challenges}\label{sec:datamodel}
% \dorx{New outline: \url{https://docs.google.com/document/d/13-pmh461S3Mj0WoVZ8l1zbN18nF7DI_luRzDRuUqe7U/edit?usp=sharing}}

\rebuttal{
Supporting 
the dataframe data model and algebra from
Section~\ref{sec:definitions} efficiently
motivates a new set of 
research challenges.
We organize
these challenges based on 
unique properties of dataframes,
and discuss their impact
on query optimization, data layout,
and metadata management. 
We first discuss the impact of flexible schemas.
%\devin{Expand for flow?}
% We draw on the distinctions between the
% dataframe and relational data models throughout.
% Here we outline the challenges in supporting the data model of the dataframe,
% as defined in Section~\ref{sec:dataframedef}. 
% These challenges
% are informed by our experience thus far
% with the implementation of a scalable dataframe system,
% \modin.
}

\subsection{Flexible Schemas, Dynamic Typing}
\input{flexible-schema-new.tex}
%\input{flexible-schema-old.tex}

\subsection{Order and Equivalence}\label{sec:order_challenges}
\rebuttal{
Unlike relations, dataframes are ordered
along both rows and columns---and users
rely on this ordering for debugging and validation
as they compose dataframe queries incrementally.
This order is maintained as rows are transformed
into columns and columns into rows via \code{TRANSPOSE},
ensuring near-equivalence of rows and columns.
Finally, as we saw in Section~\ref{sec:algebra-example}, 
row and column label metadata is
tightly coupled with the dataframe content,
and inherits the order and typing
properties. 
Unlike in
relational databases, 
where metadata is largely distinct from the data,
data and
metadata are interchangeable within dataframes. 
Data can be promoted into metadata via \code{TOLABELS},
likewise metadata can be demoted
into the data via \code{FROMLABELS}. 
In this section, we discuss
the challenges imposed by enforcing
order and the frequently changing 
schema across row and column labels and row/column orientation.
}

% \todo{
% \squishlist
% \item All about layout
% \item Users expect to see data organized in specific way (hence order)
% \item Frequently change the layout (both by changing ordering, as well as transpose) and move data to metadata \& back
% \squishend
% }

\rebuttal{
\subsubsection{Order is Central}
The order of a dataframe is determined by the
order of ingested data. 
For example, a CSV file ingested as a 
dataframe would have the same 
row and column order as the file. 
This ordering is crucial for the trial-and-error-based
interaction between a user and a dataframe system.
User expect to see the same rows 
in the dataframe in the same order
as they process it---allowing
them to validate and debug each step
by comparing its result to the previous step.
For example, to ensure that
a CSV file is ingested and parsed correctly,
users will expect the first few rows
of the dataframe to be the same
as those they would see when examining the CSV
file. 
To examine a dataframe, users
will either use the operator
\code{head/tail} to see the prefix/suffix 
or simply type the name of the dataframe 
for both the prefix and suffix
in the expected order.
Additionally,
operators such as \code{WINDOW} and \code{MAP}  
from Section~\ref{sec:df-algebra}
expect a specific 
order for the rows (\code{WINDOW}) and
columns (\code{MAP}).
since the UDF 
argument to these operators may 
rely on that order. 
Dataframes also support \code{SELECTION} and \code{PROJECTION} 
based on the position of the rows and 
columns respectively. 
}

\rebuttal{
To support order, current dataframe systems,
such as \pandas,
physically store the dataframe
in the same conceptual order as defined by the user.
As a result, they do not obey physical data independence.
}\moved{%
This constraint is not necessary,
and removing it may open up new optimization
opportunities,
from recognizing that as long as
the displayed results preserve 
the desired order semantics
to the users, it is not necessary 
that all intermediate products 
or artifacts (unobserved by user)
adhere to the order constraint.
For example,
a sort operation can be ``conceptual''
in that a new order can be defined without
actually performing the expensive
sorting operation.
Likewise, a transpose
doesn't require the data to be reoriented
on physical storage unless beneficial
for subsequent operations, instead
being captured using metadata updates
to reflect the new
orientation of the dataframe.
}

\rebuttal{To ensure correct semantics,
while respecting physical data independence,
we must devise means to capture ordering
information, either tracked 
as a separate ``order column'',
if it is not implied via existing columns,
or recording as metadata that the dataframe
must be ordered based on one or more 
of the preexisting
columns. 
Then, the \code{ORDER BY}
on this ``order column'' or one of the existing columns
will be treated as an
operator in the query plan, and will only need to be
done ``on-demand'' when the user requests to view a result.
% For example,
% users will not see the
% results from the intermediate artifacts of a query
% that are not explicitly displayed, so those artifacts
% do not need to be ordered.
Additionally, since users
are only ever looking at the first and/or last few lines
of the dataframe, those are the only lines that are required
to be ordered; we discuss this further
in Section~\ref{sec:immediate-feedback}.}

\rebuttal{%
% \stitle{Physical data independence with order.}
% \todo{Consider cutting this as related work}
Extending physical data independence even further,
we can adapt other data representation
techniques from the database community,
optimized for dataframes.
This includes columnar
or row-column hybrid storage~\cite{abadi2013design},
as well as those from 
scientific computing~\cite{choi1992scalapack},
array databases~\cite{rusu2013survey}
or spreadsheets~\cite{bendre2015dataspread}.
Since dataframes are neither relations,
matrices, arrays, or spreadsheets, none
of these representations are a perfect fit. 
Given that rows and columns are equivalent,
one promising representation for
dataframes is storing it as
key-value pairs,
where the key corresponds to the
(row number, column number)
pair.
This representation
is especially effective when
the dataframe is ``sparse'', allowing
us to omit pairs where the value is null.
Then, \code{TRANSPOSE} conceptually 
swaps the row and column for each value:
$(column, row, value)$,
and can be recorded in metadata.
However, some operations become more expensive,
e.g. reconstructing a row for a \code{MAP}
operation requires a join.
% Alternatively, a system could maintain
% multiple indexes for row and column
% combinations\agp{I don't follow this multiple indexes business}, or maintain multiple
% different physical layouts, however
% the memory cost here is likely to be prohibitive. \agp{this is a bit abrupt. you're talking about one representation but now you're jumping to a hybrid.}
% A promising research direction is to consider a 
% hybrid approach, where subsets of the data may
% be stored in different layouts, optimized
% for the common access patterns of that
% particular subset. 
Overall,
automatically detecting the right representation
and updating it over the course of dataframe query
execution will be substantial challenge.}




% \devin{Propose to cut entire next paragraph}
\techreport{
\moved{%
Given a certain physical representation,
operations on dataframes,
from a relational perspective, often make use
of ordered access, e.g.,
editing the $i^{\textrm{th}}$ row,
as well as access
based on the row labels, e.g.,
filtering based on row labels (named notation) 
or row position (positional notation).
Because
selecting the $i^{\textrm{th}}$ physical row or projecting the $j^{\textrm{th}}$ physical column
will not necessarily correspond to selecting (resp.\ projecting) the desired {\em logical}
row (resp.\ column), additional metadata
that serves as the "order column" or "order row" must be maintained to facilitate
order-independence of the physical data.
Automatically
maintaining
indexes for this purpose can be beneficial.
Recent work has developed positional
indexing~\cite{bendre2018towards}, allowing ordered
access to be supported in $O(\log n)$,
in the presence of edits (e.g., adding or removing
rows).
Column stores take a different approach
to avoid expensive edits across columns,
instead
recording edits separately as deltas,
and periodically merging them back in~\cite{abadi2013design};
it would be interesting to investigate which approach is more effective for a given set of dataframe operations.
Similarly, for matrices, accesses often
happen in a row-major or column-major order,
and identifying the right indexes to efficiently
support them in conjunction
with relational-style accesses, is an important
challenge.
In particular, when a dataframe
has many rows and many columns,
we may need both row-
and column-oriented indexing.
}
}

% \todo{
% \squishlist
% \item Preserving semantics: as long as we can reconstruct the ordering, we are OK.
% \item If not implied already from a column (e.g., via an order by) we can explicitly capture ordering via a separate column
% \squishend
% }
\input{pivotplans.tex}

\rebuttal{
\subsubsection{Row/Column Equivalence}
\label{sec:rowcolumneq}
}
\rebuttal{
The presence of a \code{TRANSPOSE} operator in the
dataframe algebra
presents novel challenges in data layout and query optimization.
\code{TRANSPOSE} allows users to flexibly alter 
their data into a desired shape or schema that can be
parsed according to an appropriate schema, and 
queried using ordered relational operators.
}

\rebuttal{
To keep our data model and algebra compact, 
we have schemas only for columns, and
our operators are defined on ordered sets of rows.
By contrast, in \pandas and other dataframe implementations, 
it is possible to
perform many operations 
along either the rows or 
columns via the \code{axis}
argument.
Hence programs written in (or translated to) our algebra
are likely to have more uses of \code{TRANSPOSE} than dataframe
programs in the wild, to represent columnwise operations and/or
to reason about per-row schemas.}
% \rebuttal{
% As discussed in Section~\ref{sec:dataframedef}, our dataframe model assumes 
% a column-wise schema for a dataframe \texttt{df}. 
% If there is a desire to distinguish the types of the rows, then
% a new dataframe can be defined programmatically via \code{TRANSPOSE}, say \texttt{df\_t = df.\code{TRANSPOSE}()}. 
% By default, this requires running the type induction function $S$ on each of the columns of \texttt{df\_t}---i.e., the former rows 
% of \texttt{df}. 
% This is perhaps the most egregious example of the cost of metadata computation we discussed in Section~\ref{sec:matviews}.
% The issues raised there of materialized view caching and maintenance are critical to efficient computation of \code{TRANSPOSE}.
% }
% \moved{Instead, to minimize redundancy,
% we define operators on collections
% of rows, as in relational algebra,
% and}
\rebuttal{These operations are expressible in our simpler algebra
by first performing a 
\code{TRANSPOSE}, applying
the operation, and then a \code{TRANSPOSE}
again to return to the original orientation.
}
% \dlee{I don't think this paragraph is required, we should argue succinctly in the first paragraph that Transpose is important and leave it at that.
% - Transpose is frequent
% - Transpose is expensive}
% \rebuttal{
% \code{TRANSPOSE} allows users to conveniently leverage functions that are idiomatic
% for rows or columns, thus throwing off many data layout
% optimizations (e.g., columnar compression) specific to operators
% that are applied to rows/columns. 
% % \agp{abrupt -- how does this relate to the previous para?}
% % \agp{this is abrupt after the previous sentence.}
% For these reasons, \code{TRANSPOSE} is frequent in dataframe
% % Transpose operations that switch row and column axes are frequent in dataframe 
% workloads, since columnar operations are rewritten in terms of transposes in our 
% proposed dataframe algebra. 
% Changing the physical layout of the dataframe for 
% every transpose operation is expensive and unnecessary in most cases. One
% potential option is to perform transpose logically, by maintaining transpose axes
% information
% in the metadata and rewriting subsequent queries to leverage the metadata 
% information, instead of shuffling the layout upon every transpose operation.
% \agp{This part is ignoring what was discussed earlier wrt the key-value representation}

% \moved{
% Moreover, given the \rebuttal{frequent use of}
% \code{TRANSPOSE} in \rebuttal{typical dataframe workflows},
% we need to be prepared to handle
% dataframes that are not only extremely high in cardinality (``tall'')
% but also extremely high in dimensionality (``wide'').
% }
\rebuttal{The prevalence of \code{TRANSPOSE} in 
dataframe programs overturns many axis-specific assumptions made in traditional database storage.
Axis-specific data layouts like columnar compression are problematic in this context. 
Metadata management also requires rethinking, since dataframes are as likely to
be extremely
``wide'' (columnwise) as they are ``tall'' (rowwise).}
\rebuttal{
Both traditional and embedded RDBMSs typically limit the number of columns in a
relation (e.g., SQL Server has an upper limit of 1024
columns, or 30k columns using the wide-table feature)~\cite{raasveldt2019duckdb, sqlite2020hipp}. 
By applying \code{TRANSPOSE} on
a tall and narrow dataframe, 
the number of columns can easily exceed the millions 
in the resulting short and wide dataframe.
}


\rebuttal{
% \stitle{Query optimization.}
Dataframe systems
will need careful consideration to ensure that a \code{TRANSPOSE} call does not
break assumptions made by the data layout layer.
}
\rebuttal{
Given that the cost of performing a physical transpose will often
be high, 
one potential way to handle the data layout layer optimization
problem is to do a {\em logical} \code{TRANSPOSE} ``pull-up''. This would
delay or eliminate transpose in the physical plan as much as
possible since it will often destroy or render moot many
existing data layout optimizations. 
}

\rebuttal{
%As with most cost-based optimization, there are access patterns that admit
% exceptions to the rule. For instance, i
In some cases, we may want to consider optimizing
the \emph{physical} layout of the data given a \code{TRANSPOSE}
operator as a part of a query plan. 
This is in stark contrast with most existing data
systems which create and optimize for a static data layout.
A physical transpose may help the optimizer match the layout to the
access pattern (e.g. matrix multiplication). A fixed data layout
is likely to have a significant performance penalty when
the access pattern changes.
Additionally, consider a case where \code{TRANSPOSE}
allows us more flexibility in query planning.
In the \code{pivot} case in Section~\ref{sec:algebra-example},
we observed that transposing the result of a pivot
is effectively a pivot across the other column. 
This flexibility allows us to potentially do the \code{GROUP BY}
on a sorted column, if it more cost effective
to do the \code{TRANSPOSE} at the end.
This is an interesting example of a
new class of potential optimizations within
dataframe query plans that exploit an efficient
\code{TRANSPOSE}. Because the axis transpositions are happening in query expressions,
the data layout becomes a physical plan property akin to ``interesting orders''~\cite{selinger1979access}
or ``hash teams''~\cite{graefe1998hash},  expanding the rules for query optimization.
}

\rebuttal{
\subsubsection{Metadata is Data (and Data is Metadata).}
Dataframes have the unique capability to move data to metadata
and back. This is available through the \code{TOLABELS}
and \code{FROMLABELS} operators, where a column of
data is elevated to the row labels in \code{TOLABELS},
or the labels are inserted into the data with \code{FROMLABELS}.
This capability provides extreme flexibility in manipulating
and coercing data, but presents some new challenges in
metadata management.
}

\rebuttal{
From the perspective
of an RDBMS, integration of row labels would not be particularly 
challenging; 
they can be defined as a ``special column'',
perhaps optimized for fast performance of filter or point queries
with an index structure. 
However in the presence of millions of rows,
a \code{TOLABELS} becomes as expensive as
creating a new index,
which is frustrating if the new labels
only serve an aesthetic purpose.
It may make sense in some cases to do a logical
\code{TOLABELS} by flagging the label column, and postpone building an index on the
labels in the interest of performance. 
% A logical \code{TOLABELS}
% would just flag a specific column as the labels and
% postpone any physical updates.
The tradeoff with this optimization will be the
speed at which filter queries on the labels can
execute. 
% If the label selection is purely aesthetic for the
% user, there is little benefit to physically reshaping the
% data, however in cases where physical reshaping is valuable,
% the dataframe system should take advantage of that time
% to build an indexing structure on the new labels to
% support faster filter queries.
This requires an understanding not only of the workload of expressions in the data science
program, but also the user's intent (Section~\ref{sec:interactivity}).
}

\jmh{I think we should redo or chop this paragraph. I think what we're saying here (that's not
somewhere above) is
that TOLABELS/FROMLABELS changes the column position values, which could cause you
to consider changing the table layout. We already said that we have expensive type induction
and optimization opportunities for table layout; I'm not sure why we're focusing on it here.
The idea that we have to redo all the column position indexing is vaguely annoying but probably easily handled
in an appropriate index.}
\rebuttal{
The column and row label metadata in dataframes 
come from the same
set of domains as the data. 
This creates new challenges in metadata placement
for dataframes. Metadata placement is likely to
become a new operator in the query plan, where
a dataframe query optimizer will need to decide whether to
keep metadata in the data or separate. 
% \dlee{It's a bit weird to call metadata placement an operator, since this is more a choice that the optimizer, it might make more sense to name a term and call the `physicalization' of metadata to data as the operator.}
Since the schema induction function $S$
is not defined on the column labels,
a column's type must be induced before
it is physically separated from the data.
This introduces new tradeoffs between physically
separating the labels from the data to create
fast point queries with indexing structures.
There is a non-trivial overhead to physically
separating a column of data into the metadata
due to the maintenance of the indexing structure,
type induction, and the cost of physical data movement. 
If the user is frequently
moving data to and from the dataframe
labels, the performance penalty for physical
updates is likely to dominate the overall query cost.
The query optimizer must model likely user interactions
in the physical plan for a \code{TOLABELS} operation.
}

\jmh{I have problems with this paragraph too. (1) This is not schema \emph{mutation}, since we don't update the dataframes, we just compute new ones.
It's not really like DDL or migrations. The example is not like DDL. And relational operations like Project ``change the schema'' of the output relative to the input. So I don't get what's new from that perspective. (2) The example doesn't require
metadata manipulation like pivot, I don't think. I believe it's an example of a groupby optimization: if your table $(X,Y,Z)$ is sorted by $X$ and you want to group by $Y$ and there are lots of different $Z$ values, you can group by $(X,Y)$ for cheap first to shrink the $Z$s away, and then group the smaller result by $Y$. I'm not sure where I've seen it, probably in datacube papers. In any case, I don't think it has much to do with schema changes.}
% TODO(smacke): figure showing different plans for pivot where output has years as column names; flatten will be more expensive if flattening over sorted year versus unsorted month
\rebuttal{
Schema changes are typically performed offline
as explicit DDL statements in relational databases. In contrast,
dataframe schemas mutate frequently \emph{during} typical queries,
thanks to the transpose and label-moving operations.
As such, {\em dataframe query
optimizers must model schema-changing operations explicitly}.
% Optimizer has to be aware of metadata (such as column labels) that will be associated with the ultimate output of certain queries, and know that we can get to this metadata in different ways
% Harken back to pivot: can either pivot one way, or do other pivot + transpose (which may make sense if the `flatten` column arg is sorted already) in order to get columns with "month" headings.
%Dataframe query optimizers will need to be
%aware of the metadata associated with the ultimate output
%of queries, and be able to retrieve
%to the desired metadata in different ways.
Consider the pivot example from Section~\ref{sec:algebra-example},
and suppose the narrow table in Figure~\ref{fig:pivot} is to be pivoted
into the wide table with \code{Month}s as columns.
The desired output can be achieved in at least two ways: {\em (i)} the straightforward way,
whereby the \code{Month} column is used in an initial \code{GROUP BY}, or {\em (ii)}
the optimized way, whereby the optimizer proceeds as if the pivot were over the \code{YEAR}
column, but then transposes the final result so that the \code{Month} attribute values
are used as column headers. 
% \jmh{Are you sure you don't need a second groupby for month? TOLABELS and Transpose won't help with the fact that there
% are $n$ copies of March over $n$ years right?
% }
These two plans are depicted in Figure~\ref{fig:pivotplans}.
The latter plan will be faster if the optimizer leverages knowledge
about the sorted order of the \code{Year} column to avoid hashing the groups.
To do so, however, the optimizer must be deeply aware of how the \code{Month} attribute values
(ultimately destined to be column headers) flow through the plan, which we foresee as a
major challenge moving forward.
}

\jmh{If I don't like FROM/TOLABELS or this schema mutation idea, what would I say here? Why is the promotion of data into metadata hard for query processing? (1) Operations like pivot or map make query cost estimation
tricky because now we have to estimate the number of rows AND columns in output. For pivot or 1-hot-encoding this is distinct value estimation so maybe some tricks, but MAP is a black box! (2) We have to derive the metadata before we derive the data, so it's easy to end up with 2-pass algorithms if you're not smart. Example: UNION over two MAPs, where the MAPs can return an unknown schema. Do we first run the maps, then scan them to figure out types, then check union-compatibility? Can we pipeline? Sorry not to write this out in more detail but it's late and I need to get to the next paper.}

% \moved{
% \code{FROMLABELS} is the opposite of 
% the \code{TOLABELS} operator, and the two of these give the
% user complete control over moving data to and from the
% dataframe's labels. This allows users to apply operators
% on the dataframe's metadata (specifically the row labels), 
% which is particularly useful for
% operators like \code{JOIN} and \code{GROUPBY}. 
% Conceptually,
% this operator also allows the positional 
% notation of the dataframe to be treated as data if
% multiple \code{FROMLABELS} are chained together. 
% However, because the order of any dataframe is immutable,
% it is impossible to update the order of the dataframe
% directly in this way. 
% Despite providing the ability to promote data to row
% labels (named notation), 
% it is impossible in this algebra to
% promote data to positional notation.
% If the users wished to reorder the
% data, they may \code{JOIN} with another dataset
% with a specific order 
% or \code{SORT} based on some column(s).
% }

% \moved{
% From a relational perspective, this operator is rather unusual
% in that it converts data into metadata.
% Dataframe users are interested in wrangling and cleaning data,
% so operations that let them move entries 
% between metadata
% and data are popular and convenient to use.
% In fact, \code{TOLABELS}
% followed by \code{TRANSPOSE} 
% is, in effect, promoting data values into column
% labels, which is impossible using 
% relational operators.
% }

% \moved{
% From a relational point of view, \code{FROMLABELS} enables
% the capability to push metadata into the data to be queried
% and operated on. 
% Thanks to this operator and \code{TOLABELS}
% specifically, column and row labels must be of type
% $\Sigma^*$ so that these operators make sense.
% \code{FROMLABELS} also has some interesting interaction
% with the schema induction function $S$, where labels
% can be interpreted as any type in $Dom$ when they
% are added to the data via \code{FROMLABELS} and then operated on. It
% is important to point that out here in the definition, but we leave
% the enumeration of the nuances of this interaction to future work.
% }


% \subsection{STOP}

% \rebuttal{
% \stitle{Lazy schema implementation challenges.}
% % \dlee{Can we have a more specific subtitle here?}
% We see one of the greatest challenge in handling the unique schema properties of
% dataframes as being the optimization of the schema induction function.
% We wager that solutions to this problem will yield a great body of work that may
% enable some new optimizations for relational systems as well.
% }

% \moved{
% The presence of a schema
% induction function allows for undefined 
% output schema of certain operators
% like \code{TRANSPOSE}
% (see the Schema ($D$) column in Table~\ref{tab:df-algebra}), 
% meaning the \rebuttal{column domains} are unknown
% in the absence of a specific array of data. 
% This can lead to runtime type
% errors in algebraic expressions 
% based on the values of data in the inputs,
% which is impossible in either relational 
% or linear algebra. 
% It is thus no surprise that dataframes 
% are most natural in languages like Python and R,
% which support dynamic typing and runtime type errors.
% }

% \rebuttal{
% Different dataframe implementations may handle types differently, or choose
% to optimize for inducing certain types over others, similar to how 
% special-purpose relational databases optimize for specific use-cases. We
% envision a dataframe landscape similar to the relational database landscape, 
% where some
% implementations adhere strictly to the data model, and others relax some 
% constraints to optimize for a specific use case. We predict that the handling
% of type induction will be a major differentiating factor between implementations
% of dataframes, in part due to how difficult it is to do generally. For example,
% an individual bytestring value of \code{``1''} may be interpreted in many
% different ways. \smquote{Some implementations may choose to forgo type induction
% altogether and handle each piece of data as raw bytes}{Not sure what this means --
% maybe an example would help?}.\smacke{TODO: talk aboutspecific example of shuffling data.} Other implementations
% may choose to interpret the \code{``1''} value depending on contextual data
% from the rest of the column and cast accordingly, e.g. \smquote{1.0 if the remaining
% values are floating point}{If we are deciding between int and float,
% isn't this technically impossible? (Since the same bytes can be interepreted as
% both floats or ints.)}.\smacke{TODO: talk about additional metadata that could be maintained to avoid an induction, e.t. that columns are ``Numeric'' after a transpose on int / float columns.} Obtaining such contextual
% data is likely to be very expensive, requiring at least a full scan of the data
% to determine what type each value should be, then casting the relevant values
% to their appropriate domain. Yet other implementations may choose to require
% a schema upfront, but we argue that these would not be dataframe 
% implementations, instead calling these dataframe-like systems. 
% This particular property of dataframes is perhaps the most unique in terms
% of other data structures and will yield a very interesting body of work
% in the future. \smacke{My main takeaway from this section is that we should try and come up with some better examples than the running int vs float.}
% }

% \rebuttal{
% \stitle{Query planning with schema induction}
% }

% \todo{hellerstein@berkeley.edu}

% \subsection{Metadata is data (and data is metadata)}


% \todo{Should we cut row schema discussion?}


% \moved{
% The asymmetry of 
% row and column types in the relational model makes 
% \code{TRANSPOSE} impossible to define for relations with non-homogeneous
% column domains (for which the sets in $D_n$ differ):
% there is no data-independent way to derive a relational 
% output schema for \code{TRANSPOSE} from the input schema. In the 
% dataframe data model, the data-dependent schema induction function
% $S$ provides an output schema.
% }

% \rebuttal{
% \stitle{Domains of the labels.}
% The explicit labels of the dataframe are a useful property. As we
% mention in Section~\ref{sec:dataframedef}, dataframes have the unique
% property that its column and row labels come from the same set of 
% domains $Dom$ as the data. This unique property can be used to labels columns or rows with data rather than just names, which enables
% some powerful expressive capabilities to the query language. 
% For example, a user may
% choose to label their columns with datetime objects and perform
% projections based on specific dates or date ranges. From the perspective
% of an RDBMS, integration of row labels would not be particularly 
% challenging; 
% they can be defined as a ''special column``
% that has some unique properties as syntactic sugar. However,
% column labels in RDBMSs typically must be labeled with a string:
% they are intentionally not represented as data for optimization
% purposes. One potential solution is to represent the column labels
% as a row of data, however this will cause problems for the schema
% if the precise domains of each of the values in the columns do not
% match the domain of the data itself, which will happen often in 
% practice. 
% }

% \subsection{Row/Column Equivalence \& Order}
% \smacke{The title of this subsection is a bit vague -- its content seems to focus
% on the independence of the physical layout of the data with its logical order,
% but there is no mention of physical layout in this subsection's title.}
% \todo{Comment how common reordering is in dataframes vs arrays/etc. (data prep)}

% \todo{Column and row ordering}


% \moved{%
% One possible starting point for an 
% in-memory representation format is
% is Apache Arrow~\cite{pyarrow}, an efficient 
% in-memory column store
% that aims to be a cross-language
% standard for flat and hierarchical tabular data,
% with high-performance
% compute kernels.  
% Arrow is not designed to be
% a user-facing dataframe library, 
% but instead aims to be the canonical 
% in-memory tabular storage format
% across systems. 
% In fact, \modin uses Apache Arrow for serialization
% of dataframe partitions when they being shuffled. 
% However, Arrow's representation 
% does not support vectors of row labels
% $R_m$ (unlike our model),
% nor does it support \code{TRANSPOSE};
% it is also not
% clear what 
% the new column labels of a \code{TRANSPOSE} 
% would be without any row labels.
% \smacke{Maybe say ``since eager schema induction is impossible
% in the case of \code{TRANSPOSE}''}
% }


% \stitle{Indexing and views.}
% Given a certain physical representation,
% operations on dataframes,
% from a relational perspective, often make use
% of ordered access, e.g.,
% editing the $i^{\textrm{th}}$ row,
% as well as access
% based on the row labels, e.g.,
% filtering based on row labels.
% Automatically
% maintaining
% indexes for this purpose can be beneficial.
% Recent work has developed positional
% indexing~\cite{bendre2018towards}, allowing ordered
% access to be supported in $O(\log n)$,
% in the presence of edits (e.g., adding or removing
% rows).
% Column stores take a different approach
% to avoid expensive edits across columns,
% instead
% recording edits separately as deltas,
% and periodically merging them back in~\cite{abadi2013design};
% it would be interesting to see which approach works
% better given a certain set of operations.
% Similarly, for matrices, accesses often
% happen in a row-major or column-major order,
% and identifying the right indexes to efficiently
% support them in conjunction
% with relational-style accesses, is an important
% challenge.
% In particular, when a dataframe
% has many rows and many columns,
% we may need both row-
% and column-oriented indexing.

% Another approach to speed up dataframe queries
% would be to defer the creation of new 
% dataframes as a result of queries
% and instead allow for the results
% of dataframe queries to be essentially
% non-materialized ``views''.
% This could be useful, for example,
% when a dataframe query essentially adds
% a new derived column for feature engineering.
% In this case, we don't actually add the derived
% column and create a new dataframe,
% simply recording the operations instead,
% and materializing the result on-demand.
% % (In fact, today's dataframe systems already share 
% % common physical storage of data across multiple 
% % derived dataframes to reduce the memory requirements,
% % but employing views would lead to further improvements\agp{citation?}.)
% Deferring the operations also opens up
% opportunities for pipelining through subsequent
% operations, saving overall computation costs.
% In fact, the Vaex project~\cite{vaex},
% which is a dataframe-like system (as we described in Section~\ref{sec:dataframedef})
% that supports querying on HDF5 files,
% implements virtual columns.
% With virtual columns,
% the column is not actually materialized
% until required for output, printing, or for a query.
% In cases where the computation
% that creates a column is expensive,
% virtual columns will
% need to be paired with intelligent caching mechanisms
% that prioritize caching
% columns that were expensive to generate.


% \stitle{Metadata managment.}
% An important new concern in dataframes,
% since they are lazily typed,
% is when
% and how to infer the types of columns and maintain
% them across operations.
% One approach is to defer type inference
% to when the operation is performed.
% However, this could lead to errors being detected
% too late, e.g., an arithmetic
% operation on a given column, which
% contains numbers except for
% a string in
% the $n^{\textrm{th}}$ row that throws an error.
% If, instead, we kept track
% of the types after operations,
% e.g., a given column contains
% mainly floats, except for
% strings in positions
% $n_1, n_2, \ldots, n_k$,
% this could accelerate the detection of
% such errors.
% However, maintaining this typing information
% also introduces overhead, and therefore
% must be balanced against the potential benefit.
% Types are often cumbersome to detect after
% a transpose; to ameliorate this, types could also be maintained
% at both the row and column level across operations,
% allowing type inference to be faster.
% For example, in Figure~\ref{fig:example},
% if we had detected that each row in \code{Out[1]}
% had
% a uniform type, we could have skipped
% columnar type inference after a transpose.


% \removed{
% \stitle{Pipelining and rewriting.}
% The next challenge emerges when processing queries involving
% the new dataframe algebra.
% Existing dataframe systems
% execute queries in an imperative way,
% one step at a time,
% and do not perform any query rewriting~\cite{mckinney2010data, R}.
% Pipelining is performed only
% when explicitly
% requested using \code{pipe}.
% Pipelining can prove to be
% effective in reducing latencies;
% for example, instead of materializing
% the result in-between two map operations,
% we could use pipelining to perform both
% at the same time.
% }

% With respect to rewriting rules, some of
% the same rewriting rules
% apply to the ordered analogs of
% relational algebra, but many don't.
% For example,
% \code{R JOIN S $\neq$ S JOIN R};
% however, this identity can be repaired
% if the right hand side is subject to an
% additional sort of the
% rows and a rearranging of the columns.
% Likewise, the set oriented operations
% do not obey commutativity due to an incorrect
% output order, but
% the incorrect order can be fixed 
% with an appropriate sorting
% of the result rows and columns.
% However, filters still commute even 
% under ordered semantics,
% when combined with the ordered
% relational operations. 
% Associativity and distributivity still apply 
% for most of the ordered relational operations.
% The \code{TRANSPOSE} operation presents
% some particularly interesting opportunities
% and challenges, and in some cases the operation itself
% can be avoided entirely
% using clever rewrite rules.
% For example, the query \code{TRANSPOSE}, \code{SORT}, \code{TRANSPOSE}
% to reorder columns can be
% rewritten as a \code{MAP} and \code{RENAME}.
% And a query \code{TRANSPOSE}, \code{SELECTION}, \code{TRANSPOSE}
% to drop columns can be rewritten similarly.

% \stitle{Cost modeling and optimization.}
% Once we have rewrite rules, the next
% step is to support cost modeling
% and query optimization.
% Current dataframe users perform manual query optimization
% by trying out various possible
% rewritten query variants to find one with low latency,
% often turning to external resources for guidance~\cite{optimizing-pandas}.
% Unlike Selinger-style query optimization~\cite{selinger1979access},
% where the notion of interesting orders is simply for performance reasons,
% here, ordering is a first-class citizen, and therefore,
% gains special prominence.
% Thus, operations that generate the output in the ``correct order'',
% e.g., a nested loop join as opposed to a hash join, are more valuable.
% When employing partitioned parallelism, query optimization
% becomes even more challenging, 
% since it may be beneficial to change
% the partitioning scheme between operations.
% For example, we may start with a row-oriented partitioning
% well-suited for map operations,
% followed by re-partitioning to a block-oriented
% partitioning to allow for an efficient transpose.
% Determining how and when to repartition in the query plan
% is an interesting challenge.


% \stitle{Summary.} Overall,
% there is a rich panoply of research challenges
% in supporting the dataframe data model and algebra
% by revisiting all
% the typical layers of a ``database stack'',
% from layout and indexing,
% to query planning and optimization.


%\stitle{Apache Arrow.}
% Apache Arrow\cite{pyarrow} is an in-memory column store targeted at setting a cross-language
% standard for flat and hierarchical tabular data. \modin uses Apache Arrow for serialization
% of dataframe partitions when they being communicated or shuffled between processes. Apache
% Arrow has an in-memory tabular format called Arrow Tables and several high-performance
% compute kernels that can be used to operate on Arrow Tables. Arrow is not designed to be
% a user-facing dataframe library, but does aim to be the in-memory storage format
% for tabular data computation. Arrow Tables do not directly conform to the dataframe data model
% presented in Section~\ref{sec:dataframedef} primarily because there is no vector of row labels
% $R_m$ in an Arrow Table. Arrow Tables also do not yet support \code{TRANSPOSE}, and it is not
% clear what the new column labels of a \code{TRANSPOSE} would be without explicit row labels.

%Some systems that market themselves as dataframes (e.g. Spark, Dask) are declarative but do not support operations
%beyond the traditional relational table operations~\cite{Armbrust:2015:SSR:2723372.2742797, dask}.

% Indeed, manual query optimization
% on the part of the developer can be a daunting task
% due to the large number of possible ways to perform an operation~\cite{wu2019diel}.
% In addition to the numerous ways of writing any given query at the API level,
% the problem is further exacerbated by the fact that
% there is a large and diverse set of operations beyond relational operators to consider when creating rewrite rules. \eat{An important area of future
% work in \modin will be in defining rewrite rules to efficiently
% handle cases that traditional systems cannot.}

%\agp{End dunno what to do with}


==> dataframe.tex <==
%!TEX root = modin-vision.tex

\section{Dataframe Example}\label{sec:usecase}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{motivating_example.png}
    \caption{Example use case of the \pandas library, highlighting the versatility of dataframes for the end-to-end data science workflow, from data ingestion, cleaning, wrangling, to analysis. 
    % \dlee{Figure suggestion: 1) highlight the 120MP and 12MP cell in line 1 and 2, 2) If we have space, add a line of description (markdown) for each cell so that the reader can get a rough idea of what is done without looking at the syntax. 3)Line 6 is doing two things at once, split out one-hot encoding and merge to separate cells if space permits.}
    }
    \label{fig:example}
\end{figure}

To illustrate how dataframes can be a more appropriate tool choice over
traditional relational tables, we consider an example of an analyst
exploring the relationship between price, rating, and product
features for different iPhone models. Figure~\ref{fig:example}
illustrates the steps taken and the results in the context
of a Jupyter Notebook\cite{jupyter}. With this example,
we aim to illustrate key aspects of a typical dataframe workflow and contrast
it with that of a relational database.

\stitle{Data ingest and cleaning.} Initially, the analyst reads in the
iPhone comparison chart
from an e-commerce webpage, as shown in the cell labeled
\code{In[1]} in Figure~\ref{fig:example}. The analyst prints out
the first few lines of the dataframe to verify that the \pandas data
loading function call resulted in the expected dataframe.
Based on this preview of the dataframe, the analyst identifies a set of subsequent actions for cleaning their dataset:
\squishlist
\item C1: The Camera description for the iPhone 11 Pro has an anomalous
value of 120MP, far exceeding the capabilities of other models. 
This is likely a data entry error.
\item C2: To make it easier to compare across different products, the
rows and columns should be switched.
\item C3: The string column "Wireless Charging" should be converted from Yes/No to 1/0.
\squishend
To resolve the data entry error (\textbf{C1}), the analyst performs spreadsheet-like
point updates to a separate cell. The cell update can be done by setting a new value for the cell at row 2 column 0 via the \code{iloc} command, as shown in
cell \code{In[3]}.
After performing the update, the analyst prints the dataframe again
to verify that the cell was updated to the correct value.

The analyst also inspects the output after operations C2-C3 and A1-A3, but we omit this in the following for succinctness.
Next, the analyst is interested in
comparing between different iPhones with attributes of the iPhones as columns
and individual iPhones as rows (\textbf{C2}). To represent each
row as an iPhone, the analyst needs to transpose the table. 
As shown in the cell \code{In[3]} in Figure~\ref{fig:example},
the analyst prints the resulting dataframe after the transpose operation (\code{.T}) 
to ensure that dataframe conforms to the anticipated schema.

Since the dataset was scraped from a webpage intended for human consumption,
the column labeled
``Wireless Charging'' contains ``Yes/No'' values instead
of a binary boolean value (\textbf{C3}), the latter of which
may be preferable for downstream processing.
The analyst
can make this change in \pandas by setting an existing
column label to the
result of a \code{map}, and define a user-defined function for that \code{map}
that modifies the data.
Using \code{map} to update columns is a common dataframe workflow pattern during
wrangling and cleaning, as depicted in cell \code{In[4]}.

To prepare integrating a different dataset into the workflow, the analyst
now loads in an additional dataset from a spreadsheet
containing price and rating information for various iPhone models,
depicted in cell \code{In[5]}.

\stitle{Analysis.} With the data cleaned, the analyst intends to perform the
following operations to analyze the data:

\squishlist
\item A1: Encode categorical features as binary indicators (0/1) across multiple columns via the one-hot encoding scheme.
\item A2: Join the product feature dataframe with the price and ratings dataframe.
\item A3: Compute the covariance between each dataframe column.
\squishend

As shown in line 1 of cell \code{In[6]}, one-hot encoding is invoked via the \code{get\_dummies} function (\textbf{A1}). Next, the analyst performs a left inner join
via \code{.merge()} on the
column corresponding to iPhone model names (\textbf{A2}). The left dataframe
contains the price and review data, and the right dataframe
is the one-hot encoded feature dataframe.

With all the relevant numerical data in the same dataframe,
the analyst now computes the covariance
between the price, ratings, and each of the individual features
via a call to \code{df.cov(...)} (\textbf{A3}).

This example demonstrated only a sample of the capabilities of the
dataframe.
Nevertheless, it serves to illustrate the common use cases for dataframes:
incremental visual inspection after most operations, point and batch updates
via user-defined functions,
and a diverse set of operators for wrangling,
cleaning, and analyzing data. Moreover, dataframes offer additional flexibility
for data manipulation compared to traditional RDBMSs.
In the following section, we formally define the dataframe,
data model, and query language.

\section{Dataframes}\label{sec:definitions}
% \smacke{Maybe call this ``Dataframe Background''?
% Or simply ``Dataframes''?
% }
%  \jmh{I wish there was history here. Is R responsible for the idea? Matlab?
% I have assumed that R is the reference, and
% Pandas is just a terrible implementation
% that we're now unwinding and expanding. 
% I realize we may 
% not want to say so in this paper, but
% knowing/sharing the history would be cool.}\dlee{I'm adding some history related to dataframes into S7.}

% Despite the fact that many systems
% market themselves as dataframes,
There are many competing implementations of dataframes in both open source and commercial products, but
there is no formal definition of the dataframe or an 
enumeration of its properties described in the literature to date.
In this section, we provide a reference data model (Section~\ref{sec:dataframedef}) and algebra (Section~\ref{sec:df-algebra}) for dataframes to ground subsequent 
discussion. 
We then
discuss an empirical study detailing commonly-used functionality
from the \pandas library (Section~\ref{sec:usage}).

\subsection{Dataframe Formalization}\label{sec:dataframedef}

Dataframes exhibit a number of fundamental deviations
from traditional relational tables.
In this section, we describe the dataframe data model
and propose a set of dataframe algebra operators that
represents the APIs and operators in
traditional dataframe implementations like \pandas and R.

% \smacke{I like the bit about the inherent symmetry,
% but this still feels a bit too vague in my opinion.
% Since dataframes are best understood by the
% functionality they provide, would it make more sense
% to give a formal specification of properties that
% dataframes exhibit? E.g. 1. two-dimensional ordered data, 2. typing and labels / names attached to both rows and columns,
% 3. symmetry between rows / cols (anything that holds for cols holds for rows and vice versa), 4. weakly schema'd, 5. provides API with host interpreted
% language for use in an interactive environment like
% a Jupyter notebook.}
% We define a dataframe as an {\em ordered} tabular relation \dorx{???}
% \smacke{Maybe say: {\em Dataframes} organize data in two dimensions
% and allow for many of the same operations permitted by traditional relational
% algebra, while also enforcing {\em ordering semantics} in both the rows and
% columns and allowing for additional expressivity due to the inherent
% symmetry between rows and columns.}


\subsubsection{Dataframe Data Model}
Due to the wide and varying use of the term {\em dataframe},
we now propose a formal definition. 

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\begin{definition}{Dataframe:}
A dataframe is an ordered collection of tabular data
with inherent symmetry between rows and columns. In
a dataframe, both rows
and columns are associated with a label, are ordered,
and have types.
\end{definition}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{dataframe_data_model.png}
    \caption{The dataframe data model.
    %  \smacke{From in-person discussion: ``relational table''
    %  includes DB schema $\Leftrightarrow$ column metadata, so we lose a bit of symmetry with the
    %  row metadata by calling the inner big box a ``relational table''. Alternative suggestion:
    %  call it ``relational data'' or ``tabular data'' and then say that combined with 2, 4, 5, and
    %  maybe 6? Then we have a relational table.}
    }
    \label{fig:datamodel}
\end{figure}

At a high-level a dataframe is an {\em ordered}
tabular relation. Dataframes contain an inherent
order for rows and columns which is commonly used for display purposes, order-dependent
operations (e.g. \code{CUMULATIVE MAX}), and selection/projection.
Unlike users of the relational model, dataframe users heavily 
depend on the order of the data in their workflows, 
similar to the users of a spreadsheet. 
A user expects to see and operate on the data in the exact order
that it was ingested.
It is important to note here that the data model
is {\em ordered}, but not necessarily {\em sorted}. This
distinction is important because the order that the user
prefers may not necessarily be the sorted order of any
column in the dataframe. Some recent systems \cite{dask} have adopted a
sorted data model, which deviates from the data model of 
traditional dataframe systems like \pandas and R.

Metadata in dataframes are treated differently than that
in the relational data model. 
Columns and rows in a dataframe are equivalent
and can be treated interchangeably. This
property is also shared with matrices, where columns and rows both
have associated metadata. As a result, columns {\em and} rows have
data types, labels or names, and an order.

Figure \ref{fig:datamodel} shows a high-level overview of the data
model as it relates to a relational table. The various components
of the dataframe data model will now be explained in detail.

\noindent\circled{1} \stitle{Tabular data.} The tabular data in a
dataframe is a ``grid'' of 2-dimensional data. In this data model,
the tabular data need not be physically ordered so long as the order ranks of each row and
column are maintained in the row and column metadata.

\stitle{Columns.} Columns in a dataframe are conceptually similar to
relational table columns: a series of row values for a particular
label. In dataframes, the columns are ordered, such that a column
can be projected either from its column label or its numeric index
in the column labels.

\noindent\circled{2} \emtitle{Column Labels.} The column labels identify a given column.
Unlike relational algebra, in a dataframe, column labels
have a name and data type. The data type is useful for
classifying non-string data. Dataframes support
hierarchical column labels in the form of multiple column label ``rows'',
each having an individual type and a name.

\noindent\circled{3} \emtitle{Column Metadata.} The column metadata contains each
column's data type and rank order. The rank order for the
column is present to ensure that the column order is maintained
as well. The type of the columns can be \code{ANY} type, which subsumes
all other types.

\stitle{Rows.} Rows in a dataframe are an ordered tuple of values
associated with a given row label. Rows can be selected either by their label
or by the integer offset of the row in rank order. For example,
in Figure~\ref{fig:example} \code{In[2]}, the row was selected
via \code{iloc}, which is the integer rank of the row. This row
could have also been selected via \code{loc["Front Camera"]}, which
is that row's label.

\noindent\circled{4} \emtitle{Row labels.} The row labels in a dataframe
identify a row. They are collectively one or more 
special columns in the
dataframe, primarily serving as to give symmetry
with columns (so that rows have names just
like columns, particularly useful after a dataframe
transpose). An important distinction between row
labels and the primary key of a table is that
these row labels need not be distinct.
They also provide syntactic sugar for
selecting rows. The row labels column(s)
has a name and can be any data type. The
order of the dataframe is not necessarily
the lexicographic order of the row labels. As with
column labels, dataframes support
hierarchical row labels in the form of multiple row label columns,
each having an individual type and a name.

\noindent\circled{5} \emtitle{Row metadata.} The row metadata contains
each row's data type and rank order, 
an integer offset. The collection of offsets is called
the order column, and can be
conceptualized as an invisible column that allow each row
to be accessed by its offset. Note that in the relational
model, because order is not guaranteed between queries,
this metadata represents the user's row order. Additionally,
each row has an associated type, ensuring
that columns are typed after a transpose. As with columns,
the type of the rows can be \code{ANY} type, which subsumes
all other types.

\noindent\circled{6} \stitle{Global metadata.} The global metadata
serves the function of being metadata about the dataframe's metadata.
Column labels and row labels can have a ``name'', which can make
hierarchical labels distinct and individually accessible. The global
metadata also holds the types of the row and column labels.

\subsubsection{Data model Comparisons}
We now illustrate some of the key similarities and differences
between dataframes, matrices, and relational tables.

\stitle{Comparison with matrices.}
It may be tempting to classify a dataframe as a matrix or an array
with column and row labels.
While such an abstraction would exhibit some of the properties
of dataframes, matrices on their own are not capable of capturing
polymorphic behavior due to differing data types. The abstract
notion of a ``matrix'' does not have a schema, and all the entries
of a matrix must be of the same type so that the matrix is an
element of a vector space over a particular field. For this reason,
it does not make sense to, say, compute the mean of some matrix
column using groups defined by the elements of another column (a group by);
if the matrix elements are categorical, numeric operations like
``take the mean'' lack well-defined semantics, and similarly if
the matrix elements are real-valued, computing groups for a
``group by'' operation likewise does not make sense.
Rather, dataframes subsume matrices: different subsets of dataframe
rows and/or columns with the same numeric type can be used in
familiar linear algebra operations while preserving their relationship
to other dataframe rows / columns when it is desirable to do so.

\stitle{Comparison with relational tables.}
Due to the presence of schema and typing information, dataframes are
more closely related to traditional relational tables than
to matrices. However, it is precisely the characteristics
that are shared with matrices that serve to distinguish
dataframes from traditional relational tables. Namely, in
dataframes, both rows and columns are {\em ordered} and can
be selected via a label or rank order. Furthermore, just as matrices have
symmetry between rows and columns, so do dataframes: while
relational tables typically only give names and types to columns,
dataframe schemata assign names (called ``labels'') and types to rows
as well, so that a dataframe ``transpose'' has well-defined
semantics. It is not surprising, therefore, that dataframes evolved
primarily in runtime-typed languages like Python and R, which allow
for schema-level types like ``Object'' or ``Any'', so that the
same row or column can contain multiple different runtime types.

\stitle{Comparison with spreadsheets.}
Dataframes have many features inspired by and in common
with spreadsheets. Both enable single-point updates
to individual cells and have a data model where
columns and rows are both ordered. In spreadsheets,
however, the data representation can be sparse with
multiple empty values and gaps between data cells.
It is possible in the spreadsheet data model to keep multiple
datasets in the same spreadsheet with some empty cells
separating them. The spreadsheet data model comes at the
cost of complexity in implementing relational operators.
Dataframes, on the other hand, do not allow for this sparse
representation. Dataframes have a dense representation, where
one dataframe correlates to one dataset, enabling easier
implementation and optimization of relational operators. 

\subsubsection{Dataframe Algebra} \label{sec:df-algebra}

\begin{table*}[]
\begin{tabular}{|l|c|c|c|c|l|}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Operator} & \textbf{Metadata} & \textbf{Data} & \textbf{Origin} & \textbf{Order of Result} & \textbf{Description}                                       \\ \hline
UNION             &                   & \xmark             & REL             & Parent$^\dag$            & Set union of two dataframes                                \\ \hline
INTERSECTION      &                   & \xmark             & REL             & Parent$^\dag$            & Set intersection of two dataframes                         \\ \hline
DIFFERENCE        &                   & \xmark             & REL             & Parent$^\dag$            & Set difference of two dataframes                           \\ \hline
SELECTION         &                   & \xmark             & REL             & Parent                   & Eliminate rows                                             \\ \hline
PROJECTION        &                   & \xmark             & REL             & Parent                   & Eliminate columns                                          \\ \hline
JOIN              &                   & \xmark             & REL             & Parent$^\dag$            & Combine two dataframes by element                          \\ \hline
RENAME            & \xmark                 &               & REL             & Parent                   & Change the name of a column                                \\ \hline
DROP DUPLICATES   &                   & \xmark             & REL             & Parent                   & Remove duplicate rows                                      \\ \hline
GROUP BY          &                   & \xmark             & REL             & Parent$^\dag$            & Group identical attributes                                 \\ \hline
SORT              & \xmark                 &               & REL             & New                      & Lexicographically order rows                               \\ \hline
MAP               &                   & \xmark             & DF              & Parent                   & Apply a function uniformly to every row                    \\ \hline
FLATTEN           &                   & \xmark             & DF              & Parent$^\ddag$           & Convert elements containing collections into multiple rows \\ \hline
WINDOW            &                   & \xmark             & DF              & Parent                   & Apply a function via a sliding-window (either direction)   \\ \hline
TRANSPOSE         & \xmark                 & \xmark             & DF              & Parent$^\lozenge$                & Swap data and metadata between rows and columns            \\ \hline
AS LABELS         & \xmark                 & \xmark             & DF              & Parent                   & Set one or more data columns as the row labels column(s)             \\ \hline
RESET LABELS      & \xmark                 & \xmark             & DF              & Parent                   & Convert the row labels column(s) into a data column        \\ \hline
AUGMENT           &                   & \xmark             & DF              & Parent                   & Create a new column from a function applied to another     \\ \hline
\end{tabular}
\caption{
Dataframe Kernel Algebra. \hfill\break
$\dag$: Ordered by left parent first, then right parent to break ties. \hfill\break
$\ddag$: Ordered by parent first, then by the order of the collection. \hfill\break
$\lozenge$: Order of columns is inherited from order of rows and vice-versa.
}
\label{tab:df-algebra}
\end{table*}


In this section, we propose a set of operators that encompasses
most functionality provided by dataframes. The
purpose of this section is to help frame the
dataframe definition and explicitly contrast dataframe
algebra with relational algebra. We do not
argue that this is the minimum set of operators. 
\devin{We cover a lot and will show by examples}. At this time,
we use this set of algebra to help explain the significant
difference between dataframe algebra and relational algebra
and the challenges in bringing this algebra to traditional relational
systems.

The kernel of operators we have derived are described in
Table~\ref{tab:df-algebra}. Our proposed dataframe algebra ecompasses
ordered analogs of the
operators from the extended relational algebra.
Dataframe algebra additionally supports other
data and metadata transformation operators,
and three operators that transforms
both data and metadata: \code{TRANSPOSE}, \code{AS LABELS}, and \code{RESET LABELS}.
Since these are the
main deviations from relational algebra, we
will describe the additional data and metadata manipulation
operators in detail.

\stitle{Transpose.} 
Transpose interchanges column and row metadata, so that the columns of the
dataframe become the rows, and vice-versa. 
Not only does this allow users extreme flexibility when coercing
a dataset to their desired schema and orientation, but it also
allows them to perform SQL operations along either columns or rows.
In our example in Section~\ref{sec:usecase}, we note a case where
the table was not oriented
properly from ingest, and a transpose was required to give us the desired
table orientation.

In \pandas and other dataframe implementations, it is possible to
perform operations along either the rows or columns via the \code{axis}
argument. We simplify this in the design of the algebra by defining
operators only on the rows and defining the \code{TRANSPOSE} operator.
To do an operation along the columns, take the \code{TRANSPOSE}, apply
the operator, then take the \code{TRANSPOSE} again to return to the
original orientation.
With this flexibility, operators
on the dataframe can be performed along either the columns or
the rows.

\code{TRANSPOSE} presents unique challenges for traditional relational systems
primarily because of the metadata transformation needed.
Relational algebra
does not have an abstraction that provides the ability to
efficiently swap the axes and modify the metadata in this way.
While prior work in the relational literature
describes how to perform
a \code{PIVOT} in a relational database~\cite{cunningham2004pivot},
it is not in general possible to transpose a relational
table with columns of varying types without losing typing information,
as the schema only tracks column-level (and not row-level) metadata.
\code{TRANSPOSE} can also be extremely computationally expensive
depending on the relational database's architecture and partitioning.
In the implementation of \code{TRANSPOSE}, often it will
be important to postpone the calculation of \code{TRANSPOSE}
until the last possible moment because of the associated computation
costs.

\stitle{Map.} The map operator takes some function {\em f}
and applies it to each row individually. The function
{\em f} has only a single requirement: for each row input
there must be a single row output with the same number of attributes.
Thus, the output dataframe will be contain the same number of columns
and rows as the input.
The purpose
of the map operator is to alter the data of each dataframe element
uniformly. \code{MAP} is useful for data cleaning
or to wrangle certain data that is poorly structured
or lacks appropriate formatting (e.g. Figure~\ref{fig:example} \code{In[4]}).

Extended relational algebra supports map via the use of functions
in the subscript of projection operators (i.e., in the \code{SELECT}
clause of SQL). The primary challenge associated with porting map
to existing relational systems is the fact that the dataframe map
is capable of operating on many columns without explicitly naming
them. For example, in a relational system,
the equivalent of a \code{fillna} operation would
likely require code refactoring after a schema changes introduces an
additional column (wherein the new column is explicitly named in the
\code{fillna} equivalent), but no such refactoring is necessary if
an additional column is added to a dataframe.

\stitle{Window.} Window is an operator that is order-dependent
and takes some function {\em f} and applies
it on a sliding-window of a column of the data. The function {\em f} has the special
requirement that it must be applied in the order of the rows,
and the number of output rows for a given window is 1.
Like \code{MAP}, the resulting dimensions of the dataframe
are identical to the input dataframe.
Window allows an arbitrary number of previous rows to
be passed as a parameter to the function {\em f} and can
slide in either direction.

The main challenge that window presents to traditional relational
systems is the order requested by the user. Many relational database
systems already support some version of
window functions \cite{postgresql_window}, so the only additional consideration
would need to be ensuring that
the order is correct.

\stitle{Flatten.} The flatten operator splits a dataframe
element containing an ordered collection (e.g. list)
into multiple dataframe elements, one element for each
element in the collection. This results in
an increased number of rows in the dataframe. The
values in the other columns and the row labels
of each row are replicated for each resulting row in the
flattened dataframe.
Flatten maintains the original order of the dataframe,
but adding rows follows the rank order of the collection
in that column. The
main use-case for flatten is to normalize the dataframe,
such that each row represents a single piece of data.

There are relational database implementations that support
a \code{FLATTEN} operator\cite{postgresql_unnest}. The order semantics
of dataframes may pose some additional challenges related
to correctly setting the rank within the row's metadata to ensure
correct order of the result. \smacke{This doesn't seem like a
unique difficulty faced by relational tables -- if it's been solved
by dataframes, I don't see why a relational system can't just borrow
the same technique?}

\stitle{As Labels.} The \code{AS LABELS}
operator projects one or more columns out
of the tabular data to be
set as new row labels for the
dataframe, dropping and replacing the old labels.
The type(s) of the new labels are inherited
from the type of the column(s) that are set
as the new labels.
This allows the user to have some control over
the row labels they interact with. With this capability,
data can be moved into the dataframe's metadata.

From a relational database perspective, this operator is
rather unusual, because users do not typically interact
with the metadata of a table. Despite this, in a relational
context, the ``movement" of data to metadata could be done
by simply updating the metadata of the selected columns.
Since the row labels can be thought of as ``special columns", it suffices
to update the metadata for the columns. As for a projection,
the rank-order metadata will need to be updated as well.
\smacke{I'm lost after reading this entire paragraph.
Skipping and moving to the next operator.}

\stitle{Reset Labels.} \code{RESET LABELS} takes all of the row label columns
and sets them as data columns at position 0.
The respective data types of the new column(s)
are directly inherited from the labels column(s).
The labels are set to the default label:
the order rank of each row. \code{RESET LABELS} is the opposite of 
the \code{AS LABELS} operator, and the two of these give the
user complete control over the row labels, and with \code{TRANSPOSE},
column labels as well. This allows users to apply operators
on the dataframe's metadata, which is particularly useful for
operators like \code{JOIN}, \code{GROUP BY}, and \code{DIFFERENCE}.
Many \pandas operators treat the metadata of a dataframe as data, so
it is important to enable the ability to move columns between
the metadata and the data to support this behavior. Conceptually,
this also allows the order of the dataframe to become data if
multiple \code{RESET LABELS} are chained together. However,
because the order is only mutable in the context of a \code{SORT},
it is impossible to update the order of the dataframe
directly in this way.

In a relational context, \code{RESET LABELS} poses
unique challenges. Inserting the new columns
at position 0 will cause the metadata of all columns
to be updated because each order rank will be shuffled
by the number of columns inserted. The typing information
is maintained between row/column labels during this operation
and its opposite, \code{AS LABELS}. The fact that metadata
can become data explains the need for typed labels.
\smacke{Again, I don't understand why this difficulty is
unique to relational systems. If we can solve it in a system
that uses dataframes, why aren't those techniques directly
applicable to the relational system? To put it in a different
way, the challenge outlined above seems just as applicable
in the context of dataframes.}

\stitle{Augment.} Augment creates a new column in the dataframe
at the last position, \code{LENGTH(COLUMNS)},
from the result of some function \code{f} on the rows. 
The name of the new column is provided at invocation. The
function \code{f} must take as argument an entire row
and must return a single value to be inserted into the new
column. For example, the function can sum the numeric
columns of a row. For users, it is often useful to
see some summary statistics alongside the regular
data.

\code{AUGMENT} can be reduced to a \code{MAP} followed by a \code{PROJECT}
and \code{UNION}. We create this operator as a simplification
of these steps, and there is a precedent for this
in relational algebra with \code{JOIN} being \code{CROSS PRODUCT}
followed by a \code{SELECT}. This operator is already
supported by most relational database implementations
with the \code{SELECT} statement: \code{SELECT ID, V1, V2, V1 + V2 FROM table}.

\subsubsection{Kernel Algebra demonstration}\label{sec:algebra-example}

In this section, we demonstrate how a few of the more
exotic \pandas operators can be written with
the algebra presented in Section \ref{sec:df-algebra}.

Some examples of map operators in the \pandas API are:

\squishlist
\item \code{fillna}: Convert NULL values to another value.
\item \code{isna}: Determine if a dataframe element is NULL,
often used as a step in counting NULL values.
\item \code{str.upper}: Converts the string element to upper-case.
\squishend

Some examples of window operators in the \pandas API are:

\squishlist
\item \code{cummax}: Take the cumulative max of a column.
\item \code{diff}: Take the difference between an element and its neighbor.
\item \code{shift}: Shift rows down to align with a new row label,
maintaining the order of the data.
\squishend

\code{AS LABELS} is captured in the \pandas API by the following example operators:

\squishlist
\item \code{set\_index}: Set the dataframe row labels using existing column(s).
\item \code{reindex}: Conform the dataframe row labels to new labels.
\item \code{index}: The row labels of the dataframe. They can be assigned to a column.
\squishend

Flatten is used as a part of the follow \pandas operators:

\squishlist
\item \code{explode}: Transform each element of a list-like to a row, replicating the row labels.
\item \code{melt}: Unpivot a dataframe from wide format to long format
\squishend

\code{RESET LABELS} is captured in the \pandas API by the
\code{reset\_index} method.

There are several \pandas operations and behaviors that require
\code{TRANSPOSE} when defined in this algebra.
We present a sample of these operators, to be further discussed in
Section~\ref{sec:algebra-example}:

\devin{Move these to the next section}

\squishlist
\item \code{transpose}: Transpose column and row labels.
\item \code{pivot}: Return reshaped dataframe organized by given row/column values.
\item \code{stack}: Stack the prescribed level(s) from columns to rows.
\squishend

\subsubsection{Workflow definitions}

In this section, we describe the definitions of different
components of a given dataframe workflow.

\stitle{Operator.} A dataframe operator is a single
API call on or with a dataframe. This follows the SQL definition
of an operator, see Section \ref{sec:df-algebra} for the operators
exposed in dataframe APIs.

\stitle{Statement.} A dataframe statement is the smallest unit of 
submission a user can
provide to the system and contains one or more operators.
This presents itself in different ways depending on how
the user is interacting with the dataframe system. In an interpreted
environment (e.g. iPython), this will be a single block of code.
In a notebook environment, a statement is a single cell. We define
a statement in this way to draw parallels to a single SQL query statement
in the way it is interacted with, however a statement is not a full
query.

\stitle{Query.} A dataframe query is a series of statements that are
composed to answer a larger overall question. If we consider the 
data\-frame system as a DAG
of operators and their dependencies, a query ends at each of the
leaf nodes. A dataframe query is the equivalent of a SQL query.

\stitle{Session.} A session is a complete, end-to-end workflow. It
begins when the user starts a notebook or interpreter environment
and ends when the user shuts down that environment. A session
is composed of one or more queries. Because dataframe systems
are typically in-memory, the results of the query are not
persisted unless the user explicitly expresses this by writing
the result to a file.

% \subsection{The history of the dataframe}\label{sec:history}
% \agp{This is a biased set of rough notes.}

% \stitle{Asynchronous Computation.}
% Battle and Heer~\cite{Battle2019} studied how analysts perform exploratory visual analysis and found that 
% the speed of analysis often involves long ``think time'' for performing complex inference task. They also found that many exploratory workloads can be ``bursty'', involving long think time, followed by a sequence of fast and small experimentation steps.smaller things fast). These characteristics of analytical behavior motivate asynchronous computation, a middle-ground between eager and lazy evaluation that maximizes the use of CPU and idle time to ensure interactivity when iterating on dataframes. Asynchronous computation have also been applied to reduce the overhead associated with web requests when combining Web and relational queries~\cite{goldman2000wsq}, enabling users spreadsheet control during long, complex formula computation~\cite{bendre2019anti}, and reducing crowdsourced query execution by parallelizing tasks involving high, human-incurred latency~\cite{parameswaran2012deco}.

% % Examples of existing systems that makes use of asynchronous computation include: 
% % WSQ/DSQ: embedding search queries into SQL
% % w/ asynchrony~\cite{goldman2000wsq}, asynchronous formulae
% % in spreadsheets~\cite{bendre2019anti}, embedding crowd queries into SQL w/
% % asynchrony~\cite{parameswaran2012deco}, AIDA~\cite{Dsilva2018AIDAA}


% \stitle{Partial Results.}
% To ensure interactivity on large datasets for exploratory analytics, a popular approach has been to return approximate or partially-computed results to users progressively throughout their analysis~\cite{Fekete2018,hellerstein1997online}.
% \cite{raman2002partial,lang2014partial,viglas2002rate}
% optimizing for the LIMIT clause in SQL queries~\cite{kim2018optimally}


% \stitle{Approximate Computation.} \cite{hellerstein1997online}
% \smacke{I'm not sure that ``dataframes'' as we think of them
% have been given much specific attention in the AQP literature.
% Also, if we want to keep this, maybe we should merge with the
% preceding ``Partial Results'' bullet?}

% \stitle{Other Dataframes.} 
% Parallelized: Dask~\cite{dask}, SparkSQL~\cite{Armbrust:2015:SSR:2723372.2742797}, Weld~\cite{DBLP:journals/corr/abs-1709-06416}, ... 
% Regular dataframes: R~\cite{R}, \pandas~\cite{mckinney2010data}
% AFrame~\cite{sinthong2019aframe}

\subsection{Dataframe usage statistics}\label{sec:usage}

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{user_stats.png}
    \caption{Pandas user statistics from Github dataset.}
    \label{fig:user_stat}
\end{figure*}

To study how dataframe users interact with the \pandas API, we analyzed a comprehensive dataset of 1 million Jupyter notebooks hosted on \hyperlink{github.com}{github.com} from Rule et.al.~\cite{ucsd-dataframe-study}. Out of the 1 million Jupyter notebooks, about 40\% imported and used the \pandas dataframe library at least once. We will focus on three questions to investigate how people work with \pandas. 

\stitle{What are some high-density functions used in interactive analysis?}
We studied the \textit{total} occurrence of each \pandas dataframe method in our data. The most notable methods are methods to inspect the data (\code{plot, shape, head}), methods to perform numeric aggregation (\code{mean, sum}), methods to perform relational operations (\code{groupby, join}). It is worth noting a lot of data modification (both point queries as well as column and row queries) using \code{loc, iloc, drop, append}. Columns and index metadata inspection and manipulation are common as well with \code{index, columns}. 

\stitle{What kind of functions were common in day-to-day usage?} 
We counted the number of files that each \pandas methods has occurred in. The occurance measures the frequency of usage per analytic job.
The most commonly used methods are used to perform actions such as creating DataFrames (\code{read\_csv, DataFrame}), inspect partial result (\code{head, shape}), visualizing result (\code{plot}), perform aggregation (\code{mean, sum, max}), perform point queries (\code{loc, ilo, ix}), adding or removing data (\code{append, drop}), apply arbitrary user defined transformation (\code{apply}), relational operation (\code{groupby, join}). It is worth noting that type-casting (\code{astype}) and direct access or manipulation of columns and index metadata, and underlying data storage (\code{columns, index, values}) are also high in the list. 

\stitle{What are some methods are common used together?}
We also investigate the number of co-occurrence of methods in the same line of code. This typically mean user chaining \pandas method together or calling them inside a single statement. For example, \code{df.dropna().describe()} is fairly common across our sample. It is also common for \pandas user to perform multiple operation in single execution cell. For example, \code{print(result = df["col1"].mean(), df["col1"].max())} prints a tuple of summary statistics. The popularity of chained or parallel invocation suggest opportunities to accelerate one statement at a time as well accelerate multiple statements at a time. 

% \stitle{Footnote} Method: We used \code{jupyter nbconvert} to convert notebook to python script, \code{2to3} module to transform python 2 to python 3, and python \code{ast} module to parse and extract method invocation. Some method counters might be noise. For example, \code{.append} is both a python built in list method as well as a \pandas method. 


==> flexible-schema-old.tex <==
\moved{
% \stitle{New Challenges in Dataframe Types.}
When the domain for any dataframe column is left
unspecified, it can be induced via
the schema induction function $S$.
In doing so, $S$ must examine
every value in that column
to determine the most specific
domain from $Dom$ that can be used
to classify the data in that column. 
Since $S$ is applied by the system on-demand,
it can be done lazily or eagerly, presenting
optimization opportunities. 
For example, the $\code{map}$
operation in step C3 in  Figure~\ref{fig:example}
involves a function that explicitly
transforms elements in a given column into
boolean values, allowing us
to infer the output type for that column.
As another example, prior to the \code{.cov()} operation
in step A3, 
we need to verify
that the dataframe is a matrix dataframe;
this could be done lazily when the \code{.cov()}
is called. 
}
\rebuttal{
Since types do not need to be declared upfront, many relational
optimizations cannot be employed until the
types are induced via the schema induction function $S$, defined in
Section~\ref{sec:dataframedef}. When this is paired with the composable
nature of the query language, types may have to be induced many times,
even within a single query. In this section, we discuss the implications
of the {\em post-hoc} type induction feature of dataframes and some candidate
avenues of research into the optimization of schema induction.
}

\rebuttal{
\stitle{Row and Column Typing.}
}
\rebuttal{
One potential optimization would be to
maintain a row-level schema as well: a per-row domain from $Dom$ defined in 
Section~\ref{sec:dataframedef}. There would be significant 
storage overheads to
maintaining fine-grained row-level metadata for tables which
have billions of rows or more.
First, an implementation can induce the types of the columns from the
data itself after the \code{TRANSPOSE} operation has been completed.
This operation is expensive, and
may not be necessary if the row types of the input dataframe are
already known.
Alternatively, one could infer the row schema without materialization
as the supertype of
all column domains in the dataframe, $D_n$. When a \code{TRANSPOSE}
is invoked, the new column domains can be computed as the domain
which represents all domains in $D_n$. This, however, may result in
lossy behavior. Consider the case where multiple \code{TRANSPOSE}
operations are chained together: \code{TRANSPOSE(TRANSPOSE(DF))}.
Unless all domains are the same, as is the case with a homogeneous
dataframe, the first \code{TRANSPOSE} will result in 
domains that are more generic than the initial domains, often
$\Sigma^*$, a bytestring. The second \code{TRANSPOSE} will reorient
the dataframe into its original position, but with all of the domains
identical the original type information has been lost. This particular
case can be solved by adding a rule for chained \code{TRANSPOSE}
operations, but in some cases the correct types for a row cannot
be inferred from the column domains of the input data. For example, in the workflow in Section~\ref{sec:usecase}, if the data contained a 
row with only
floating point data, the type of that row would be induced as $float$,
however if we infer the
resulting column domains after a \code{TRANSPOSE} based on the input
domains, the system will lose precise domain information for that column.
}

\rebuttal{
In practice, it is common during data cleaning and querying
to inspect the types
of a dataframe at runtime to ensure that operations will behave as
expected. Systems which implement the dataframe data model will need
to allow for runtime inspection of the types, and additional
challenges emerge when attempting to enable this functionality
underneath lazily-induced schemata. If types for a dataframe are not
yet specified, they will need to be induced, or materialized,
via the $S$ function defined in Section~\ref{sec:dataframedef}.
}
\rebuttal{
A dataframe system may not need to materialize the entire
types depending on the information user needs to make
a decision.
For example, a user may only need to know
that the domain of a column is numeric, and not need to know
whether it is \st{int} or \st{float} specifically. Determining
whether or not the type of a column is numeric will be significantly
faster than inducing a specific type on an entire column.
In other cases, a user may be satisfied with a best guess of
the type for a column until the actual type is
materialized. Providing a guess of the type of the column based on
a subset of the rows will also significantly improve the
responsiveness of the dataframe system for the user.
% \smacke{I wonder if there is a cooler example for this
% paragraph than just int vs float.}
}

\rebuttal{
\stitle{Lazy vs. Eager Type Induction.}
\moved{
An important new concern in dataframes,
% since they are lazily typed,
is when
and how to infer the types of columns and maintain
them across operations.
One approach is to defer type inference
to the time of operation invocation.
However, this deferred induction could delay
error detection unacceptably. Consider
an arithmetic
operation on some column
containing all numbers except for
a string in
the $n^{\textrm{th}}$ row -- the type error will
not be apparent until this row is processed.
If, instead, we kept track
of the types after operations
(e.g., a given column contains
mainly floats, except for
strings in positions
$n_1, n_2, \ldots, n_k$),
this could accelerate the detection of
such errors.
However, maintaining this typing information
also introduces overhead, and therefore
must be balanced against the potential benefit.
Types are often cumbersome to detect after
a transpose; to ameliorate this, types could also be maintained
at both the row and column level across operations,
allowing type inference to be faster.
For example, in Figure~\ref{fig:example},
if we had detected that each row in \code{Out[1]}
had
a uniform type, we could have skipped
columnar type inference after a transpose.
}
}
\todo{
\squishlist
\item At a high level schema induction should be regarded as another operator in the query plan. Lazy v.s. Eager is a special case of the query planning problem. 
\item Schema induction in general is expensive so we should think about costing it as part of query plans. 
\item By chaining relational operators together, we can avoid having schema induction ``in-between'', which argues for rewrite rules that can help with that.
\item Laziness is beneficial because it delays an expensive operation
\item Eager reduces query latency
\squishend
}

\rebuttal{
\stitle{Type Induction Mechanisms.}
}
\todo{
\squishlist
\item We want to avoid the use of S if we can infer it automatically
\item Identifying types of UDFs for Maps 
\item If you are restricted to ord relational ops, it can be automatically inferred; 
\item Maintain small data structures for incremental schema update. For certain columns if it is succinct (low entropy), you can record a summary of the types across values 
\item Detect if the type has changed (from Obj to a number)
\item Approximate schema inference:
\item If you have columns whose types you know are ints and floats, then you know that after a transpose you still have a table that can be interpreted as “numeric” (inference just from column types prior to transpose)
\squishend
}

==> groupby-and-window.tex <==
\stitle{\rebuttal{GroupBy.}}
\rebuttal{
The \code{GROUPBY} operator in our proposed algebra is analogous to that
of traditional relational database systems, with a key difference. In normal
SQL, a \code{GROUPBY} is always paired with some sort of aggregate, e.g.\ \code{SUM},
\code{AVG}, \code{FIRST}, etc. The flexible schema admitted by dataframes permits the
use of \code{GROUPBY} {\em without} a companion aggregate, as dataframe schemas are flexible
enough to admit multiple ``rows'' in the rows of the dataframe output by \code{GROUPBY}.
While current implementations like Pandas always materialize the \code{GROUPBY} dataframe\footnote{Technically,
a Pandas \code{GROUPBY} additionally performs a \code{TOLABELS} and a \code{MAP}+flatten in terms of
our proposed algebra.}, an optimized implementation could detect via program analysis techniques
when the output of a \code{GROUPBY} is immediately passed to an aggregate as an rvalue, obviating
the need for materialization; we foresee developing such an optimizer capable of this kind of
static analysis as a major challenge moving forward.
}

\stitle{\rebuttal{Window.}}
\rebuttal{
\code{WINDOW}-type operations are arguably more natural to express
in a dataframe setting than in a relational setting for two reasons.
First, because some operations require an additional ordering context,
many SQL windowing functions require the additional use of an \code{ORDER BY}
clause so that functions like \code{LAG}, \code{LEAD}, etc.\ are well-defined.
In our proposed dataframe algebra, the dataframe already has an ordering,
obviating the need for this additional clause (although an \code{ORDER BY}
can always be optionally done prior to a \code{WINDOW} if an alternative order
is desired). Second, SQL does not permit the use of \code{GROUP BY}
in conjunction with windowing functions in order to specify partitions.
Instead, SQL windowing operations are typically accompanied with a
\code{PARTITION OVER$(\ldots)$} clause, where $(\ldots)$ contains some
expression.

In dataframe algebra, the same effect can be achieved through
the use of our \code{GROUPBY} operator, since this operator actually
partitions the data over the group attribute, unlike the SQL \code{GROUP BY}.
Furthermore, even if the expression used to create partitions is not a simple
column name but a more complicated expression (e.g.\ $df.x + df.y$), dataframe schemas are flexible,
allowing for the creation of a new column for this expression that is
computed via the \code{MAP} operator, and then passed
to the \code{GROUPBY}. In many ways, \code{WINDOW}
functionality feels ``bolted on'' to traditional SQL, but for dataframes
it is elegantly expressible by composing existing algebraic primitives, although,
as with \code{GROUP BY}, eliminating unnecessary materialization is a major challenge.
}

==> interactivity.tex <==
\section{Optimizing for Interactivity~\label{sec:interactivity}}

With dataframes,
users tend to build their queries incrementally, where multiple
statements compose a larger overall query. 
These queries are typically
built in a trial-and-error approach with sub-queries that are
reused multiple times. 
Interactivity, defined by quick feedback, is highly desirable with this style of development.
To optimize for dataframe interactivity, we are required to consider two properties that are not typical in the traditional database use case:
(i) users are more amenable to partial and approximate feedback
(ii) a larger portion of the optimization opportunities exist across multiple queries.
We identify research opportunities associated with each of these properties in the rest of the section.
\devin{Mention skinner and citations of that paper}

\subsection{Evaluation Paradigms}
\smacke{AGP: merge this with 6.2?}

In the \stitle{Eager Computation} paradigm,
users are forced to wait for computation to complete 
after each statement they enter.
In this case, the CPU is idle as the users are thinking and typing their query.

\stitle{Lazy Evaluation} has emerged as a popular
method to bring traditional query optimization (planning and rewriting)
techniques to interactive systems~\cite{dask, Armbrust:2015:SSR:2723372.2742797}. However, this approach of delaying computation until results are explicitly requested introduces new burdens for users, particularly when they are debugging, since bugs are not revealed
until computation is triggered. Lazy evaluation can result in wasted
time where the system could be working toward a result while
the user is thinking or typing, but instead waits for the
user to trigger computation. As a result, interactive users often end up manually triggering computation, overriding the system
and limiting the amount of query optimization that could be done.

To address latency issues with the incremental, interactive construction of queries one statement at a time, \stitle{Asynchronous Evaluation} performs computation during user think time.

In an attempt to find a middle ground between these eager and lazy evaluation paradigms,
we developed \modin with an asynchronous computation
scheme that balances between the idle time of
the user and the available system resources.
Instead of making users wait for code to
execute after every statement,
\modin passes control back to the user immediately with a
pointer to the eventual computed dataframe.
Passing back control immediately is an improvement over an eager computation scheme
as users do not have to wait for their code to execute to 
continue developing their query.
Furthermore, asynchronous computation is able to improve over
lazy computation
by transparently computing the results immediately after execution,
rather than waiting for the user to request computation.
Although this comes at a cost of being able to find an optimal
query plan for the user's query,
we can leverage prior work in the database community
on incremental query optimization and update
the query plan as new statements are submitted.


\subsection{Immediate Feedback}

Providing immediate feedback is an important interactivity feature that would improve the
usability of dataframes. While it is important to aim for preserving the semantics of
the dataframe, it may be possible to get significantly better performance by sacrificing a bit of the semantics to
gain performance. 

In this section we discuss two examples of optimizations common in databases that
can be integrated into \modin to optimize for providing immediate feedback to the user, 
and the challenges therein: Prefix/Suffix Computation and Approximation.

\subsubsection{Prefix/Suffix Computation}
As illustrated in Section~\ref{sec:usecase}, building queries incrementally through trial-and-error typically involves printing some subset
of the rows and columns through the 
\code{head}, \code{tail}, or \code{print} operations.
The \code{head} and \code{tail} commands print the first
or last $k$ rows (5 by default), respectively. 
Printing a dataframe, also,
shows both the first and last $k$ rows. 
This is also another case where the user relies heavily on the
order of the data in their mental model. When a user prints
the first $k$ rows, they expect to see the first
$k$ rows ingested,
and they expect that the system will print the same
$k$ rows each time. The performance of displaying these first and last
$k$ rows is important as users rely on these operations to verify the correctness of their data and query and subsequently make decisions about what to do next.

While it is possible to use strategies similar to those that optimize for the \code{LIMIT} clause in RDBMSs \cite{kim2018optimally}, additional
consideration must be made for the \code{ORDER BY} clause to ensure that the order is the same every time. 
However, this approach limits interactivity, or the time to reach a partial result,
for increased query performance, or the time to reach the final result,
and increased accuracy as it will be always correct.
At the opposite end of the spectrum,
we can avoid the \code{ORDER BY} on every computation
by logically removing the first and last $k$ rows to be 
separate tables and performing computation on those results
to get much better interactivity, as the time to reach a partial result decreases significantly.
Clearly, this will reduce query performance, as it will take longer to reach the final result.
Additionally, this will also reduce the accuracy.
For instance, when calculating \code{GROUP BY} on the first or last $k$ rows
will return a result that is significantly different than 
calculating \code{GROUP BY} on the entire dataframe and taking the first or last $k$ rows.
Furthermore, \code{TRANSPOSE}s will be significantly harder with the first and last $k$ rows
logically separated.
Thus, this introduces an interesting line of work
as we can explore the trade-offs between
interactivity, query performance, and accuracy.
% \dorx{What is the research problem here? Rewrite the rest of the section to state the research challenge (e.g., what are the tradeoffs?) instead of proposing a solution.}
% To avoid computing the \code{ORDER BY}
% on every computation,
% the first and
% last $k$ rows can be logically removed as separate tables, 
% and perform computation on those
% tables to print the results faster. The remaining data can 
% be computed separately following the lazy evaluation paradigm,
% enabling query planning on the remaining data. 
% In the case
% that the query modifies the order of the data, the
% printed rows will have to wait until the \code{ORDER BY} to 
% ensure that the user sees the data in the order they have
% specified. In these cases, there is a limit to the amount of
% query planning that can be applied because the print forces
% the \code{ORDER BY}. 

\subsubsection{Approximation}
Approximate computation is another way to provide users with faster query responses to facilitate interactive workflows. In some cases, the user may be content with an approximation
rather than waiting for the full result. Existing RDBMS approximation
techniques for online aggregation~\cite{Fekete2018,raman2002partial,lang2014partial,viglas2002rate,rahman2017ve},
barchart, histogram, scatterplot, and map plot generation~\cite{kim2015rapid,ding2016sample+,park2016visualization},
histogram matching~\cite{macke2018adaptive}, stratified sampling~\cite{agarwal2013blinkdb}, and
error estimation~\cite{zeng2014analytical,park2018verdictdb} are directly applicable
toward accelerating individual dataframe operations. 
However, dataframe semantics
offer some unique opportunities for further speedups via approximation.

\william{These subsubsections feel like they are just listing a lot of cool things you can do with dataframes from AQP but do not give a research problem. There is also a lot of prefix/suffix computation stuff listed here. The query rewriting section does a good job of giving the research problem.}

\stitle{Cumulative Aggregates.}
The ordering of rows in a dataframe can create bottlenecks when the
computation required to display the bottom $k$ rows depends on the
result of the computation for all previous rows. For example,
a cumulative sum or cumulative max must be done in order from the
top of the dataframe to the bottom, causing significant latency
before the bottom $k$ rows can be displayed.

While it is well known that an aggregate like \texttt{MAX}
cannot be approximated~\cite{mozafari2015handbook},
the user may be satisfied to see approximations of cumulative sums or means
in the bottom $k$ rows that
either update progressively as more data is processed, or satisfy a
probabilistic accuracy requirement.

\stitle{Estimating Counts on Filtered Dataframes.}
Dataframe libraries
like \pandas typically show summary statistics like \texttt{COUNT}
after each operation.
If a user applies a filter on a dataframe, without prior knowledge
it is impossible to know the exact number of rows passing the filter 
until the full computation has completed. One strategy is to
automatically identify such cases and adaptively estimate the
selectivity of the filter on-the-fly, again progressively updating the estimate as more tuples passes through the filter.

\stitle{Approximating Expensive Filters.}
For a filter that is both selective and expensive
(e.g., one that performs classification on
a dataframe where one of the columns contains large objects), there might not be any row in the top or bottom
$k$ that satisfies the filter. As such, determining the top and bottom
$k$ rows that pass the filter can itself be a high-latency
operation, even without a complete filter application.
In this case, dataframes present a perfect use case for
{\em exploiting correlations}~\cite{joglekar2015exploiting}
between the filtering attribute
and the other attributes in order to quickly approximate
the top and bottom $k$ rows that might pass the filter and
quickly display them to the user, refining as
additional filter evaluations are performed.


\stitle{Approximation and Asynchrony.}
When used in conjunction with \modin's
inherent asynchronous background execution,
exact results may be scheduled in the background for
later verification (as in~\cite{moritz2017trust}).
This may result in many exact queries getting queued in the
background as the user rapidly issues statements and achieves
immediate approximate feedback. To increase throughput of
these statements that build up in the execution queue,
we can apply {\em multiquery optimization techniques}
and to take advantage of opportunities for shared computation,
to be described in detail in Section~\ref{sec:mqo}.


\subsection{Multiquery Optimization} \label{sec:mqo}
We envision that \modin will prioritize interactivity, returning
control to the user as quickly as possible by displaying
preview (head/tail) or
approximate results and defer calculation of full or exact results to background computation using techniques from Section\label{sec:singlestatement}.
As such, many operations may be queued for execution at once. These statements may
operate over similar or even identical subsets of data. 
To exploit this workload, \modin can make use of multiquery optimization (MQO) techniques~\cite{sellis1988multiple}
to allow operations that share significant amounts of data to run underneath the
same scans or seeks, thereby reducing the overhead required to funnel data up
through the memory hierarchy. However, MQO presents a significant challenge when employed
in an interactive environment, 
where the results of the operation is displayed in-situ the coding/input environment, 
such as a Jupyter notebook cell. In this case, the optimizer will have to balance
between maximizing operation throughput and
minimizing the latency required to compute output of the important ``to-be-displayed'' operations.

\subsubsection{Query Rewriting}
Current approaches to planning queries for dataframes are either
(i) strictly imperative and do not perform any 
query planning~\cite{mckinney2010data, R, dask}
or (ii) declarative but do not support operations
beyond the traditional relational table operations~\cite{Armbrust:2015:SSR:2723372.2742797}.
As an example of query rewriting, consider the \code{TRANSPOSE} operation, which in some cases can be avoided using clever rewrite rules. For example, the query \code{TRANSPOSE}, \code{SORT}, \code{TRANSPOSE} to reorder columns can be 
rewritten as a \code{MAP} and \code{RENAME}. 

\eat{Because it is not feasible
to physically do the \code{TRANSPOSE} in most RDBMSs, the rewrite
rules for these systems will have to work around this architectural limitation.
Developing rewrite rules for relational systems
in the context of the \code{TRANSPOSE} operator will produce some
interesting research on how to support dataframe operators in
relational systems.}
The challenge of supporting declarative query processing across a wide range of dataframe operators is that
the cost of extending rewrite rules beyond relational operations, 
to support spreadsheet and linear algebra operations, requires a significant development effort.
As a result, dataframe users either have to sacrifice performance, 
operate on a feasible subset of their data, 
or manually construct and profile various possible rewrite to determine the optimal approach to execute the query~\cite{optimizing-pandas}. 
When creating rewrite rules for dataframes, we have to consider (i) how to group the dataframe operations into queries and (ii) when to rewrite the queries.
Manual query optimization on the part of the developer can be a daunting task due to the large number of possible ways to perform an operation~\cite{wu2019diel}.
In addition to the numerous ways of writing any given query at the API level,
the problem is further exacerbated by the fact that
there is a large and diverse set of operations beyond relational operators to consider when creating rewrite rules. \eat{An important area of future
work in \modin will be in defining rewrite rules to efficiently
handle cases that traditional systems cannot.}


In addition to the large query space to cover with rewrite rules,
we still have to consider when the query rewriting will occur.
Traditional databases operate in a declarative environment.
As a result, it is obvious that the query rewriting occurs 
once the query is submitted.
However, there is no clear cut line to even differentiate separate queries for dataframes because most existing dataframe frameworks are imperative and execute operations eagerly.

\subsubsection{Materialization and Reuse}
\smacke{JMH: the distinguishing factor here vs materialization in a traditional
RDBMS setting is that we might reuse an intermediate result an unknown number of
multiple times, and we can do fancy things like predict what we think the user
will use again.}
The incremental and exploratory nature of dataframe query construction 
leads to nonlinear code paths 
where users revisit the same intermediate results repeatedly 
to refine the query results. 
% Recomputing the same intermediate result repeatedly
% is time-consuming and wasteful. 
% Ignoring re-computation can also be costly for operations such as data loading, which often does not need to be re-executed.
We envision the \modin optimizer can automatically materialize and reuse intermediate results
to significantly reduce execution time by removing redundant computation across statements.

% To concretize the discussions of the research challenges
% associated with this optimization, consider the following example.
% \begin{lstlisting}
% r1 = df.groupby(...).count().query("c1 > 0")
% r2 = df.groupby(...).count().query("c2 <= 0")
% \end{lstlisting}
% Intermediate results refer to the output of any combination of operations.
% In this example, the intermediate result accessed by both \code{r1} and \code{r2} 
% is \code{df.groupby(...).count()},
% which is computed twice when executing the statement verbatim.
% We could eliminate the redundant computation 
% by identifying this common subexpression in both statements
% and substitute it with a reference to the intermediate results.
% This is a common technique in compilers known as common subexpression elimination\cite{cocke1970global}. Applying these techniques to dataframes is non-trivial due to the tradeoff between storage cost and compute savings.

The objective of this optimization problem is to trade the
\textit{materialization overhead}, including both the storage and the time to persist the results,
for the \textit{reduced execution time} due to reuse. 
There are two components to this optimization.
First, we need to identify reusable intermediate results, 
which can be accomplished using standard program analysis.
Then, we need to decide whether an intermediate result should be stored and reused,
and the optimizer needs to utilize storage in a way that maximizes 
saved compute---small 
objects that are time-consuming to compute and reused frequently 
should be prioritized over large objects that are fast to compute.
% Storage can refer to either memory or disk, 
% depending on whether reuse takes place within a single session 
% or across multiple sessions.
A storage budget is often imposed, especially in the single-session case, making the problem NP-Hard (by reduction from the Knapsack problem).
Effective solutions need to adapt to variable reuse patterns.



==> interactivity_agp-5-22-bkp.tex <==
%!TEX root = modin-vision.tex

\section{User Model Challenges}\label{sec:interactivity}
% \todo{Reorient sections}
% \todo{(1) incremental queries}
% \todo{(2) Debugging - cite something}
\rebuttal{
Unlike in SQL where queries are submitted {\em all-or-nothing}, 
dataframe users construct queries 
in an incremental, iterative, 
and interactive fashion.
Queries are submitted as a series of subqueries, 
a few operators at a time, 
in trial-and-error-based \textit{sessions}. 
Users rely on immediate feedback 
to debug and rapidly iterate on subqueries 
and frequently revisit subquery results 
for experimentation and composition 
during exploration. 
This interactive session-based 
programming model for dataframes 
creates novel challenges for overall system performance
and imposes additional constraints on query optimization. 
For example, operator reordering is often not beneficial
when the results are materialized for viewing after every step (subquery).
At the same time, dataframe query 
development sessions are bursty, 
with ample think time between issuance of subqueries, 
and tolerant of incomplete results as feedback---as long
as the original goals of experimentation and debugging are met, 
offering new opportunities for query optimization.
In this section, we discuss new
challenges and opportunities in query optimization 
arising from the interactive and incremental
trial-and-error query construction of a typical
dataframe user.
}

% (Kill after reorg) Unique characteristics of DF programming:
% \begin{itemize}
%     \item opportunity: People incrementally construct queries: 6.2.1: ``Incremental query construction with composable subexpressions''
%     \item latency requirement: they rerun subqueries often in an ad-hoc trial and error fashion: 6.2.2:``Frequent ad-hoc experimentation''
%     \item latency requirement(can use ``sloppiness'' to support this particular use case): they inspect results primarily for debugging: 6.1.2: ``Previewing intermediate results for debugging''
%     \item opportunity: they ``think'' between steps : 6.1.1: ``Leveraging user think-time.''
% \end{itemize}

% Old text
% Here we outline our vision on the challenges in supporting
% and optimizing for user behaviors in an interactive session-based setting. These challenges are based
% on our experience working with users and our observation of
% how users interact with systems like \pandas and \modin. We first describe usage requirements in the interactive setting and describe ways to provide users with {\em immediate feedback} for a given dataframe query. Given these user requirements, we then describe how dataframe systems can leverage the iterative nature of how users constructs dataframe queries to further speed up query execution. 

% ------, users often
% wish to quickly examine the results
% of each intermediate statement
% along the way towards accomplishing
% a larger query, we aim 
% Second, over the course of
% a session, there are often
% many different statements and queries
% that are assembled, by building on
% top of each other,
% so we target {\em sharing and reuse}
% across the session.

% In particular, there are two classes of optimization opportunities and usage requirements in the interactive setting based on 1) iterative nature of how users constructs dataframe queries, and 2) their need for interactivity for debugging purposes.

% This section focuses on the challenges for optimizing dataframe usage in an interactive session-based scenario, as these optimizations differ greatly from dataframe operations submitted through batch jobs or scripts.


% \subsection{Inefficiently written queries}\label{sec:prefix-suffix-computation}

% At the opposite end of the spectrum,
% we can avoid the \code{ORDER BY} on every computation
% by logically removing the first and last $k$ rows to be
% separate tables and performing computation on those results
% to get much better interactivity, as the time to reach a partial result
% decreases significantly.
% Clearly, this will reduce query performance, as it will take longer to
% reach the final result.
% Additionally, this will also reduce the accuracy.
% For instance, when calculating \code{GROUP BY} on the first or last $k$
% rows
% will return a result that is significantly different than
% calculating \code{GROUP BY} on the entire dataframe and taking the first
% or last $k$ rows.
% Furthermore, \code{TRANSPOSE}s will be significantly harder with the
% first and last $k$ rows
% logically separated.
% Thus, this introduces an interesting line of work
% as we can explore the trade-offs between
% interactivity, query performance, and accuracy.

% \moved{
% As we discussed in the previous subsection,
% this is a setting where ordering,
% in conjunction with prefix computation
% can actually help us achieve lower 
% latencies---a reasonable 
% estimate of the prefix of the output
% (which usually corresponds 
% to some prefix of the input dataframe) 
% would suffice.
% For example, we don't need to 
% produce an estimate of all of the groups,
% in a \code{GROUP BY}, 
% just the first $k$ that appear in the input.
% }

% \moved{
% Finally, when used in conjunction with opportunistic
% evaluation, exact results may be scheduled in the background,
% and displayed explicitly to the user (e.g., as a pop-up) for
% later verification, as in Moritz et al.~\cite{moritz2017trust}, where
% they found that this approach of showing users an inexact result,
% while allowing them to proceed with their analysis,
% and letting them know when the exact results are ready,
% is an effective approach to optimization.
% However, this may result in many exact queries getting queued in the
% background as the user rapidly issues statements and achieves
% immediate approximate feedback. To increase throughput of
% these statements that build up in the execution queue,
% we can apply {\em multiquery optimization techniques}
% and to take advantage of opportunities for shared computation,
% to be described in detail in Section~\ref{sec:mqo}.
% }

% \subsection{Interactive feedback for query composition}\label{sec:immediate-feedback}
\subsection{Interactive Feedback and Control}\label{sec:immediate-feedback}
\rebuttal{
Dataframes are typically used in 
exploratory workloads, 
where interactive response times 
are crucial to providing a fluid user experience. 
Past studies have shown that latency 
in response times of greater than 500ms can lead
to fewer hypotheses explored and
insights generated during data exploration~\cite{liu2014effects}. 
As another example, 
for data preparation---often performed on dataframes---users 
often rely on system feedback 
to guide and decide what operations 
to determine their next steps~\cite{Heer2015}.
This feedback usually comes in the form
of a display output by the dataframe system
that contains a prefix or suffix of rows and columns,
as in Figure~\ref{fig:example}.
The need for frequent materialization 
of intermediate subquery results
to provide feedback to the user
% for feedback \agp{what is feedback here? is it for deciding what to do next? for debugging? we should clarify globally} 
makes it particularly 
difficult to satisfy the 500ms query 
latency requirement for interactivity.  
Fortunately, we can leverage two
user behavior characteristics to improve
interactivity:
that users spend time thinking between 
steps, and that the inspected intermediate 
results are typically restricted 
to a prefix/suffix of rows/columns---which is sufficient 
for debugging
and validation.
We discuss these ideas next.
}
%, motivating past research on interactive visual specification systems for data cleaning ~\cite{Kandel2011,Raman2001}. 
%One unique challenge in providing interactivity for dataframes is that because dataframes are designed to be general-purpose, supporting not just data cleaning but a variety of data science tasks, the optimizations needs to be designed in a way that ensure that the assumptions and results are applicable to the wider use case. \agp{arguably you can do fairly ``general-purpose'' things in an RDBMS. Weak argument.}


% \rebuttal{
% In this section,
% we describe two classes of user behavior challenges:
% (1) Subquery materialization and think time
% % \agp{here and below: 
% % this is not a characteristic. You want to capture the insight here
% % which is that there users inspect subquery results, and 
% % think between steps.}
% and (2) prefix and suffix inspection.
% % \agp{While this is a characteristic, this overlaps with the previous---this 
% % one should be more about how approximation/prefixes are 
% % OK because it is about debugging/sensemaking/confirmation. 
% % }
% As we will see, preserving the structural and order information to ensure that users have a sufficiently accurate display of the resulting dataframe is a
% recurring challenge.
% % \agp{operationalize is a weird usage -- reword prev sentence.}
% % A variety of different strategies can be employed depending on what is 
% % appropriate for the use case data requirements.
% % \agp{previous sentence is noise, unless there is a deeper meaning which I can't
% % fully follow}
% }

% data validation ---- structure.

% In an interactive workflow for data cleaning or exploratory data analysis,
% users are often waiting for results after they are computed.
% During these workflows, 
% many incremental query sub-expressions are constructed
% and executed over the course of a session.


% Providing immediate feedback
% to the user during data exploration
% would greatly improve the usability of dataframe systems.



% \subsubsection{Opportunistic Evaluation}\label{sec:opportunistic-evaluation}
% \stitle{Query Optimization in interactive environments.}
\rebuttal{
\subsubsection{Subquery inspection and think time}
\label{sec:opportunistic-evaluation}
Present-day dataframe systems 
are targeted toward ensuring users
can inspect intermediate results, so they often operate
in an {\em eager} mode where every statement is evaluated as
soon as it is issued.
Thus, program control is not returned to the user
until the statement has been completely evaluated,
forcing the user to be idle during the computation.
However, there are many cases where users do not inspect the
results, or where results are discarded. These
statements can potentially be deferred for computation later.
In fact, users can spend a significant amount of time
between analysis steps, allowing us to perform computation
then.
While interactive latency is important 
to support immediate feedback, recent 
empirical studies have also shown 
that optimizations can be relaxed to account 
for user's long think time 
between operations in exploratory 
analysis~\cite{Battle2019}. 
We describe a novel \emph{opportunistic} query 
evaluation paradigm suitable for optimizing dataframes 
in an interactive setting.
}

\moved{
There are two standard modes of query evaluation
in data processing systems:
lazy and eager.
In the eager paradigm, adopted
by current dataframe systems like \pandas,
program control is not returned to the user
until the statement has been completely evaluated,
forcing the user to be idle during the computation.
Query optimization is not possible in an eager
system because each operator within the statement
must be completely evaluated 
\rebuttal{in the order that the statement is written
by the user}.
\devin{
For example,
suppose there are two commutative operations \texttt{op1}, and \texttt{op2}. Suppose the user submits the subquery \texttt{x = df.op1()}
followed by \texttt{y = x.op2()}. 
In eager evaluation, \code{x} will be fully materialized before
execution begins on \code{y}, even if \code{x} is never used again. 
In lazy evaluation, execution will be deferred until
explicitly requested, so the
expression that creates \code{y}
could be optimized to run \texttt{df.op2().op1()}.
}
% \jmh{See my comment above. Providing specific examples
% as I did in the comment should clarify what you want to get across
% in terms of limiting optimization opportunities.}
Thus, a significant amount of computation
is wasted for statements
that are never used or inspected,
and users are either rewarded or punished
based on the efficiency of a query as it is written.

On the other hand, in the lazy paradigm
% which has recently emerged as a popular
% alternative in some
% \rebuttal{dataframe-like} systems~\cite{dask, Armbrust:2015:SSR:2723372.2742797},
control is returned to the user immediately,
and the system defers the computation until the user
requests the result.
By scheduling computation later,
the system can wait for larger query sub-expressions to be assembled,
leading to greater opportunities for optimization,
as is done in systems such as
Spark~\cite{Armbrust:2015:SSR:2723372.2742797}.
For example, if the user composes a cross-product
followed by a filter, this filter
can be rewritten to be performed first.
% \jmh{be clear what you mean by a ``step'' - is it a part of an dotted chain expression, or a request for output to be computed (Shift-Return) or what...}
The downside of lazy evaluation is that
computation only begins when the user
requests the result of a query.
This introduces new burdens for users,
particularly for debugging, since bugs are not revealed
until computation is triggered.
Moreover, during the
time a user is thinking or typing, the system
could be working toward a result---however, in
the lazy paradigm, the system is idle during think time,
leading to lost computation.
For smaller datasets or simple queries this can
potentially lead to a longer overall runtime if there are
periods of think time
that exceed the runtime of the statements
in the query.
\techreport{In fact, most users of such systems
 end up requesting the results after each operation,
 essentially defaulting to the eager mode.}


Instead, we propose a middle ground that aims
to preserve the benefits of both lazy and eager evaluation;
a mode we call {\em opportunistic evaluation}, that
we have started to implement in \modin,
which makes the best use of 
system resources during user think time.
Like lazy evaluation, opportunistic evaluation
does not require the user to wait after each statement.
Instead, the system opportunistically
starts execution, while passing control back to users
with a pointer to the eventually computed dataframe,
which is asynchronously computed in the background.
In this manner, opportunistic evaluation
makes use of system resources to compute
results in the background as users
are composing the next step of the query.
Like eager evaluation, opportunistic evaluation
does not wait for users to complete the entire
query to begin evaluation.
However, when a user requests to view a certain
output, opportunistic evaluation prioritizes
producing that output over all else.
Opportunistic evaluation allows queries to be rewritten
as new statements are submitted to get to the requested
answer as fast as possible, taking into account
the statements that are partially computed.
There are also new opportunities within opportunistic evaluation
to do speculative query execution, 
where during 
idle time the system can start
executing statements that commonly follow previous statements.
Opportunistic evaluation also leads to new
challenges in sharing and reuse
across many query fragments whose computation
has been scheduled in the background,
which we will discuss in Section~\ref{sec:trialanderror}.
}

\rebuttal{
\subsubsection{Prefix and suffix inspection.}
\rebuttal{
The most common form of feedback provided by dataframe systems is the tabular
view of the dataframe, as shown in Figure~\ref{fig:example}. The tabular view
serves as a form of visualization that not only allows users to inspect
individual data values, but also convey the structural information associated
with the dataframe. Structural information, especially as it relates to order,
is important for validating the results of queries that manipulate and
reshapes the dataframe or its index. 
This tabular visualization typically contains a partial view of the dataframe,
displaying the first and last few lines of the dataframe. During dataframe
query construction, table visualizations are frequently requested via the
\code{head}, \code{tail}, or other print commands, as we saw in
Section~\ref{sec:usecase}.
}
% \moved{\agp{There is a lot of repetition in the following lines 
% w.r.t the previous.
% The partial view stuff is repeated. The order is repeated. Once is plenty.}
% % As we saw in Section~\ref{sec:usecase}, 
% % building queries incrementally
% % through trial-and-error
% % typically involves printing
% % the first or last few rows of the dataframe,
% % via the \code{head}, \code{tail},
% % or other print commands.
% The \code{head} and \code{tail} commands,
% in \pandas, print the first
% or last $k$ rows (5 by default), respectively,
% while printing a dataframe displays
% both the first and last $k$ rows.
% When building queries through trial-and-error, 
% the user
% relies heavily on the order of the displayed data
% in judging the correctness
% of the intermediate
% query sub-expression,
% and deciding what to do next.
% When the user employs these printing commands,
% they expect the same $k$ rows to be displayed,
% in order.
% }

One way to give the
users immediate feedback
is to return
the output to the user as soon as these $k$
rows are assembled, computing the rest of the output
in the background using opportunistic evaluation.
This is reminiscent of techniques that
optimize for early
results~\cite{viglas2003maximizing,viglas2002rate}
for \code{LIMIT} queries~\cite{kim2018optimally},
or 
for representative tuple identification~\cite{singh2012skimmer},
but a key difference in dataframes is that order
must be preserved, and there are many more blocking operators.
% \agp{I think we should "amp up" the differences.
% Omit special care etc. Say a KEY difference is that the order
% must be preserved and that there are many more blocking operators
% } 
Therefore, techniques that try to find
samples anywhere in the data that match query predicates
as in Kim et al.~\cite{kim2018optimally},
will not apply.
One starting point would be to design or select physical operator implementations that not just prioritize high output
rate~\cite{viglas2002rate},
but also preserve order, thereby ensuring
that the first $k$ rows will be produced as quickly as possible.
As an example, if only the first $k$ rows
of an ordered join were to be computed,
a nested loop join, with the result displayed
after $k$ rows are computed, might work well.
Returning the first $k$ rows following a
\code{TRANSPOSE}, especially when using columnar storage,
can be fairly efficient as well.

However, certain blocking operators will cause problems.
For example, it is hard to produce the first $k$ tuples
of a \code{GROUP BY} or \code{SORT}
without examining the entire data first. 
\techreport{(Indeed,
for small enough $k$, sorting may be faster
than $O(n \log{n})$, but still requires an $O(n)$ sequential scan.)}
Optimizers in RDBMSs draw upon techniques such as predicate pushdown to reduce the amount of data processed for a query. 
Unfortunately, due to the order requirement in dataframes, predicate pushdown is often not directly applicable to prefix/suffix computation. 
\code{SORT} is an obvious example where the top $k$ rows cannot be narrowed down a priori; a full scan is inevitable also for \code{GROUPBY} on non-clustered columns. 
Since the top and bottom $k$ rows are often the only results inspected for a dataframe query, maintaining additional intermediate results and data structures for these regions \`{a} la incremental view maintenance can significantly speed up query processing without exorbitant storage overhead. What these data structures are and how to maintenance them in the ordered setting present interesting research opportunities.
We may also be able to exploit approximation
to produce
the prefix/suffix early for these blocking operators, discussed next.
% For example, a \code{GROUP BY} might correctly produce
% an approximate estimate
% of the first $k$ groups without
% filling in the aggregates, and a \code{SORT}
% might be able to produce an approximation
% of the top-$k$ after reading a large
% enough random sample\techreport{---however
% guarantees on correctness may be minimal}.
% \agp{See if we can amp up the novelty for group by and sort -- they
% are pretty traditional ops}
% \dorx{How's the new blurb?} \devin{it is great}
}

\moved{
\rebuttal{\agp{This entire subsection seems very generic.
What is new here? One thing that is new is the interaction
with order, allowing us to prioritize samples
targeted towards order. Others?}
\devin{Propose TR next paragraph}
% \subsubsection{Approximate execution across different dataframe operations.}\label{sec:approximate-execution}
% \dorx{Merge with the previous section.}
% is essential to the user's analytical workflow,
Another way to provide immediate feedback is to take advantage of approximate query processing (AQP) techniques to quickly display inexact
results at significantly reduced latencies. AQP is suitable for interactive query composition since users often do not require exact results when simply inspecting results for debugging or exploratory purposes.}
Traditional AQP has been applied to accelerate
the generation of specific aggregates, e.g.,
\code{SUM} or \code{AVG}, and bound
their estimates with confidence
intervals~\cite{zeng2014analytical,park2018verdictdb}.
AQP is performed either offline, or online,
where the former involves maintenance of materialized
stratified samples, with some
sample selection happening
online~\cite{ding2016sample+,agarwal2013blinkdb,park2018verdictdb},
and the latter involves sampling on-the-fly with no
pre-materialization decisions.
Due to the highly ad-hoc nature of dataframe processing,
we expect online sampling to be more effective.
Specifically, online aggregation-type schemes~\cite{hellerstein1997online}
can be used to produce
progressively improving
aggregates to the
user~\cite{hellerstein1997online,rahman2017ve,Fekete2018}---and
these schemes will work well in the context
of opportunistic evaluation, as discussed in
Section~\ref{sec:opportunistic-evaluation},
but we expect the dataframe model and algebra to introduce
new challenges.
Recent work has also introduced
the notion of guarantees
across collections of aggregates,
often optimizing for user tasks or
perceptual
guarantees \rebuttal{for visualizations}~\cite{kim2015rapid,park2016visualization,macke2018adaptive,alabi2016pfunk},
e.g., ensuring that the
ordering of the aggregates
matches the correct ordering,
even if the values of the aggregates are
inexact,
and these techniques
may be a good fit to the dataframe setting.
}

\techreport{    
\moved{
% \dorx{Move the rest of this section to TR?}
While it is well known that some aggregates like \code{MAX}
cannot be approximated~\cite{mozafari2015handbook},
even blocking operators such as \code{SORT} can return
early approximate results, using results
from the 1990s~\cite{raman1999online}.
There may be additional opportunities for approximation
if the user simply wants to inspect the approximate
structure of the result for debugging purposes,
especially in conjunction with prefix/suffix computation.
For example, we can provide the
overall structure of the output of
a pivot table computation
(displaying the row-wise groups and column headers),
without actually filling
in any of the aggregate values, and doing so
progressively.
Similar ideas of adding ``placeholder'' values
for in-progress tuples have been proposed in
streaming~\cite{raman2002partial}, web-database
hybrid~\cite{goldman2000wsq},
and crowdsourcing~\cite{parameswaran2012deco} contexts,
but not, as far as we can tell, for a group-by aggregation setting.
This idea could also be applied, 
for example, to \code{TRANSPOSE},
where the structure of the 
output dataframe is prepared first, with
the values filled in progressively.
}
% \devin{One paragraph tech-reported here}
\moved{
Other notions of approximation may also be valuable,
e.g., the incomplete/phantom notions in Lang et al.~\cite{lang2014partial},
wherein the result may contain additional rows
not present in the dataframe query result,
or rows that should be present, but are absent.
This could be valuable, for example, for expensive filters.

In fact, we could also exploit correlations~\cite{joglekar2015exploiting}
between the filtering attribute
and the other attributes in order to quickly approximate
the rows that might pass the filter and
quickly display them to the user, refining as
additional filter evaluations are performed.
}
}

\input{incremetal_query_construction}


==> intro-bkp-5-24.tex <==
%!TEX root = modin-vision.tex

\section{Introduction}


For all of their commercial successes, 
relational databases have notable limitations 
when it comes to 
``quick-and-dirty'' exploratory data analysis 
(EDA)~\cite{tukey1977exploratory}. Data needs to be 
defined schema-first before it can be 
examined, 
data that is not well-structured is 
difficult to query, 
and any query beyond
\code{SELECT *}
requires an intimate 
familiarity with the schema, which is particularly problematic for wide tables. 
% % Begin additional EDA comments
% Exploratory Data Analysis (EDA) often involves examining and querying un-
% or semi-structured data where types may be dynamically inferred or
% specified, making it difficult and sometimes impossible to define the schema
% upfront.
% % End additional EDA comments
For more complex analyses, the 
declarative nature of SQL makes it
awkward to develop and debug queries in a piecewise, modular
fashion, conflicting with best practices for software development.
\rebuttal{In part, thanks to these limitations, SQL is
often not the tool of choice for data exploration. 
As an alternative,}
programming languages such as Python and R support 
the so-called {\em data\-frame}
abstraction. Dataframes provide a functional interface 
that is more tolerant
of unknown data structure and well-suited 
to developer and data scientist workflows, 
including REPL-style imperative interfaces 
and data science notebooks~\cite{perez2015project}.

Dataframes have 
several characteristics 
that make them an appealing 
choice for data exploration:

\squishlist
\item a more
intuitive data model that 
embraces an implicit ordering on both rows
and columns and treats them symmetrically;
\item a query 
language that bridges a variety of data 
analysis modalities including 
relational (e.g., filter, join), 
linear algebra (e.g., transpose), 
and spreadsheet-like (e.g., pivot) operators; 
\item an incrementally composable query 
syntax that encourages easy and rapid validation
of simple expressions, 
and their iterative refinement and composition
into complex queries; and 
\item native embedding in a 
host language such as Python 
with familiar imperative semantics.
\squishend

\noindent 
% These characteristics and others have helped
% dataframes become the de-facto
% standard for EDA. \jmh{citation? can we find one
% that says they're more popular than SQL in this regard} 
% In particular, the dataframe abstraction provided
% by 
Characteristics such as these
have helped dataframes become
incredibly popular for EDA; 
for instance, 
the dataframe abstraction provided by \pandas 
within Python (\url{pandas.pydata.org}), 
has, as of 2020, been downloaded
over 300 million times, served as a dependency for
over 222,000 repositories in GitHub, 
and starred on GitHub more 25,000 times.
Python's own popularity
has been 
attributed to the success of \pandas 
for data exploration and data science~\cite{python-growing-quickly,python-growth-blamed}.
Due to its ubiquity, we focus on \pandas for concreteness.

\Pandas 
has been developed from the ground up
\rebuttal{via open-source contributions
from dozens of contributors,
each providing operators and
their implementations to the DataFrame API}
to satisfy immediate or ad-hoc needs, 
spanning capabilities
that mimic
relational algebra, 
linear algebra, and 
spreadsheet formula computation.
To date, 
the \pandas DataFrame API has ballooned to 
over 200 distinct operators~\cite{pandas-api}.
R, which is 
both more mature and more carefully curated
than \pandas, has only 70 operators---but this
is still far more than, say, relational
and linear algebra combined~\cite{R-dataframe-api}.

While this rich API is sometimes cited as a 
reason for \pandas' attractiveness,
the set of operators has significant redundancies,
often with different performance implications.
These redundancies place a considerable burden 
on users to select the optimal way of expressing their goal.
For example, one blog post cites five different ways to express
the same goal, with performance varying from 0.3ms to 600ms 
(a 1700$\times$ increase)~\cite{optimizing-pandas};
meanwhile, the \pandas documentation itself offers multiple recommendations
for how to enhance performance~\cite{enhancing-performance}.
As a result, many users eschew the bulk of the API, 
relying only on a small
subset of operators~\cite{minimally-sufficient}. 
The complexity of the API and evaluation semantics
also make it difficult to apply 
traditional query optimization techniques.
Indeed, each operator within a \pandas ``query plan'' 
is executed completely before subsequent operators are executed,
with limited optimization, and 
no reordering of operators or pipelining 
(unless explicitly done so by the user using \code{.pipe}). 
Moreover, the performance of the \code{pandas.DataFrame} API
breaks down when processing 
even moderate volumes
of data that do not fit in memory, as we will see 
subsequently---this is especially problematic
due to \pandas' eager evaluation semantics, wherein
intermediate data items often surpass main memory limits
and must be paged to disk. 


\rebuttal{
To address \pandas' scalability challenges,
we developed \modin (\url{github.com/modin-project/modin}), 
our first attempt at a scalable dataframe system,
which employs simple optimization techniques to 
enable unmodified \pandas code 
to run more efficiently on large dataframes.
\modin is already used by over 60 downstream projects, and
has over 250 forks and 4,800 stars on GitHub
in its first 20 months, indicating
the impact and need for such systems.
\modin rewrites \pandas API calls 
into a sequence
of operators in a new, compact 
dataframe algebra.
\modin then leverages simple 
parallelization and a new physical 
representation 
to speed up the 
execution of these operators,
by up to {\bf 30$\times$} in certain
cases, and is able to run to completion
on datasets {\bf 25$\times$} larger 
than \pandas (which crashes instead) 
in others.
}

\rebuttal{However, \modin only represents
our first step towards making dataframe systems
scalable and efficient; 
we have an entire 
research agenda full of novel research challenges 
ahead of us. 
% Inspired by our experiences
% with \modin, we propose a new
% research agenda centered around the development
% of scalable dataframe systems.
% \modin simply represents our first step
% for this agenda---many interesting outstanding
% research challenges remain in making
% dataframe systems scalable and efficient. 
In this paper, 
we begin with an example dataframe workflow
capturing typical 
dataframe capabilities and user behaviors.
We then 
describe our experiences with \modin 
(Section~\ref{sec:modin}).
We use \modin to ground our discussion of
the research challenges.
We {\bf \em (i)
% define a research agenda around 
% formalizing
provide a candidate formalism for
dataframes} and enumerate their capabilities with a new algebra
(Section~\ref{sec:definitions}).
We then outline research challenges and 
opportunities
 {\bf \em to build on our formalism
and make dataframe systems more scalable,}
by optimizing 
and accounting
for 
{\bf \em (ii) the unique characteristics 
of the new data model and algebra} (Section~\ref{sec:datamodel}),
as well as {\bf \em (iii)
the unique ways in which dataframes are used 
in practice for data exploration} (Section~\ref{sec:interactivity}).
We draw on tools
and techniques from the database research literature throughout
and discuss how they might be adapted 
to meet novel dataframe needs.
}



\rebuttal{While developing \modin, our original intent
was to adapt standard relational database techniques
to help make dataframes scalable.
However, while the principles (such as parallelism)
do apply, their instantiation in the form of specific 
techniques often differ,
thanks to the differences between
the data models and algebra of dataframes and relations.
Therefore, a more principled
foundation for dataframes is needed,
comprising a formal data model
and an elegant, expressive, and compact algebra.
We describe our first attempt
at such a formalization in Section~\ref{sec:definitions}.
Then, armed with our data model
and algebra,
we outline a number of outstanding
research challenges organized around 
the unique characteristics of
dataframes and the unique ways in which they are processed.
}

\rebuttal{In Section~\ref{sec:datamodel},
we describe how the dataframe data model and algebra
result in new scalability challenges.
Unlike relations, dataframes
have a flexible schema and are lazily typed,
requiring careful maintenance of metadata,
and avoiding the overhead of type inference as
far as possible.
Moreover, dataframes treat rows and columns
as equivalent, and metadata (e.g., column or row labels) and data 
as equivalent, requiring flexible ways
to keep track of metadata and orientation,
placing new metadata awareness
requirements on dataframe query planners in
order to avoid physically transposing data where possible.
Moreover, dataframes are ordered---and common implementations
often enforce a strict coupling between logical and physical
layout; we identify several opportunities to deal
with order in a more light-weight, decoupled, and lazy fashion. 
Finally, the new space of operators---encompassing
relational, linear algebra, and spreadsheet operators---introduces
new challenges in query processing and optimization.
}

\rebuttal{In Section~\ref{sec:interactivity},
we describe new challenges and opportunities
that emerge from how dataframes are used
for data exploration.
Specifically, unlike SQL which 
offers an all-or-nothing query modality, 
dataframe
queries are often 
constructed one operator
at a time, with ample think-time between query fragments.
This makes it more challenging to perform query optimization
wherein operators can be reordered for higher overall efficiency.
At the same time, the additional thinking time between steps
can be exploited to do background processing. 
Users often inspect intermediate dataframe results of query fragments, usually
for debugging, which requires a costly materialization
after each step of query processing.
However, users are only shown an ordered 
prefix or suffix of this intermediate
dataframe as part of the output, allowing
us to prioritize the execution to return
this portion quickly and defer the execution
of the rest. 
Finally, users often revisit old processing steps in 
an ad-hoc process of trial-and-error data exploration.
We discuss opportunities to minimize redundant computation
for operations completed previously.
}




\vspace{5pt}
\noindent 
In describing the aforementioned challenges, we focus on the \pandas dataframe system~\cite{pandas-api} 
for concreteness. 
\Pandas is much more popular than other dataframe 
implementations,
and is therefore well worth our effort to study and optimize.
We discuss other dataframe
implementations and related work in Section~\ref{sec:ext}.
\rebuttal{Many details about \modin as well
as our dataframe data model and algebra are 
omitted due to space limitations
and can be found in our technical report~\cite{petersohn2020towards}.}
% We also provide a bit of history into
% dataframe origins in Section~\ref{sec:dataframe-history}.
We begin our paper with a specific dataframe workflow that will serve
as a running example for the paper. 



% \newpage

% In this paper, we 
% {\bf \em (i)
% % define a research agenda around 
% % formalizing
% provide a candidate formalism for
% dataframes} and enumerate their capabilities with a new algebra,
% and {\bf \em define a research agenda that builds on our formalism
% to make dataframes faster and more scalable,}
% by leveraging tools and techniques from the database community; 
% and {\bf \em (ii) describe
% our first steps toward this goal with our prototype, \modin}. 
% \modin (\url{github.com/modin-project/modin}) 
% is an accelerated implementation of the \pandas dataframe API,
% enabling unmodified \pandas code to run with more efficiency and scalability;
% \modin is already used by over 60 downstream projects, and
% has over 250 forks and 3,900 stars on GitHub
% in its first 18 months, 
% indicating the promise and need for pursuing this agenda. 
% We cast our agenda 
% into multiple overarching goals.

% \stitle{1. Formalizing (Section~\ref{sec:definitions}) and 
% implementing (Section~\ref{sec:modin}) dataframes.}
% Dataframes are different from database relations and
% matrices. Unlike database relations,
% dataframes are ordered, treat col\-umns and rows symmetrically,
% and have weakly specified schemas.
% Unlike matrices, dataframes have heterogeneous types,
% can have row and column names as metadata,
% and are often processed via operators 
% more akin to relational algebra than linear algebra.
% Our first goal is to 
% provide a formalization
% of the dataframe data model and identify
% a concise algebra of dataframe operations
% that can capture the API of an 
% existing dataframe implementation, \pandas,
% with over 200 operators---a substantial challenge.
% Existing \pandas queries 
% can then be rewritten using 
% the algebra, and we can focus
% on optimizing queries in this algebra,
% a much more tractable problem.

% \modin, our prototype, captures our progress
% on formalization
% to date. 
% \modin rewrites 
%  \pandas API calls 
% into a sequence
% of algebraic operators,
% allowing  
% \pandas code to run as-is without changes.
% \modin then leverages simple 
% parallelization and a new physical 
% representation 
% to speed up the 
% execution of these operators,
% by up to {\bf 30$\times$} in certain
% cases, and is able to run to completion
% on datasets {\bf 25$\times$} larger 
% than \pandas (which crashes instead) 
% in others.


% \stitle{2. Optimizing dataframe {\em queries} (Section~\ref{sec:datamodel}).}
% Given the new algebra, 
% our second goal is to reduce
% the latency for dataframe queries---an expression composed of multiple
% dataframe operators---by revisiting every
% architectural layer of a typical
% dataframe query execution stack:
% ranging from data representation,
% to buffer management, 
% to indexing and views, 
% to rewriting, cost modeling, and optimization.
% Optimizing dataframes in these ways is
% substantially different from the typical database systems
% stack due to the new data model and algebra,
% leading to new challenges.

% \ctitle{Examples of Challenges.}
% From a representational viewpoint,
% how do we represent heterogeneous 
% data that is ordered along rows
% and columns, often with millions or billions of each?
% Current dataframe systems simply represent
% data ``as is'', without obeying 
% physical data independence, 
% leading to missed opportunities.
% Once we pick a representation,
% how do we support ordered access to data via indexes, as well as 
% access using row and column labels? 
% And, given that dataframes are lazily typed,
% when and how do we detect and represent 
% the column types,
% and maintain it across operations?

% From a querying viewpoint, 
% current dataframe systems don't support
% data that doesn't fit in memory---how do we go beyond main-memory limitations?
% How do we support pipelining with the new dataframe algebra---another 
% key optimization not present in current dataframe systems?
% Likewise, what rewrite rules apply for this algebra?
% Given the inherent ordering in the data model,
% certain (ordered) operators are, in fact, no longer commutative.
% Current dataframe systems do not rewrite queries, executing
% them as is. 
% Finally, how do we optimize queries in the dataframe algebra? 
% Here, the notion of Selinger-style ``interesting orders''~\cite{selinger1979access} is not simply for performance
% reasons, but is a first class citizen of the data model.
% %\agp{perhaps 2 lines on new challenges--borrow from old text}

% % The new data model and algebra make
% % all of these components
% % challenging to develop. 

% % Identifying a set of rewrite rules
% % for the entirety of the dataframe operator combinations
% % is a daunting challenge.
% % Using these rewrite rules, along with a cost model,
% % for dataframe operators,
% % we can develop a Selinger-style query optimization
% % framework~\cite{selinger1979access}. 
% % \jmh{Cascades is probably a better goal.}
% % One important nuance here is that
% % the notion of interesting orders is not simply
% % a convenience for query optimization,
% % but is also a first-class citizen within dataframes.



% \stitle{3. Optimizing dataframe {\em sessions} (Section~\ref{sec:interactivity}).}
% Dataframe queries are typically executed
% in the context of a {\em session},
% wherein simple expressions are first composed
% and validated, followed by more complex expressions
% that build on the simple ones. 
% At every stage, the user interactively 
% examines the results of intermediate expressions,
% usually for debugging purposes. 
% Our third goal aims to further
% reduce latency for session-based execution 
% by providing {\em immediate feedback} (Section~\ref{sec:immediate-feedback})
% for intermediate sub-expressions,
% and by leveraging {\em sharing and reuse} (Section~\ref{sec:sharing-and-reuse})
% to accelerate the computation of sub-expressions
% that incrementally build on top of each other,
% providing a number of interesting research challenges.

% \ctitle{Examples of Challenges.}
% Current dataframe systems evaluate each expression in its entirety
% after it is composed, forcing the user
% to wait until the result is computed; 
% other data systems~\cite{Armbrust:2015:SSR:2723372.2742797}
% opt for entirely lazy evaluation, deferring
% computation until the user requests to inspect the result, forcing them
% to wait then. 
% Instead, can we perform background computation to 
% compute the results of query sub-expressions in the background,
% while still prioritizing the 
% results that the user actively requests, giving us the
% best of both worlds?
% In doing background computation of this form, 
% we may have many query sub-expressions 
% concurrently being executed.
% How do we execute all of them while sharing computation
% as much as possible, prioritizing those 
% whose results the user might examine? 
% Then, when the user actually 
% examines a result, the user typically previews the
% first or last $k$ result rows; how do we prioritize
% returning these rows over the rest, especially with an ordered
% data model and a new algebra? 
% We can return a response even faster 
% by recognizing
% that users typically inspect intermediate results
% for debugging. 
% So how do we allow users 
% to view an approximate version of 
% each intermediate result quickly, so that
% they can move on to the next step of analysis? 
% Finally, 
% given that users often iteratively compose queries many times
% over the course of a session, 
% building on top of previously composed sub-expression results,
% how do we leverage materialization and reuse to accelerate
% computation? 



% % by leveraging (i) {\em interactive} computation that
% % displays partial, possibly approximate results
% % for quick validation (Section~\ref{XXX}), and 
% % (ii) {\em background} computation that 
% % computes many incrementally constructed query 
% % sub-expressions in parallel, and 
% % intelligently 
% % reuses materialized sub-expressions (Section~\ref{XXX}).



% % Our third goal aims to further
% % reduce latency for session-based execution,
% % by leveraging (i) {\em interactive} computation that
% % displays partial, possibly approximate results
% % for quick validation (Section~\ref{XXX}), and 
% % (ii) {\em background} computation that 
% % computes many incrementally constructed query 
% % sub-expressions in parallel, and 
% % intelligently 
% % reuses materialized sub-expressions (Section~\ref{XXX}).

% \vspace{5pt}
% \noindent 
% In describing the aforementioned challenges, we focus on the \pandas dataframe system~\cite{pandas-api} 
% for concreteness. 
% \Pandas is much more popular than other dataframe 
% implementations,
% and is therefore well worth our effort to study and optimize.
% \todo{Reference tech report}
% We will discuss other dataframe
% implementations and related work in Section~\ref{sec:ext}.
% We also provide a bit of history into
% dataframe origins in Section~\ref{sec:dataframe-history}.
% We begin our paper with an example dataframe workflow that will serve
% as a running example for the paper. 


% % \stitle{4. Clean slate design (Section~\ref{sec:clean-slate}) and other dataframe implementations (Section~\ref{sec:ext}).}
% % Our final goal involves a
% % clean-slate design
% % of dataframes without the baggage of backward 
% % compatibility---preserving the best features of dataframes,
% % while getting rid of  redundant syntax. 
% % We want to also study the trade-off between expressiveness
% % and optimization ability (i.e., 
% % how does each new operator
% % impact our ability to optimize queries efficiently). 

% % To make first steps towards that goal, we consider how
% % our work so far would apply to other 
% % dataframe implementations in Section~\ref{sec:ext}.
% % The reason we focus on \pandas 
% % for most of the paper is because
% % it is much more popular than other dataframe implementations,
% % and is therefore well-worth our effort to study and optimize.


% % \smallskip
% % \noindent 
% % We begin our paper with an example workflow that will serve
% % as a running example for the paper. 

% % \section{Roadmap: Dataframe Challenges}

% % \stitle{Challenge 1: Formalizing Dataframes.}
% % Despite the popularity of dataframes, little is known about 
% % the ``formal'' dataframe data model and algebra and its
% % relationship with relational,
% % linear, and spreadsheet algebra. 
% % As mentioned previously, the \pandas API has over
% % 200 operators, making it cumbersome to understand and remember,
% % as well as optimize queries or operators. 
% % However, as we will see later,
% % many of these operators can be viewed
% % as a combination of relational operators 
% % \william{2.2 also depends on new "dataframe operators" (e.g., transpose, flatten (maybe))}
% % on ordered relational tables, along with user defined functions. 
% % Unlike relational tables, however, column types
% % are often not defined up front, and data
% % is often in various stages of cleaning. 
% % Furthermore, since dataframes treat columns and rows
% % equivalently (like linear algebra), 
% % and treat ``metadata'', e.g., column labels,
% % like data (like spreadsheet algebra~\cite{bendre2019anti}),
% % \jmh{citation for ``spreadsheet algebra''?}
% % there is a need to support both
% % transpose-like operations and operations
% % that move metadata to data, and vice-versa. 
% % \agp{maybe also bring up our flatten as an unusual non-relational
% % and non-linear alg op.}
% % \jmh{all that stuff is in various second order query languages, e.g. for XML. Not novel per se.}
% % Dataframes also draw from similar notions
% % in array constructs in programming languages 
% % to support named ``indexes''
% % as a first class citizen. 
% % These indexes,  
% % unlike indexes in relational databases,
% % are primarily used to refer to rows and columns,
% % as opposed to being a data structure
% % to speed up retrieval.
% % Formalizing all of these notions under
% % a unified dataframe data model,
% % coupled with a concise algebra 
% % to support all of these operations,
% % is a substantial challenge, and one
% % we've made some headway in while developing \modin.
% % \jmh{awk. ``challenge; \modin
% % captures our progress to date.} 







% % \stitle{Challenge 2: Single Statement Acceleration.}
% % The algebraic kernel and data model opens up a number
% % of interesting and important optimization 
% % opportunities, drawn from the database community, 
% % centered around executing one single statement at a time.
% % Many of these
% % challenges arise from the way in which dataframes are
% % used and interacted with.

% % \emtitle{Asynchronous Computation.}
% % Dataframe users do not compose the entire
% % query at once like in SQL, instead building it up
% % over the course of several statements,
% % each appending one or more operators.
% % Taking a relational query example,
% % dataframe users may specify an ordered join first, 
% % followed by a filter, instead of specifying it all at once.
% % Instead of executing each statement immediately,
% % we can instead return control to the user,
% % and then enqueue their execution in the background
% % as they complete their data pipeline, taking
% % advantage of think time. 
% % \jmh{I agree with the spirit of this, but of course I can keep issuing more and more complex variants of a SQL query too. So it's a purely syntactic argument, and requires more syntactic argumentation. I think the main thing is the ``diff'' between a simple query and its extension into a more complex query. Function chaining syntax (essentially, algebra) is the win -- far preferable to SQL syntax for localizing the diff, in a natural place (the end!).}
% % \jmh{Frankly even relational calculus is preferable to SQL, but maybe there's a deeper point about algebra vs. logic here in terms of the need in logic to modify the quantifiers as well as the predicates???}
% % \jmh{Final note from many years with Trifacta's algebra: multi-table query expansion (JOIN, UNION) subverts this argument a fair bit because function chaining is linear and a multi-table query is a tree or DAG. So it's a less natural fit. You end up with an arbitrarily-chosen ``first'' table that ``drives'' the expression, but you get unpleasant problems when you decide that the driving table should actually be the inside of a subquery type expression (EXISTS, anti-join/NOTIN). Or if you decide the driving table isn't interesting and should be removed from the query. Still, I agree for simple cases, and simple cases take priority for exploratory work!}
% % In this case, the challenge 
% % \jmh{I'd say this is an ``opportunity''---this pattern of incremental refinement is less common in SQL, perhaps due to its syntactic ergonomics, so it got relatively little attention before. To be honest I'm not sure if you should even reveal this research idea prior to results!}
% % is to adaptively
% % change the execution strategy~\cite{deshpande2007adaptive} as the query is progressively
% % revealed, 
% % \jmh{A better ref for this may be [33], which
% % is specifically about early return of partial results.}
% % while making use of previously computed
% % partial results as much as possible (e.g., in our example,
% % reusing partial results from the join, while now switching
% % to pushing the filter down for the remaining computation).
% % \william{Confusing as we do not introduce the example until 2.1.}
% % In our preliminary \modin prototype, we demonstrate the promise
% % of asynchronous computation even without
% % adaptivity: each operator is executed in the background
% % in the order it is provided.

% % \emtitle{Parallel\phantom{y}Execution.} 
% % Most dataframe libraries
% % do not take advantage 
% % of multiple cores or sockets to speed up execution.
% % There are several challenges in enabling
% % the use of multiple cores.
% % For example, 
% % different types of operators have different
% % inherent parallelism and communication patterns.
% % We have so far identified 16 different mechanisms for parallelization
% % amongst the 240 different operators provided by \pandas,
% % and have used that insight to parallelize as much as possible
% % in our prototype, \modin.
% % However, many challenges remain unaddressed, specifically relating to 
% % preservation of order  
% % while parallelizing.
% % Relational operators
% % are commutative and associative; however, some dataframe operators
% % rely on the order and cannot be parallelized easily.
% % \jmh{There are a couple issues being conflated here. One is commutativity/associativity of operators
% % (e.g. inner join reordering). Another is commutativity/associativity of handling data (insensitivity to ordering/batching of data being processed).}
% % For example, operators that rely on windowed computation
% % (such as a cumulative sum) cannot be as easily parallelized.
% % \jmh{citations?}
% % In a single dataframe statement (i.e., smallest unit of execution), users can often mix operators
% % that can and cannot be easily parallelized, making it challenging
% % to schedule their execution optimally.
% % \william{We do not introduce statements until 2.2}
% % \dlee{expanded on the description to describe statement better}

% % \emtitle{Prefix or Suffix Computation.}
% % Users inspect intermediate
% % results during the construction of a multi-step query 
% % for debugging purposes,
% % via the \code{head} or \code{tail} operation (analogous to
% % the corresponding bash command).
% % Furthermore, \pandas already
% % caps the number of rows displayed
% % during pretty printing to a fixed parameter, 
% % \code{max\_rows}, set as 10 by default.
% % In such cases, we can provide partial results 
% % to the user, by prioritizing the execution 
% % to reveal those rows first and computing
% % the rest in the background. 
% % Unlike the traditional relational 
% % setting of returning 
% % any $k$ results quickly, e.g., via a \code{LIMIT} clause or
% % by maximizing the output rate~\cite{viglas2002rate},
% % here, the inherent order poses additional challenges
% % and opportunities.
% % \jmh{Most common use case of LIMIT is with
% % ORDER BY. I'm 100\% sure there are papers
% % on this to cite.}


% % \emtitle{Approximate Computation.}
% % Since users may not require 
% % exact results during ad hoc exploration,
% % approximate query processing techniques (AQP) 
% % may be employed to quickly display 
% % inexact results at significantly
% % reduced latency. 
% % The full computation can 
% % then continue to run in the
% % background, periodically displaying 
% % progressively refined results to the
% % user~\cite{hellerstein1997online,rahman2017ve}, 
% % or eventually displaying the exact result 
% % for the user to verify against 
% % the approximation~\cite{moritz2017trust}.
% % Traditional AQP has usually been applied
% % to accelerate the generation of specific aggregates,
% % e.g., \code{SUM} or \code{AVG}, and bound
% % their estimates with confidence intervals; 
% % however, in this case, there may be additional opportunities 
% % for approximation if the user simply wants to 
% % inspect the approximate structure of the result 
% % for debugging purposes,
% % especially in conjunction with prefix computation.
% % For example, we can provide the 
% % overall structure of the output of 
% % a pivot table computation (displaying the row-wise groups and column headers), 
% % without actually filling in any of the aggregate values. \jmh{This is very close to [33].}

% % %As we will see in Sections~\ref{sec:approx} and~\ref{sec:mqo}, while many traditional approximation techniques may be 
% % %applied in a cookie-cutter fashion, their interaction with the other dataframe
% % %optimizations we identify provides several interesting research challenges.

% % \stitle{Challenge 3: Acceleration Across Statements.}
% % Additional optimization opportunities emerge when we consider
% % accelerating across multiple statements,
% % without changing the core capabilities of dataframes.
% % All of these optimizations take advantage of asynchronous computation,
% % whereby we can string together multiple statements and
% % compute them together in the background. 

% % \emtitle{Rewrite\phantom{y}Rules and Cost-based Optimization.} 
% % Like we described in the asynchronous processing
% % case, in a dataframe workflow, 
% % we may have subsequent statements
% % that should really be executed first,
% % e.g., an ordered join followed by a filter, 
% % via two separate
% % statements,
% % where the filter can be applied first.
% % Identifying a set of rewrite rules
% % for the entirety of the dataframe operator combinations
% % is a daunting challenge.
% % Using these rewrite rules, along with a cost model,
% % for dataframe operators,
% % we can develop a Selinger-style query optimization
% % framework~\cite{selinger1979access}. 
% % \jmh{Cascades is probably a better goal.}
% % One important nuance here is that
% % the notion of interesting orders is not simply
% % a convenience for query optimization,
% % but is also a first-class citizen within dataframes.

% % \emtitle{Materialization and Indexing.}
% % As described for prefix computation, users often follow
% % a trial-and-error-based programming paradigm, where
% % the user tries a query and checks the output for
% % correctness. 
% % We may be able to leverage this insight
% % at the workflow level as well.
% % A significant amount of computation
% % can be saved if intermediate results are saved
% % and reused for future computation.
% % However, this has to be balanced against the available memory
% % and effects on caching and garbage collection---but could be
% % highly effective in large memory environments.
% % In some cases where the same workflow is re-run repeatedly with 
% % small changes, we may consider automatically constructing indexes,
% % or performing speculative execution for operations
% % the user is likely to perform.



% % %\devin{Discuss challenges related to interaction between asynchrony and parallelization. There is some speculation required because you may need to compute everything or you may only need top k results.}

% % \emtitle{Multi-query Optimization.}
% % \modin currently employs asynchrony, enqueueing operations for execution
% % in the background so that control may be returned to the user immediately.
% % These enqueued ``queries'' may operate over very similar or even
% % identical sets of data. As such, \modin can employ multi-query
% % optimization techniques~\cite{sellis1988multiple}
% % in order to schedule multiple
% % operations for simultaneous execution, reducing cache misses
% % when the same background scan can support computation of multiple
% % analytical functions.

% % \stitle{Challenge 4: Clean-Slate Implementation.}
% % Our final goal is to perform a from-scratch implementation
% % of dataframes without the baggage of backward compatibility.
% % In particular, we want to preserve the best features of dataframes
% % as outlined previously, while getting rid of the redundant syntax. 
% % We want to also study the trade-off between expressiveness
% % and optimization ability, i.e., 
% % how does each new operator that is added
% % impact our ability to optimize queries efficiently. 
% % Our goal is to identify a {\em minimal} kernel of operators
% % that every dataframe implementation should support,
% % expanding beyond \pandas to other implementations as well.
% % Subsequently, we can develop rewriting rules,
% % a cost model, and optimization techniques
% % centered around this minimal dataframe algebra.
% % \jmh{Maybe the convention we should adopt 
% % in the writing is 
% % that the logical operators form an algebra,
% % and the operator implementations form a 
% % ``kernel'' of a query engine.}





==> modin-bkp-5-22-2020.tex <==
%!TEX root = modin-vision.tex

\section{The Modin Dataframe System}\label{sec:modin}

% \removed{
% \modin 
% % \footnote{\modin's name comes from the Korean
% % word for every, as in every \pandas operator or every
% % dataframe API.}
% is our open-source  
% dataframe system that implements 
% the data model and algebra described 
% in Section~\ref{sec:definitions}. 
% }
\rebuttal{
While the \pandas API is convenient and powerful,
the underlying implementation has many scalability
and performance problems.
We therefore started an effort to develop
a ``drop-in'' replacement for the \pandas API, \modin,
to address these issues. 
We identified that while many operations in \pandas
are fast, they are limited by their
single-threaded implementation.
Therefore, our starting point for \modin 
was to add multi-core capabilities and other
simple performance improvements to enable 
\pandas users to run their same unmodified workflows
both faster and on larger datasets.
We briefly describe the challenges we encountered
in our implementation and how we addressed them in Section~\ref{sec:optim},
followed by a preliminary case study of the performance of \modin
in Section~\ref{sec:accelerate}.
We then discuss takeaways and how that informs
our future research agenda in Section~\ref{subsec:takeaways}.
We defer detailed treatment of \modin's architecture
to our technical report 
}




\rebuttal{
We started an effort to build a drop-in replacement for
the \pandas API, \modin, to solve many of the
scalability and performance problems introduced by the \pandas implementation.
In \pandas many operations are fast, but limited by their single-threaded implementation.
As an engineering challenge, we targeted making \modin a drop-in replacement
that would add multi-core capabilities and performance improvements that \pandas
users could simply plug in to their existing workflows without 
requiring additional
knowledge. 
We began by integrating simple parallelism
and more efficient data management.
As we started the effort, we expected to directly
integrate best practices from relational system literature. 
However, we quickly discovered
that dataframes like \pandas do not conform to the relational data model.
Based on these differences, 
we derived a new data model from the behaviors and capabilities
of existing dataframe systems.
Armed with a new data model and algebra, we can consider the new challenges
in integrating relational database optimizations, many of
which we discuss in Sections 5 and 6, grounded in our experience building
a parallel dataframe system.
}

\moved{
\modin supports the \pandas API by rewriting the API
calls into a minimal subset. This subset
became the algebra presented in Section~\ref{sec:df-algebra}.
\modin is implemented in Python using over 30,000 lines
of code and emulates all the functionality of
\code{pandas.DataFrame}, \code{pandas.Series}, and
\pandas  utilities (e.g., \code{pd.\-concat}), 
while also yielding substantial (30$\times$) 
speedups over \pandas for certain operations.
To use \modin instead of \pandas, users can simply 
invoke ``\code{import modin.pandas}'',
instead of ``\code{import pandas}'', and proceed
as they would with \pandas.
\modin is completely open source and can be found at 
\url{https://github.com/modin-project/modin}.
}
\rebuttal{
We will reserve the implementation details and architecture 
of this system to another
paper, however it is important that we highlight 
our experience and lessons learned with implementing
some of the more exotic components
of the \modin dataframe system and some of the challenges therein.
}

% \subsection{The MODIN Architecture}\label{sec:architecture}

% \begin{figure}
% \centering
% \vspace{-5pt}
% \includegraphics[width=.4\textwidth]{modin_architecture_updated.png}
% \vspace{-5pt}
% \caption{\modin architecture.}
% \label{fig:modin-arch}
% \vspace{-15pt}
% \end{figure}

% \modin's architecture is {\em modular} 
% for easy integration of new storage and execution engines, APIs, and optimizations. It consists of four layers: 
% the API layer, the query processing
% and optimization layer, 
% the execution layer, 
% and the storage layer, shown in Figure~\ref{fig:modin-arch}.

% \stitle{API layer.} 
% Users can leverage
% \modin via a \pandas-based API,
% or directly via a leaner and simpler \modin API
% based on the algebra in Section~\ref{sec:df-algebra}.
% In either case, the API layer
% translates each call into 
% a dataframe algebraic expression,
% and passes that to the next layer for execution.
% The layer isolates users from changes
% to the layers below, while allowing
% users to leverage the API modality they are most
% comfortable with. 
% \techreport{Future implementations may support other user
% APIs for working with dataframes,
% such as SQL or relational algebra.}
% Our \pandas-based API currently supports
% about 150 of over 200 \pandas dataframe APIs,
% and rewrites each of them into dataframe
% algebraic expressions.

% % The API layer is the user-facing 
% % component of \modin, 
% % and is responsible for translating each API call into
% % the algebra and passing that translation to the \modin
% % DataFrame layer for execution. 
% % The layer isolates users from changes to the implementations and optimizations of the layers below, while enabling users to chose to use the API
% % they are most comfortable with using. To retain the vastly-popular \pandas API, we have implemented around 150 of the over 200 \pandas dataframe APIs in
% % \modin's architecture and algebra. In parallel, we are  developing
% % a leaner and simpler API based on the
% % algebra defined in Section~\ref{sec:df-algebra}. 
% % Users can choose to use \modin either via the \pandas API,
% % which is rewritten into the dataframe algebra, or directly via the algebra.
% % Future implementation may support other user APIs for working with dataframes,
% % such as SQL.

% \stitle{Query processing and optimization layer.}
% As shown in Figure~\ref{fig:modin-arch}, 
% the query processing layer follows a
% ``narrow waist'' design, 
% exposing a small API based on 
% the dataframe algebra,
% and implements the data model 
% from Section~\ref{sec:dataframedef}.
% This layer parses, optimizes, and executes 
% dataframe queries with the help
% of layers below. 
% As we will describe in Section~\ref{sec:optim},
% \modin leverages parallel execution 
% of dataframe queries on multiple
% dataframe partitions, 
% scheduled on execution engines
% in the next layer. 
% This layer also keeps track of 
% dataframe metadata  
% including row labels, column labels, 
% and column data types.
% \techreport{Recall that data types may not be specified
% on dataframe creation, so }
% \modin
% induces types on-the-fly (using the $S$ function)
% when needed for a specific operation.






% % As shown in Figure~\ref{fig:modin-arch}, the \modin DataFrame abstraction follows a ``narrow waist'' system design, exposing a small API based on 
% % the dataframe algebra defined in Section~\ref{sec:df-algebra}
% % and implementing the data model presented in Section~\ref{sec:dataframedef}.
% % The \modin
% % dataframe layer maintains the dataframe's metadata including row labels, column labels, and column data types, and simplifies the integration of 
% % new and existing optimizations into the system. 
% % As per our definition in Section~\ref{sec:dataframedef}, 
% % data types do not have to be materialized on creation,
% % instead \modin determines the types on-the-fly when they are needed
% % by a query or optimization. Inducing and computing the types is a
% % computationally expensive task, so it is not done unless
% % explicitly requested or required. \modin follows the data model described in Section~\ref{sec:dataframedef},
% % where the $S$ function is applied to every column to induce the types.

% \stitle{Execution layer.} \modin
% supports distributed 
% processing of 
% dataframe partitions
% using 
% two execution frameworks: 
% Ray~\cite{ray} and Dask~\cite{dask}.
% Both Ray and Dask are task-parallel asynchronous 
% execution engines exposing an API that requires defining a task or function and providing data for the task to run on. 
% Integration of a new
% execution framework is simple, often requiring
% fewer than 400 lines of code.

% \stitle{Storage layer.} 
% \modin's modular storage layer
% supports both main memory and 
% persistent storage out-of-core (also called memory spillover),
% allowing intermediate dataframes to exceed main-memory limitations
% while not throwing memory errors, unlike \pandas. 
% To maintain \pandas semantics, the dataframe
% partitions are freed from persistent storage once
% a session ends.

\subsection{Engineering Challenges in Dataframes}\label{sec:optim}
% \removed{
% We have started exploring two classes 
% of optimizations within \modin: 
% parallel execution and support for billions of columns.
% }
\rebuttal{
As we began studying the \pandas implementation, we discovered many
challenges in exposing the API. In this section we discuss the engineering
challenges we have encountered that are unique to the \pandas
dataframe implementation.
}

\stitle{Massive API.}
\moved{
\Pandas has been developed from the ground up
via open-source contributions; 
\pandas DataFrame API operators 
and their implementations
have been engineered 
by dozens of contributors 
to satisfy immediate or ad-hoc needs, 
spanning capabilities
that mimic
relational algebra, 
linear algebra, and 
spreadsheet formula computation.
To date, 
the \pandas DataFrame API has ballooned to 
over 240 distinct operators~\cite{pandas-api},
}
\rebuttal{
making it challenging to engineer and ensure adequate
API coverage.
}
% \rebuttal{
% There is also a significant development effort
% around \pandas, so any library that attempts to re-implement
% its API will have a challenging time keeping up-to-date.
% }

\rebuttal{
Currently, \modin supports over 85\% of
the \code{pandas.DataFrame} API. We chose the order
of implementation based on a study we conducted on
over 1 million Jupyter notebooks, the results of
which are discussed in our tech report~\cite{techreport}.
To solve this problem, we derived a kernel of operators
that represent the \pandas API, and layered the
\modin implementation to avoid duplicating logic
as much
as possible. As we developed the dataframe data model,
this kernel of operators became the
working dataframe algebra we will present 
in Section~\ref{sec:df-algebra}.
}

\stitle{Parallel execution.}
Parallelization
is commonly used to improve performance 
in a relational context 
due to the embarrassingly parallel nature 
of relational operators.
Dataframes have 
% \removed{some unique properties and requirements}
\rebuttal{a different set of operators
than relational tables, supporting relational algebra,
linear algebra, and some spreadsheet operators.
We will discuss these operators in detail in Section~\ref{sec:df-algebra}.}
\rebuttal{Each of these operators represents
a class of data manipulation APIs from pandas.
We implemented different internal mechanisms for 
exploiting parallelism} 
% \removed{that enable} different degrees of parallelism 
depending on the 
data dimensions and operations being performed. 
Some operations 
% \remove{, e.g., \code{MAP},}
are embarrassingly parallel and
can be performed on each row independently. 
% \removed{In contrast, \code{WINDOW}}
\rebuttal{Other}
operations do not admit 
row-wise parallelism 
because
computation for each subsequent 
row must wait for the result of the
prior row.
% \removed{Our current simple approach to partitioning is to 
% do it on a per-operation basis, and to pick between}
\rebuttal{To address the challenge of differing levels
of parallelism and support all of the operations in
existing dataframe implementations, we designed
a mechanism within \modin to be able to flexibly
move between all common partitioning schemes:}
row-based (i.e., each partition has a collection of rows), 
column-based (i.e., each partition has a collection of columns), 
or block-based partitioning 
(i.e., each partition has a subset of rows and columns),
depending on the operation.
\rebuttal{This gives \modin the flexibility to
take advantage of many optimizations in row-based systems,
column stores, and block stores.}
% \removed{Each partition is then processed independently
% by the execution engine, with the results communicated
% across partitions if need be. 
% For example, \code{MAP}, in general, 
% requires row-based partitioning, but
% in certain cases, depending on the function, 
% could also use column-based or block-based partitioning,
% e.g., when we are replacing all null values with another
% predetermined value. 
% On the other hand, when 
% applying \code{WINDOW} functions on multiple columns,
% or \code{GROUP BY} aggregates on multiple columns,
% column-based partitioning could be a good option.
% Finally, \code{TRANSPOSE}, especially
% on dataframes that have many rows and columns,
% can be done more efficiently with block-based partitioning,
% as we will discuss next. }

% Some operations, e.g. \code{MAP}, 
% are embarrassingly parallel and
% can be performed on each row independently. 
% In contrast, \code{WINDOW}
% operations limit parallelism 
% to the number of columns because
% computation for each subsequent row must wait for the result of the
% prior row.

% To efficiently parallelize dataframe queries,
% we developed a partitioning structure that treats data as:

% \squishlist
% \item Row partitioned: Each partition contains a subset of rows. This is an efficient way to represent the data during relational operations (e.g. \code{JOIN}). 
% \item Column partitioned: Each partition contains a subset of columns. This is an efficient way to represent the data during columnar aggregations (e.g. \code{GROUP BY}).
% \item Block partitioned: Each partition contains a subset of both rows and columns. This is an efficient way to represent the data during matrix operations (e.g. \code{TRANSPOSE}).
% \squishend

% This flexible partitioning schema allows \modin to compose appropriate partition schemes and maximally exploit parallelism, instead of being limited to a particular partition choice.

% \stitle{Row and Column partitioned.}
% Some dataframe algebra functions,
% such as window functions,
% must: 
% (1) be computed in order,
% (2) require access to other values along the row or column,
% or (3) both.
% Thus, to ensure correctness of these operators, they must be computed with access to the
% entire column or row in the proper order.

% \stitle{Block Partitioned.} 
% For embarrassingly parallel dataframe algebra functions,
% we are able to arbitrarily break up columns and rows into individual blocks 
% and apply the function on each block independently, and thus select the degree of parallelism that best optimizes the function.

\begin{figure*}[ht!]
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.9\textwidth]{perf_plots.pdf}
    \vspace{-10pt}
    \caption{%
        For each function, 
        we show the runtime for both \modin and \pandas 
        and the 95\% confidence interval.
        There are no times for transpose with \pandas as 
        \pandas is unable to run transpose beyond 6 GB.
    }
\label{fig:performance}
\vspace{-10pt}

\end{figure*} 
 
\stitle{Supporting billions of columns.}
\rebuttal{The majority of traditional} database systems 
cannot support tables with 
billions of columns; 
\rebuttal{In the \pandas API, however, }
it is possible to \code{TRANSPOSE} a dataframe 
with billions of rows 
into one with billions of columns. 
In many settings, e.g., when dealing with large graph
adjacency matrices in neuroscience or genomics,
the number of rows and number of columns can both be very large.
For these reasons, \modin treats
rows and columns essentially equivalently,
\rebuttal{as we will} discuss in Section~\ref{sec:definitions}.
In particular, for transposing a large dataframe,
\modin uses block-based partitioning on the large
dataframe, where each block consists of a 
subset of rows and columns.
Each of the blocks are individually transposed, 
followed by a simple change of the overall metadata 
tracking the new locations of each of the blocks.
The result is a transposed dataframe that does not
require any communication.

% The \code{TRANSPOSE} operator is often used in conjunction with other operators during data exploration with large scale dataframes. This is common in scientific domains such as neuroscience, where swapping rows and columns could result in millions or even billions of columns. \modin treats rows and columns as equivalent, which when combined with block partitioning makes implementing \code{TRANSPOSE} both simple and highly parallelizable.
% In contrast, implementing  \code{TRANSPOSE} in an RDBMS is a significant challenge because the resulting millions or
% billions of columns is far beyond the capabilities of most modern RDMBSs.

% As we show in the next section (Section~\ref{sec:accelerate}), \modin can
% easily handle \code{TRANSPOSE} on over 1.6 billion rows,
% which results in the same number of columns, followed by a \code{MAP}, which demonstrates that \modin can execute operators on data with over a billion columns. Supporting billions of columns
% was a requirement when we designed and built \modin, however most modern
% RDBMSs were not designed with this requirement in mind, and cannot feasibly support such large numbers of columns.

% \eat{\agp{This is more future work and can be postponed. I would also talk about how
% it is desirable to postpone/avoid transpose as much as possible given Figure 4c}
% In integrating dataframe workflows into existing RDBMSs, this will be a
% major challenge. While some of the behaviors of dataframes (e.g. order semantics) can
% be emulated in a relational system, it is difficult to support
% behaviors and features that aren't supported in the architecture of an RDBMS.}


\subsection{Preliminary Case Study}\label{sec:accelerate} 

\rebuttal{To study how some simple parallelism can improve the scalability of the \pandas
semantics,}
we evaluated \modin's performance against that of \pandas using microbenchmarks on an EC2 x1.32xlarge (128 cores and 1,952 GB RAM) node using a New York City taxicab dataset~\cite{nyc-taxi-data} that was replicated 1 to 11 
times to yield a dataset size 
between 20 to 250 GB with up to 1.6 billion rows.
We consider four queries: 
\squishlist
\item map: check if each value in the dataframe is null, and replace it with a \code{TRUE} if so, and \code{FALSE} if not. 
\item groupby ($n$): 
%\code{GROUP BY(DF, "passenger\_count", lambda d: d.count())} - 
group by the non-null ``passenger\_count'' column and count the number of 
rows in each group.
\item groupby ($1$): 
%\code{GROUP BY(DF, 1, lambda d: d.count())} -
count the number of non-null rows in the dataframe.
\item transpose: 
%\code{MAP(TRANSPOSE(DF), lambda d: d)} - 
swap the columns and rows of the dataframe and 
apply a simple (map) function across
the new rows. 
\squishend

% \eat{\agp{rewrite these into the algebra}
% \code{df.groupby().count()}, \code{df.count()}, and \code{df.trans\-pose().map(lambda s: s)},
%  representing the performance of the operators
% \code{GROUP BY}, \code{WINDOW}, and \code{TRANSPOSE} + \code{MAP}, respectively.}
\noindent
We highlight the difference 
between group by with one group and 
$n$ groups, because in a group by
with $n$ groups 
\rebuttal{
data shuffling and
communication is a
factor in performance.
With groupby(1),
the communication overheads
across groups are non-existent.
}
We include transpose 
to demonstrate that \modin
can handle data with 
billions of columns.
This query also 
shows where \pandas crashed or 
did not complete in more than 2 hours.

Figure~\ref{fig:performance} shows that 
for the group by ($n$) 
and group by ($1$) operations,
\modin yields a speedup of up to $19\times$ 
and $30\times$ relative to \pandas, respectively. 
For example, a group by ($n$) on a 250GB dataframe, 
\pandas takes about 359 seconds 
and \modin takes 18.5 seconds, a speedup of more
than 19$\times$.
For map operations, \modin is about 12$\times$
faster than \pandas.
These performance gains come from
simple parallelization of operations within \modin,
while \pandas only uses a single core.
During the evaluation of transpose, 
\pandas was unable to transpose 
even the smallest dataframe of 20 GB ($\sim$150 million rows)
after 2 hours.
Through separate testing, 
we observed that \pandas can only transpose 
dataframes of up to 6 GB ($\sim$6 million rows) on the
hardware we used for testing.

These performance numbers are preliminary 
results that demonstrate the promise of 
\rebuttal{integrating simple optimizations}. 
We plan to perform further analyses in support of future optimizations,
\rebuttal{the possibilities of which we discuss in later sections}. 

\subsection{The Future of Dataframes}\label{subsec:takeaways}

\rebuttal{
In our experience building the \modin dataframe system, we
discovered many new challenges in integrating optimizations and
best practices from relational database literature. 
Given the amount of impact that \modin has had with the relatively
basic optimizations presented in this section,
we feel that future works in developing and optimizing
dataframes will have a profound and lasting impact on the
data science community.
}

% \rebuttal{
% The dataframe
% is distinct from relational tables, as we will discuss in Section~\ref{sec:definitions}.
% Dataframes have a distinct data model, presented
% in Section~\ref{sec:dataframedef}, and a completely new set of
% algebra operators, presented in Section~\ref{sec:df-algebra}.
% Because dataframes are distinct, a new body of scientific work
% will be needed to address the new challenges and opportunities presented by
% the new data model.
% }

\todo{Consider moving outline here}


==> modin-rebuttal.tex <==
%!TEX root = modin-vision.tex

\begin{center}
{\LARGE \bf Summary for Revised Paper ``Towards Scalable Dataframe Systems''}
\end{center}

We thank the reviewers and meta-reviewer for their detailed 
and insightful feedback, and for giving us the opportunity 
to address their feedback in a revision.  
We have prepared a new version of the paper based on their suggestions, 
with updates to every section. 
In brief, the changes made include:

%\begin{compactenum}
%\item 
\smallskip
\noindent {\bf \em A. New section on challenges 
stemming from the dataframe data model and algebra.} 
We have rewritten 
Section~\ref{sec:datamodel} to center around the
unique characteristics of the dataframe data model
and algebra, 
and framed our research challenges with respect
to these characteristics.
These characteristics include
lazy typing and flexible schema,
the equivalence between rows and columns and 
data and metadata, as well as the centrality of ordering. 
The entirety of this section was rewritten
to address the concerns of the Reviewers and Metareviewer.

\smallskip
\noindent {\bf \em B. New section on challenges
stemming from the use of dataframes in data exploration.} 
We have likewise rewritten 
Section~\ref{sec:interactivity} to focus on the unique
challenges presented by the interactive approach 
for working with dataframes during data exploration. 
In particular, the new discussion centers
around the challenges associated with supporting
the incremental composition of dataframe expressions,
the need for inspection of intermediate results
for debugging and feedback,
and the trial-and-error nature of dataframe-based 
exploration.

\smallskip
\noindent {\bf \em C. Reorganization and reframing of paper grounded
in our experiences with \modin.}
Recognizing that reviewers were unclear about the structure
of the paper and what constituted the visionary part,
we reorganized the paper to move the discussion about our existing system
\modin first.
Specifically, we highlight early on
how our experience thus far in developing \modin informed our vision and
research agenda for the development of (a) an clean formalism
for the dataframe algebra, and (b) an optimized system for implementing
this formalism. 
We also significantly trimmed our discussion of \modin
and its optimizations.
These changes affect
the overall tone of the entire paper 
but are particularly evident
in the new Section~\ref{sec:modin}.

\smallskip
\noindent {\bf \em D. Centering the discussion of challenges around differences
between dataframes and relations.}
In addition to our changes in Section~\ref{sec:datamodel}
and Section~\ref{sec:interactivity},
where we focus on novel challenges that arise in dataframe
systems when contrasted with relational databases,
we also updated the rest of the paper to reflect this tone.
In particular, large parts of Section~\ref{sec:intro} were rewritten
to describe the novel challenges with the dataframe data model
and algebra as well as novel challenges in how dataframes
are manipulated during data exploration workflows. 


\smallskip
\noindent {\bf \em E. De-emphasis and removal of non-visionary aspects.}
In addition to removing content in Section~\ref{sec:modin}, 
we have also made our example in Section~\ref{sec:usecase}
much more concise,
as they both did not add to the visionary content of the paper.
We have also removed or rewritten 
substantial portions of text 
in Section~\ref{sec:definitions} around 
obvious rewriting rules (leaving as-is a single case study
centered on pivot), the comparisons between the dataframe 
data model and other data models, as well as
extensions to the dataframe data model.
Instead, we used that space to augment Sections~\ref{sec:datamodel} and \ref{sec:interactivity} with new visionary content.


\smallskip
\noindent {\bf \em F. Other significant writing changes.} 
We have made considerable changes to the text 
of the paper to improve its overall readability. 
Specifically, we have focused on making the paper 
more clear, formal, and concise. 
We have rerun an experiment to verify that
a spike was indeed due to experimental variance.
Finally, we have also improved presentation by replotting figures, 
making our notation consistent, and fixing typographical errors.

\smallskip
The changes in the paper are highlighted in \rebuttal{\bf purple}. 
Unfortunately,
due to the new additions, this meant that our paper ended up being longer than we could fit in the 12+4 pages;
additional details  can be found in our extended technical report~\cite{petersohn2020towards}.
%\end{compactenum}
We address the specific points raised in each of the individual reviews below, starting with the meta-review.


\subsection*{Metareview}
\com{(M1) 
The description of the existing system should be reduced and rephrased
to be more of a technical background rather than 
sounding like a research paper.
}

We have substantially reduced the amount of
detail in each of 
Sections~\ref{sec:usecase}, \ref{sec:modin}, 
and \ref{sec:definitions}, and 
only kept details
that are pertinent to the vision components of the paper. 
We now describe in detail what was
removed or revised.

In Section~\ref{sec:usecase}, 
we removed portions
that were self-explanatory or easily understood. 
We also replotted Figure~\ref{fig:example} 
to take up less space. 
Descriptions of how users 
interact with a dataframe system 
were moved to later sections 
when describing the motivations for 
improving certain interaction modalities.

In Section~\ref{sec:modin}, we substantially 
reduced the amount of detail on our current implementation
of \modin.
Recognizing the purpose of this section
is to describe our experience with dataframes
thus far, and to use that to 
set the stage for our future research
agenda, we moved this section
to right after Section~\ref{sec:usecase}
as our prior work.
We entirely removed any architectural
descriptions about \modin as they are not relevant
for our vision. 
Since the techniques underlying \modin 
thus far are straightforward, we
made their description much more concise.
Since there was also 
some confusion about what had been implemented 
and what was future work, we
also cleared that up by making 
Section~\ref{sec:modin} the ``already implemented''
component and making 
latter sections more vision-oriented to convey
that those are indeed future work. 

In Section~\ref{sec:definitions}, we have made substantial
changes to all subsections.
We removed much of the detailed
discussion on the finer points of the described
data model in Section~\ref{sec:dataframedef}.
Some of this detail was moved
to Section~\ref{sec:datamodel} to motivate 
some of the research challenges in dataframes, 
but many details were removed entirely from the
paper if they did not add to the overall vision.
We also replaced some lengthy text with two compact
tables. 
We entirely removed the workflow definitions part,
choosing to introduce some of these terms 
as needed later on.
In Section~\ref{sec:df-algebra}, 
we made significant cuts to the explanation of
the operators. 
Since this paper does not try to argue
minimality, we use
these operators more as a frame of reference 
to describe the new challenges in efficiently
processing dataframes as opposed to providing
formal definitions. 
We only kept the components that tie 
directly to later sections of the paper 
where our future research problems are described. 
We have revised Section~\ref{sec:algebra-example}
to only convey one single case study on \code{pivot}
as opposed to many straightforward examples
of rewriting of \pandas API operators into
the dataframe algebra.
(We also enhanced this case study to add more
detail, along with a new figure.)
Former Section 3.5 (now would be 4.5) was entirely
removed, since the extensions to the data model
does not add much to the vision portion of the paper.


While we have cut back substantially in all of
Sections~\ref{sec:usecase}, \ref{sec:modin}, 
and \ref{sec:definitions},
further cuts would hurt understanding 
for database readers. 
Specifically, we believe an important contribution 
of this paper is to provide some background into 
dataframes and their characteristics.  
One of our reviewers remarked that they were skeptical of
any difference between dataframes and databases before they read this paper,
but this background was effective in convincing them 
that they are distinct artifacts
and will require a new body of research.


\com{(M2) 
The integration between the technical background and the vision needs to be improved.
Specifically, the vision focuses on the more general problems in data exploration
and does not focus on how these problems are different in dataframes
(as compared to relational settings).
}

\com{AND}
% We combine our comments for (M2) and (M3) to avoid repetition and
% for ease of review.

\com{(M3) 
The identification of the unique challenges of dataframes needs to be better.
Additionally, the challenges of relational systems which dataframes exacerbate
and that which dataframes lessen. 
}

To highlight how the discussed 
challenges are specific to dataframes,
we have significantly restructured the paper to provide
a more familiar flow
and have substantially revamped
Sections~\ref{sec:datamodel} and \ref{sec:interactivity}
taking the reviewer comments into account.

Specifically, for Section~\ref{sec:datamodel},
we had originally anchored our discussion around
``layers'' of a database system architecture 
to provide a familiar point of entry for a VLDB audience.
Likewise, for Section~\ref{sec:interactivity},
we had originally organized our proposed directions 
around ideas (many of them stemming from general
data exploration) as opposed to unique dataframe aspects.
We also focused too much on solutions rather than the underlying problems and why they are interesting
and unique.
After reading the reviews, 
however, we realized that this was not an optimal approach
for conveying our vision for scalable dataframe systems. 

As such,
we have now focused these sections around 
unique challenges in the dataframe
data model and algebra (Section~\ref{sec:datamodel}) 
and in how dataframes are manipulated over
the course of a user exploration session
(Section~\ref{sec:interactivity}).
When describing these challenges, we focused
on the key differences between operating on dataframes
and on relations. 
%We have also added a new section,
%Section~\ref{sec:algebra-challenges}, to discuss the challenges specific to
%the new algebra and our vision on how systems might solve some of those problems.
Prior to these sections, we 
set the stage for our research vision in the
substantially revised Section~\ref{sec:modin}
which describes what has been implemented,
and how that informs our future agenda.
We now explain the changes to Sections~\ref{sec:datamodel} and ~\ref{sec:interactivity}
in detail.

In Section~\ref{sec:datamodel}, we organize
our discussion around various unique properties
of dataframes, including flexible schema, lazy typing,
row-column equivalence (thanks to operators such as transpose), data-metadata equivalence (thanks to the presence of 
row and column labels
and operators that allow labels to become part of data),
and the centrality of order for both rows and columns. 
We ground this discussion by drawing on prior work in the
relational database community, and discuss why those
techniques would not apply to dataframes without violating
key dataframe properties. Grounding
the discussion in this manner helps us contrast the future
work needed to develop dataframe systems with existing work 
on relational databases.

% \agp{There is some text following this that I don't like 
% that elaborates on the previous. We can possibly
% omit it and leave it as it is above. Or revise it as time permits.}
% \devin{See above}
% \done{
% We first focus
% on the challenges of supporting flexible schemata, which is a particularly
% salient property for dataframes. Re: lazy typing, we describe when and how the schema 
% induction function $S$---a costly operation---should be invoked
% to induce the schema, 
% and how its invocation can be avoided if possible.
% We also discuss how difficult certain optimizations, like memory layout and
% compression, will be difficult in dataframes and require new techniques which
% will be developed as dataframes are researched.
% We then
% describe another unique property of dataframes, order as a first-class citizen,
% and the challenges involved in supporting order. We discuss works in relational
% algebra that may partially apply and certain cases where novel approaches will
% be needed. We discuss different hypothetical memory layouts for presenting
% data as ``ordered'' without placing physical requirements on ordering the
% data. We also discuss challenges and potential solutions in the area of query
% optimization when users must be presented an ordered view.
% }
% \agp{end text that may be deleted/revised}


%\done{
%\stitle{Section~\ref{sec:algebra-challenges}}. Many points in the algebra section
%were discussions on the challenges in supporting the algebra, but this structure was
%not condusive to the vision structure. Instead, we have created a new subsection and
%included the discussion around the challenges in supporting
%specific operators. We have expanded on the challenges and included
%our vision of potential pitfalls of certain approached moving forward.
%}

In Section~\ref{sec:interactivity},
we have centered our research challenges around the unique
ways in with dataframes play a role in data exploration.
Specifically, dataframes are usually manipulated interactively
over the course of a long-running user session,
with dataframe queries composed incrementally as individual \stmts,
a small number of operators at a time,
with subsequent invocations building on previous ones. 
Users often revisit previous steps in their exploration,
trying out different exploration strategies in a trial-and-error fashion.
They also inspect intermediate results often with 
an eye towards debugging and validation.
These characteristics are unique to how dataframes
are manipulated across data exploration sessions
typically performed in an interactive environment
such computational notebooks.




% \done{
% This feedback was addressed while resolving (M2).
% }


\subsection*{Reviewer 1}
\com{(A1) It is unclear as to which parts are the technical details
that are currently implemented in the system (which are less suited for a vision paper)
and which parts are the novel visionary contributions of the paper.
}

This feedback was addressed while resolving (M2/M3).


\com{(A2) 
It would be nice to see more discussion 
on the semantics of the group-by (resp. window) operator.
}

We thank the reviewer for this suggestion. We agree that
the semantics of dataframe \code{GROUPBY} and \code{WINDOW} deserve
special attention, particularly the ways in which they
deviate from their SQL/relational algebra counterparts. 
In particular, the fact that dataframes can support
composite types per cell
means that the dataframe algebra can use a broader class of aggregation
functions, not restricted to those that result in a single atomic value. This behavior
is also reflected in \pandas' \code{groupby} operator.
We have added additional
discussion in Section~\ref{sec:df-algebra}, highlighting how certain
functionality can be expressed more elegantly using the dataframe
variants of these primitives.
% , while additionally admitting challenges
% for query planning and optimization.

%\agp{We need to do something for this. A few lines
%in the algebra section will do.}
%\devin{Do we? Can't we say that there are no real dataframe
%challenges outside of the order? We discuss the Window op there}
%\done{
%To keep the vision central to the paper, 
%we have added an entire section to the paper on our vision
%of the challenges related to the algebra and operator set that is 
%exposed by \pandas and other dataframe implementations, 
%Section~\ref{sec:algebra-challenges}. The new section serves as the discussion
%for the vision of optimization based on query planning and optimization
%given a new set of algebra operators.
%Specifically, in \pandas, the semantics are a column-wise groupby followed
%by some operator. There is an intermediate object created by
%\code{df.groupby} calls in \pandas, which can be reused. We can express this
%semantic difference in the algebra with a \code{GROUPBY} on each column,
%followed by the aggregation.
%}

% \todo{
% \stitle{Alternative.}
% We added a discussion around the challenges of the groupby and
% window operators in dataframes in Section~\ref{sec:interactivity}
% to keep the discussion centered around future challenges and our vision
% on dataframe optimization with respect to the operator semantics.
% Specifically, the semantics of \code{GROUPBY} in \pandas are
% different than the traditional \code{GROUPBY} in relational algebra,
% but those semantics can be expressed in the algebra we presented.
% In \pandas, the semantics are a column-wise groupby followed
% by some operator. There is an intermediate object created by
% \code{df.groupby} calls in \pandas, which can be reused.
% }

\com{(A3) 
It would be nice to see more discussion
on the interplay between dataframes and data visualizations.
}

Visualization is indeed 
an important component
of data exploration with dataframes,
and not mentioning it was an oversight.
We now have added a brief 
discussion in Section~\ref{sec:interactivity} 
on how the default 
tabular view displayed when dataframes are printed
(a prefix/suffix of the rows and columns)
is a simple form of visualization for 
debugging and validation of structure and order,
but other forms of visualization may also be 
valuable.
We also have added a discussion around 
how prior work on approximate
decision making with visualization for
debugging and validation may be adapted.
% We then 
% focus our research questions around
% activities performed during data exploration,
% including visualization;
% one specific instance is how 
% approximate query processing (AQP) 
% can be applied to dataframes to 
% generate aggregate visualizations.


% \agp{Revise in a way that can highlight unique aspects to dataframes.}
% \done{
% Visualization is an important component of the dataframe data science
% life-cyle, and not including a discussion about this relationship
% was an unfortunate oversight. We have added a discussion in Section~\ref{sec:interactivity} on how dataframes are used with visualization and how they may be optimized in the future. Specifically, we argue how the tabular view is the one of the most common form of visualization of a dataframe. We also describe three class of optimizations for providing interactive feedback, so that users can quickly visualize and validate structural and order information of the dataframe. In addition, we also describe how approximate query processing (AQP) can be applied to dataframes to generate aggregate visualizations, citing prior work in this space.
% }


\com{(A4) 
The visonary aspects of the paper are dissappointing.
The authors discuss standard interactive data exploration tasks rather than
discussing the specific challenges posed and opportunities created 
as a result of dataframes.
}

We appreciate this comment, and have taken it to heart -- please see responses to
(M2/M3).


\com{(A5)
It is hard to print the PDF and, having gotten it printed,
the math symbols were not properly rendered.
}


We have re-rendered the Math symbols in the PDF to allow for easier printing.


\com{(A6)
It was surprising that there were no row-level schemas.
}

%\agp{This needs fixing based on joe's updates}
% \agp{We need two lines in the dataframe data model
% section about this.}
% \devin{We go into deep detail in this in Section 5, is that not enough?}
This is an interesting point!
Both the relational model and \pandas have schemas on only one axis: columns.
For relations, this is because of the distinct semantics of rows and columns.
Perhaps in \pandas this is because of the desire for a single default interpretation of a cell:
we always use the column type to interpret the bits in a cell. 
One could of course have an alternative row-based interpretation 
as you suggest, though. This is achieved in dataframe libraries like \pandas, as well
as our algebra, by applying a transpose operator (which of course is not in SQL!)
to shift interpretation.
However your observation is intriguing. We now highlight this point in Section~\ref{sec:dataframedef},
and discuss the resulting optimization challenges (i.e. the need to transpose
just to shift one's interpretation) in Section~\ref{sec:rowcolumneq}. 

% We opted for column-level schemas without row-level schemas 
% as is traditional in relations,
% as well as in \pandas via the \code{dtype} operator.
% We could have instead opted for row-level schemas 
% without column-level schemas
% wherein we apply our schema induction function on rows.
% In our formalism, we effectively 
% achieve this by transposing first,
% and treating the result column-wise.
% Our decision to opt for a single axis of schematization
% is so that 
% we have
% a unique interpretation for the value of each cell
% in the dataframe.
% That said, we could support schematization across both axes,
% and we discuss the performance implications
% for doing so in Section~\ref{sec:datamodel}.

% Indeed, we could have chosen to include row-level schemas.
% Row-level schemas or row typing, 
% for example, could be very useful
% if a dataframe has a fixed type across
% the rows but not the columns, so that
% on transposing it, we can recover the types correctly.
% Row typing is less useful (and adds a lot of unnecessary storage overhead) 
% when there is an array
% of types along a row, e.g., [<int>, <string>, <float>],
% as is likely when the column types are all distinct.
% Therefore, instead of forcing row typing in our model,
% we made it optional. 
% Implementations are free, however, to keep track
% of row-level schemas to avoid
% expensive schema induction after a transpose.
% We have added a discussion
% on these tradeoffs are a future research challenge
% in Section~\ref{sec:datamodel},
% and mention the fact that row-level schemas
% can be used in Section~\ref{sec:dataframedef}.





% \done{
% We have added a discussion on maintaining row-level schema in 
% Section~\ref{sec:datamodel}.
% We choose not to define row-level schemas as a part of the core data model,
% rather we allow it to be an extension that implementations
% can choose how to handle.
% We chose not to enable tuple types in the supported Domains
% to simplify the data model, and rows would be most specifically typed by a tuple
% containing each type of the columns. In practice, implementations are free to
% track and maintain a row-level schema if they choose, but it is not a
% requirement of the data model itself.
% A dataframe with heterogeneously typed columns will have rows that are
% tuple-typed. With a TRANSPOSE, the columns would become tuple typed.
% }

\com{(A7)
In the performance figure, why was there was a spike in variance around 100GB,
which was followed by a normalization of perofmance numbers.
}

After rerunning the experiments, we concluded that the spike in variance
was due to some contention in resources. We repeated the experiments additional times and did not see the variance spike in the
updated results. The new numbers are reported in 
Figure~\ref{fig:performance}.



\subsection*{Reviewer 2}
\com{(B1) 
The microbenchmarks do not demonstrate the strength of the underlying data model
as it's strength is in the assembly of the operators,
which does not occur in the microbenchmarks
}

Our goal with the microbenchmarks is to 
validate that simple optimizations (such as parallelism) 
within \modin 
can lead to substantial improvements
in scalability and performance over \pandas,
which has severe issues, despite being widely used.
To clarify this point further, we have moved
the \modin section to Section~\ref{sec:modin}
as opposed to Section 4 (in the previous version),
and focused more on lessons learned from our engineering
experience with \modin, and how that guides 
our future research directions. 
Indeed, further experiments to test the strength of
the underlying model and rewriting rules are needed, 
but we consider that as part of our future research agenda
and will do so in future work.



% The purpose of the microbenchmarks is to demonstrate that \modin gets
% considerable speedup over existing implementations with simple
% parallelism. It points out that despite having a lack of 
% scalability and performance, \pandas is extremely widely used.
% As a future work, we will add benchmarks demonstrating
% the strength of the algebra, however since this is a vision paper not
% focused on any specific implementation's performance, we would
% prefer to keep the current microbenchmarks simple as-is, so as not to distract
% from the central message of the paper.


\com{(B2) 
The paper, after the technical details of Modin,
is a grab bag of notes on existing work in databases and data science.
The discussion is somewhat direction-less and there is no true vision expressed here.
}
This feedback was addressed while resolving (M2/M3).
We have taken this feedback to heart and entirely revamped
Sections~\ref{sec:datamodel} and \ref{sec:interactivity} to be centered
on novel dataframe aspects. 


\com{(B3) 
Table of operator is not legible in printouts.
}


We have fixed the table to be more legible in printouts 
with a larger text size.


\com{(B4) 
Typo when discussion operators:
``... as well as four new operators.. We briefly describe... the three new operators.''
}


We have fixed this typo to describe the four new operators.


\com{(B5) 
It is unclear whether the types of values are represented and inspectable at run time.
}

Types are inspectable at runtime, and inspecting the types
will trigger their materialization if they are already not
materialized. We have added this clarification to 
Section~\ref{sec:datamodel}.
% \agp{Where is this? I don't see it. To me, it should be in Section~\ref{sec:definitions}, not in Section~\ref{sec:datamodel}.}
% \devin{
% We frame this as a challenge because it's really only accessible via 
% \code{GROUPBY} or \code{MAP}.
% Is this worth mentioning in \ref{sec:definitions}?
% }


\com{(B6) 
Some of the rewrites should be removed and 
be replaced with fewer but more in-depth rewrites.
}

We agree with the reviewer that the number of rewrites
in Section~\ref{sec:algebra-example}
was excessive and was not adding much to the discussion.
We have instead decided to focus on \code{pivot} as a single
case study---a challenging operator for relational algebra---and
described it in more detail with a new diagram.
% We have trimmed the number of rewriting examples in 
% Section~\ref{sec:algebra-example} and gone more in-depth about the
% pivot case, which is the most challenging case for relational algebra.
% The section has been rewritten to focus more generally on the display of
% the data model and less about any specific implementation.
% }

\com{(B7) 
The statement that ``query optimization is not possible in an eager system''
is misleading because most query optimization is performed before the evaluation of the program.
}

We were not clear in our writing 
and did not intend for this interpretation.
Dataframe systems, unlike relational databases,
support an incremental mode of composition of queries
where programmers can specify a \stmt 
composed of one or more operators at a time (i.e., a query sub-expression),
building on the variables declared in previous \stmts.
We revised Section~\ref{sec:interactivity}
to clarify that, by ``eager'',
we mean that the query processor executes each \stmt
as soon as it is invoked by the programmer, without waiting.
By ``lazy'', we mean that the query processor waits 
until the dataframe is either printed or saved before
it finds an optimized query execution plan that is 
semantically equivalent 
to executing each of the operators 
of query sequentially,
and executes this optimized query plan.
In this context, we believe that the ``eager'' mode
makes it difficult to perform query optimization
since the query processor will need to produce
results for each intermediate sub-expression as assembled by the user.
We have reworked this entire section and 
taken out the ``not possible'' part as it was confusing;
we have also added an example to illustrate this further.

% Thus, in this context, we believe that it is impossible to have
% efficient query plan when the query processor 
% naively and immediately executes
% each operator in the order that the programmer 
% calls them in the statement.
% \agp{agp to review}

\com{(B8)
The idea that lazy query processors ``recently emerged'' is flawed
as the on-demand evaluation of complex algebraic plans (e.g., Volcano)
has been the default mode of execution in query processors for decades.
}

We were not clear in our writing when stating that 
``the lazy paradigm ... recently emerged.''
We revised our submission to make it clear that
we are discussing eager and lazy evaluation
in the context of other dataframe and dataframe-like systems 
such as Pandas, Dask, and Spark, 
and not in relational databases 
which do not have
an incremental mode of composition.
In the context of dataframe systems,
eager execution, as described in the previous point,
is the canonical approach as is the approach used
in dataframe systems up until recently (e.g., Pandas and R Dataframes).
It is only recently with Spark dataframes and Dask 
have dataframe or dataframe-like 
systems begun operating within a lazy paradigm.
But since this point is subtle, we removed
any mention of whether the emergence was recent, 
and focus more on conveying the two modes as is,
centered on dataframe and dataframe-like systems.
% \agp{agp to review}
% \devin{I took out the whole ``recently emerged'' argument. It added nothing and served as a distraction.}

\com{(B9)
There should be more discussion around multi-query optimization and materialization.
Particularly, there should be more discussion on how the system would
predict which intermediate results would be more likely to be used.
What information would be necessary to drive such inferences?
}

% \agp{I don't believe we have added any discussion on this to the paper AFAIK.
% We should be talking about statistics that can help drive prediction.}
We have added further discussion on materialization and reusing
query results to Section~\ref{sec:interactivity},
taking advantage of ample user think-time. Specifically,
we discuss the need to predict user intent based on past workloads~\cite{ucsd-dataframe-study}
and operator lineage. We discuss the challenges in materialization
of intermediate results given that we may have many query fragments
partially completed. 
We also propose interesting future work on
embedding materialization decisions within the opportunistic
evaluation query planner to further accelerate the interactive user experience with speculative execution.
% We also discuss some interesting future work in
% integrating a materialization decision engine with the opportunistic
% evaluation approach to interactive query planning to enable
% some speculative execution as a part of the query plan for even
% faster results for the interactive user.
% \agp{At least a couple more sentences that start with "Specifically, we ..." }

\com{(B10)
It may be hard to do prefix computation when considering more complex expressions
as the system may need more than k rows to be able to display a prefix of size k
after more operations have been added to the expression.
What is the approach that Modin will take to this issue?
}

% \agp{I don't think this is our approach to answering this question. We
% are describing novel aspects wrt prefixes and order. Need to discuss.}
% \done{
% Because prefix computation with complex expressions is not a challenge that is
% specific to dataframes, we chose not to focus on it to place a higher importance
% on dataframe-specific challenges.
% }
% \devin{This needs to be updated if it is not already}
We have added a deeper discussion in Section~\ref{sec:datamodel} 
on the novel aspects of prefix computation
and the challenges in preserving order 
with prefix computation. As the reviewer mentions, it is
not always possible to know how many
rows a given query will output, and keeping aside
only $k$ rows will not always work, especially in complex queries
with selective predicates---this question is not new to dataframe systems
but the ordering aspect is novel. 
One approach, for example, would be to use operators that generate
results in order, such as index nested loop joins,
which progressively ingest more of the input dataframes until 
$k$ output rows are produced.
We can also leverage parallelism to 
prioritize the ingest
and processing of ``enough'' of the inputs to guarantee
the output of the first $k$ rows.
Since dataframes
must {\em guarantee} both the top $k$ and its order,
that dataframe query optimizers may need to use both 
selectivity and cardinality estimates, along with
models of past user behavior to gain 
insight into how many
input rows may be necessary to generate $k$ output rows. 
% This research may yield
% some interesting results that can also be applied to
% RDBMSs.
% \agp{this is weak: we only say we will look at past history. need a better argument.
% will revisit after i read s6}

\com{(B11) 
Sections 5 and 6 should be more concrete and try to have a focused vision
that shows how the algebraic approach can be an advantage on the current
state-of-the-art (e.g., Pandas and R).
This may be the focus on query planning to defer or avoid costly
data restructuring operations or 
a reversal of roles of data data and meta-data.
}

\com{AND}

\com{(B12)
There should be a connection between the technical details described in the beginning
and the vision described in the rest of the paper.
It is ok if this makes the vision of the paper becomes specific to the Modin view of dataframes.
}

This feedback was addressed while resolving (M2/M3).
We thank the reviewer for the query planning points---we have used them 
when reframing our vision when centered around novel
aspects of dataframes.
We have also substantially revised the previous portions of the paper
to keep only as many technical details as is needed
to ground our discussion on the vision.

\subsection*{Reviewer 3}
\com{(C1) 
Please cut out a bunch of details, we don't need a 12 page vision paper.
\squishlist{}
    \item I don't really need a 1-page example on data frames.
    \item Why do I need to know the history of data frames?
    \item Perhaps we do not need the exact formalism for the data model and all operations and
    a detailed sketch would suffice.
\squishend{}
}

This was resolved while addressing (M1). We provide some additional
details below.

We thank the reviewer for these suggestions.
We retained the example, but substantially reduced its length
and detail as it allows database readers who are unfamiliar
with dataframes to establish a basic understanding.
We have also redrawn the figure to reduce the space taken for it.

We have reduced the length for the history of dataframes,
only emphasizing key background for the interested database reader.
Specifically, we retained the portions that 
contribute a meaningful and largely unknown piece 
of how dataframes
emerged to the scientific community. 
This background also 
gives a basis on which we can
understand how dataframes were intended to be used, 
so that we can optimize
them in this context.


Finally, we have substantially reduced the length 
and details 
in the formalism
for the data model and algebra, 
reduced the number of rewritings,
and removed the extensions. 
We focus on the
components which make dataframes difficult to scale. The formalism
is important because it provides a basis upon which we can build
our research vision---and we only retain as much as is needed
to support that. 
We have also clarified the intention of this section.

Given the overwhelming popularity of dataframes
and their important role in the data science ecosystem,
as well as the relative lack of awareness and understanding
from the database research community,
we believe that the length of this paper is justified.

% Given the overwhelming popularity of dataframes and their important position in the data analysis ecosystem, we believe that the length of this paper is commiserate with the urgency for the database community to seize on this historic opportunity to make its mark on the future of computing. 
%This warrants detailed and exhaustive introspection on future research directions. As such, we have added substantial content on concrete research opportunities spanning many relevant areas of databases research.


\com{(C2) 
Missing related work.
There should be explicit mention of embeddable DBMSs such as DuckDB and SQLite
and, at least, a theoretical comparison of them and the vision proposed in the paper.
Also, please cite Tukey's book on EDA.
}

Regarding embeddable DBMSs, from an architecture perspective, we now 
clarify in Section~\ref{sec:modin} that Modin is a library, much like an embeddable DBMS. (This is standard for 
dataframe libraries, including pandas, so we overlooked mentioning it in this environment. It's a nice
connection to make, thanks!) In Section~\ref{sec:flexschemas} we also address some of the implications that arise 
for dataframes from having their storage external to the application, including some of the work in the 
community (e.g. Apache Feather) to address this. Finally, with respect to theoretical issues, the bulk of the 
paper focuses on distinctions (both theory and practice) that arise from the semantic distinctions
between relational databases (embedded or otherwise) and dataframes, so we hope there's sufficient discussion
of DBMSs vs. dataframes in general.

% \jmh{Why fight? I vote to skip this}
% Our entire thesis is that
% we must design dataframe systems from the ground up to support
% the unique characteristics of dataframes, including 
% flexible schema/dynamic typing,
% data-metadata and row-column equivalence,
% centrality of order, and differences in algebraic operators.
% Thus, any system whose interface is SQL-like and whose data model
% is relational is not a good fit, including embeddable databases.




% While embeddable DBMS systems could be a possible candidate
% for a processing and storage engine for dataframes, 
% given the vast differences
% in characteristics, including flexible schema/dynamic typing,
% data-metadata and row-column equivalence,
% centrality of order, and differences in algebraic operators,
% we do not believe it would be a good fit---and instead believe an
% approach that takes these characteristics as first-class citizens
% as opposed to bolting them on post-hoc, would
% be much more efficient and scalable.
% \agp{I think the following line should be dropped.
% Instead, we can replace it with one line around how the goals
% and vision are very different.
% Perhaps they may be satisfied if we add a line that says 
% that we can use an embeddable DBMS 
% as a storage/processing layer for dataframes?}
% We did not included the comparison of embeddable DBMS and dataframe as we believe that the scope of these systems are somewhat tangential, so we have limited this discussion to keep the dataframe vision the central point of the paper.

% We have clarified the related work section, Section~\ref{sec:}
% and
% The theoretical comparison to the data model was expanded upon
% and clarified, but to keep the vision the central point of the paper
% we have limited this discussion.
With respect to Tukey, we are big fans, and have happily added a citation to Tukey's book in the introduction.
Thanks for pointing that out -- sometimes we take our heroes for granted!

\com{(C3) 
The future vision is a bit generic.
Although sections 5-7 are the more interesting parts
with a particular emphasis on section 6,
they are only 2 pages out of the entire paper.
These sections should have a higher fraction of the paper
by adding more depth to the challenges and future directions
and making them less generic would also help.
}

This feedback was addressed while resolving (M2/M3).
We have taken this feedback to heart and have substantially revised
the vision portions of this paper.



==> multi_statement.tex <==

\section{Acceleration across Statements}\label{sec:acrossstatement}

One of the most-used features of dataframes is the ability to compose longer
queries one statement at a time and save, store, or return to
intermediate results.
In a SQL database, this can be done with views, 
which are selectively materialized by the query optimizer.
In a pure dataframe implementation such as pandas, 
intermediate results are materialized
in memory as long as there is a pointer to it in scope.
Users rely on these intermediate result in the typical data scientists workflow,
primarily because a
significant amount of dataframe interactions follow the trial and error
programming paradigm.
Despite its usefulness from the user's perspective,
materialization of every intermediate result is expensive
and memory intensive. The cost and potential
optimizations of this behavior across 
sub-queries will be discussed in Section~\ref{sec:acrossstatement}.

There is a significant missed opportunity for optimization if
we only focus on optimizing single statements. For example, taking a
reduction (e.g. \code{COUNT}) followed by a projection. If we perform
the projection first, we can significantly reduce the amount of
computation. In this section, we will discuss several ways we can apply techniques from relational database literature to speed up the execution of dataframe operations.


\subsection{Multiquery Optimization}\label{sec:mqo}
We envision that \modin will prioritize interactivity, returning
control to the user as quickly as possible by displaying
preview (head/tail) or
approximate results and defer calculation of full or exact results to background computation using techniques from Section\label{sec:singlestatement}.
As such, many operations may be queued for execution at once\dlee{not sure what this sentence is saying}. These statements may
operate over similar or even identical subsets of data. To exploit this workload, \modin will make use of multiquery optimization (MQO) techniques~\cite{sellis1988multiple}
to allow operations that share significant amounts of data to run underneath the
same scans or seeks, thereby reducing the overhead required to funnel data up
through the memory hierarchy. However, MQO presents a significant challenge when employed
in an interactive environment, where the results of the operation is displayed in-situ the coding/input environment, such as a Jupyter notebook cell. In this case, the optimizer will have to balance between maximizing operation throughput and
minimizing the latency required to compute output of the important ``to-be-displayed'' operations.

\subsection{Rewrite Rules}

Current approaches to planning queries for dataframes are either
(1) strictly imperative and do not perform any 
query planning~\cite{mckinney2010data, R, dask}
or (2) declarative but do not support operations
beyond the traditional relational table operations~\cite{Armbrust:2015:SSR:2723372.2742797}.
The challenge of supporting declarative query processing across a wide range of dataframe operators is that the cost of extending rewrite rules beyond relational operations, to support spreadsheet and linear algebra operations, requires a significant development effort.
% This is the case because it is simply not feasible to write rewrite rules
% for, not just the relational, but also spreadsheet, linear algebra operations
% and their interactions.
As a result, dataframe users either have to sacrifice performance, operate on a feasible subset of their data, or manually construct and profile various possible rewrite to determine the optimal approach to execute the query~\cite{optimizing-pandas}. When creating rewrite rules for dataframes, we have to consider (1) how to group the dataframe operations into queries and (2) when to rewrite the queries.

% completely ignoring performance when writing their queries
% or have to manually profile and determine the optimal way
% to do each query by hand~\cite{optimizing-pandas}.
Manual query optimization on the part of the developer can be a daunting task due to the large number of possible ways to perform an operation~\cite{Wu2019}.\dlee{I don't think the example for sum is necessary, or we could simply say that there are X number of ways of performing certain operation. Add citation to Yifan's paper.}
% \st{For instance, we can calculate the sum of each column with
% either of the following
% \begin{lstlisting}
% sum1 = df.sum(axis=0)
% sum2 = df.apply(sum, axis=0)
% \end{lstlisting}
% Although we use the \pandas API here,
% this is not a \pandas specific problem \cite{???}.
% With the numerous ways of being able to calculate something as simple as a sum,
% the flexibility given to users also makes the task of rewriting queries for dataframes significantly harder.} 
In addition to the numerous ways of writing any given query at the API level,
the problem is further exacerbated by the fact that
there large, diverse set of operations beyond relational operators to consider when creating rewrite rules.
Traditional databases typically focus exclusively on relational  
operators~\cite{???}.
Although there has been work to cover spreadsheet and linear algebra 
operations~\cite{???} \william{Cite that pivot paper.} \simon{and stonebreaker scidb},
they still rely on the underlying rewrite rules made 
with relational operations in mind.
Thus, there is simply too large of a space of API and functionality
to cover in comprehensively with proper rewrite rules.

In addition to the large query space to cover with rewrite rules,
we still have to consider when the query rewriting will occur.
Traditional databases operate in a declarative environment.
As a result, it is obvious that the query rewriting occurs 
once the query is submitted.
However, there is no clear cut line to even differentiate separate queries for dataframes because most existing dataframe frameworks are imperative and execute operations eagerly.

\subsection{Optimizing user time} % for humans-in-the-loop
Although there are dataframe implementations that already do query 
rewriting~\cite{Armbrust:2015:SSR:2723372.2742797},
they operate within a lazy computation environment.
While laziness simultaneously solves the problem of
how to group the queries and when to rewrite the queries,
as we have already seen from Section~\ref{sec:modin}, the lazy execution model is not ideal for interactive dataframe workloads with a human-in-the-loop.

From the system's perspective, lazy evaluation seems like the best way to
conduct query optimization: the system will optimize the number of CPU
cycles it takes to get to an answer. However, from the user's
perspective, lazy evaluation removes the interactive capabilities of data frames, namely incremental query building
and checking intermediate results. %two components of the dataframe
% system that make it more useful in interactive environments
% than a DBMS: 
When the user checks the result of every
statement, it limits the amount of query planning possible in a system using 
lazy execution. 
% Users in the interactive environment also spend a large amount of time thinking in a typical workflow. 
Moreover, users are usually idle in the interactive workflow when thinking and re-writing the program.
When this happens, the CPU ends up waste cycles being
idle while the user is also idle or thinking.

Instead of focusing on minimizing the CPU cycles it takes to arrive at an answer, a more effective objective would be to minimize the overall wall clock time for an interactive
workflow.In other words, we prioritize the user's time over the CPU's time to provide a more productive environment for users. In order to be useful in a
general setting, a system that prioritizes a user's time in an interactive
environment should also be able to perform as well as the state-of-the-art
systems that prioritize a CPU's time when running in a batch environment or
in the worst case for interactive workflows.

Thus, though rewriting dataframe ``queries'' may appear to be a solved problem,
dataframes bring a unique set of problems that will require their own unique approach,
while simultaneously borrowing from approaches used in traditional databases.

\subsection{Materialization and Reusing Results}
The incremental and exploratory nature of dataframe query construction 
leads to nonlinear code paths 
where users revisit the same intermediate results repeatedly 
to refine the query results. 
Recomputing the same intermediate result repeatedly
is time-consuming and wasteful. Ignoring re-computation can also be costly for operations such as data loading, which often does not need to be re-executed.%On top of that, there is a real need to remove such redundancies. For examples, it makes no sense to use Pandas' APIs to repeatedly store and reload dataframes in PyTables via HDFStore.
We envision the \modin optimizer to automatically materialize and reuse intermediate results
to significantly reduce execution time by removing redundant computation across statements.

To concretize the discussions of the research challenges
associated with this optimization, consider the following example.
\begin{lstlisting}
r1 = df.groupby(...).count().query("c1 > 0")
r2 = df.groupby(...).count().query("c2 <= 0")
\end{lstlisting}
Intermediate results refer to the output of any combination of operations.
In this example, the intermediate result accessed by both \code{r1} and \code{r2} 
is \code{df.groupby(...).count()},
which is computed twice when executing the statement verbatim.
We could eliminate the redundant computation 
by identifying this common subexpression in both statements
and substitute it with a reference to the intermediate results.
This is a common technique in compilers known as common subexpression elimination\cite{cocke1970global}. Applying these techniques to dataframes is non-trivial due to the tradeoff between storage cost and compute savings.
% which when applied to dataframes becomes more complex 
% because it will involve trade-offs between storage cost and compute savings.

Formally, the objective of this optimization problem is to trade
\textit{materialization overhead}, including both the storage and the time to persist the results,
for \textit{reduced execution time} due to reuse. 
As we can see from the example above, there are two components to this optimization.
First, we need to identify reusable intermediate results, 
which can be accomplished using standard program analysis.
The second component is deciding whether an intermediate result should be stored and reused,
and the optimizer needs to utilize storage in a way that maximizes 
saved compute---small 
objects that are time-consuming to compute and reused frequently 
should be prioritized over large objects that are fast to compute.
Storage can refer to either memory or disk, 
depending on whether reuse takes place within a single session 
or across multiple sessions.
A storage budget is often imposed, especially in the single-session case, making the problem NP-Hard (by reduction from the Knapsack problem).
Effective solutions need to adapt to variable reuse patterns.

\subsection{Cost Modeling and Optimization}

Once we have identified a set of simple rewrite rules,
we will develop a simple cost model for optimization purposes.
Since much of the data for dataframes sits in-memory, we will need
to develop a cost model that is appropriate for hierarchical
memory systems\cite{manegold2002}. However, we do not simply
want to model the cost for the CPU's time. Because of the interactive
nature of dataframes, we will want to model the cost to
both the user's and the CPU's time and prioritize the
optimization of the user's time. 

For example, in a case where the user is engaged with a challenging task that requires significant think time between executed statement,
% is thinking for significant amounts of time between statements invocations.
it is possible to begin processing parts of that statement immediately,
and complete the processing of the statement during
the user's think time. For exceptionally complex statements, such as  nested joins, it is possible to wait for the next
statement to see whether the user provides a filter or some
other operator that would reduce the amount of computation necessary.
This way, the system can be selectively lazy and choose when
or if to delay computation, while
optimizing for the user's valuable analysis time.

Asynchronous computing is a middle ground that will allow
us to choose whether or not to be lazy for any given
statement without placing any of this decision burden
on the user. When the user submits a statement,
the cost modeler will determine whether or not to
immediately execute that query based on the cost
model we develop to model the user's time. If the
system chooses to delay computation, when the user
submits their next statement, the cost modeler
will again determine whether to execute immediately
given the new statement from the user.

In order to develop a cost model for the user's time,
we will first have to study how users interact with the
system. Understanding what operations typically follow
others, when users pause for thinking, and how long
pauses are. This study must be conducted on a large
number of users to ensure generalizability across tasks and datasets, 
and will be an important first step in
modeling users behavior when interacting with dataframes.
Modeling the user behavior is a common practice in the HCI literature \cite{Battle2019}.


==> notes_macros.tex <==
\newcommand{\jeg}[1]{\textcolor{cyan}{jeg: #1}}
\newcommand{\agp}[1]{\textcolor{blue}{Aditya: #1}}
\newcommand{\devin}[1]{\textcolor{orange}{Devin: #1}}
\newcommand{\william}[1]{\textcolor{green}{William: #1}}
\newcommand{\simon}[1]{\textcolor{teal}{Simon: #1}}
\newcommand{\dorx}[1]{\textcolor{brown}{dorx: #1}}
\newcommand{\dlee}[1]{\textcolor{violet}{\textbf{dlee: #1}}}
\newcommand{\adj}[1]{\textcolor{red}{Anthony: #1}}
\newcommand{\omkar}[1]{\textcolor{purple}{Omkar: #1}}
\newcommand{\rehan}[1]{\textcolor{magenta}{Rehan: #1}}
\newcommand{\jmh}[1]{\textcolor{red}{JMH: #1}}
\newcommand{\smacke}[1]{\textcolor{pinegreen}{\textbf{Stephen: #1}}}
\newcommand{\smquote}[2]{\textcolor{pinegreen}{\string{#1\string}\textbf{[Stephen: #2]}}}
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\done}[1]{{\color{pinegreen}{#1}}}

==> old_intro.tex <==
% THIS IS AN EXAMPLE DOCUMENT FOR VLDB 2012
% based on ACM SIGPROC-SP.TEX VERSION 2.7
% Modified by  Gerald Weber <gerald@cs.auckland.ac.nz>
% Removed the requirement to include *bbl file in here. (AhmetSacan, Sep2012)
% Fixed the equation on page 3 to prevent line overflow. (AhmetSacan, Sep2012)

% \documentclass{vldb}
\usepackage{graphicx}
\usepackage{balance}  % for  \balance command ON LAST PAGE  (only there!)


% Include information below and uncomment for camera ready
\vldbTitle{Modin: The DataFrame Strikes Back}
\vldbAuthors{Ben Trovato, G. K. M. Tobin, Lars Th{\sf{\o}}rv{$\ddot{\mbox{a}}$}ld, Lawrence P. Leipuner, Sean Fogarty, Charles Palmer, John Smith, Julius P.~Kumquat, and Ahmet Sacan}
\vldbDOI{https://doi.org/10.14778/xxxxxxx.xxxxxxx}
\vldbVolume{12}
\vldbNumber{xxx}
\vldbYear{2019}

\begin{document}

% ****************** TITLE ****************************************

\title{Modin: The DataFrame Strikes Back}


% possible, but not really needed or used for PVLDB:
%\subtitle{[Extended Abstract]
%\titlenote{A full version of this paper is available as\textit{Author's Guide to Preparing ACM SIG Proceedings Using \LaTeX$2_\epsilon$\ and BibTeX} at \texttt{www.acm.org/eaddress.htm}}}

% ****************** AUTHORS **************************************

% You need the command \numberofauthors to handle the 'placement
% and alignment' of the authors beneath the title.
%
% For aesthetic reasons, we recommend 'three authors at a time'
% i.e. three 'name/affiliation blocks' be placed beneath the title.
%
% NOTE: You are NOT restricted in how many 'rows' of
% "name/affiliations" may appear. We just ask that you restrict
% the number of 'columns' to three.
%
% Because of the available 'opening page real-estate'
% we ask you to refrain from putting more than six authors
% (two rows with three columns) beneath the article title.
% More than six makes the first-page appear very cluttered indeed.
%
% Use the \alignauthor commands to handle the names
% and affiliations for an 'aesthetic maximum' of six authors.
% Add names, affiliations, addresses for
% the seventh etc. author(s) as the argument for the
% \additionalauthors command.
% These 'additional authors' will be output/set for you
% without further effort on your part as the last section in
% the body of your article BEFORE References or any Appendices.

\numberofauthors{8} %  in this sample file, there are a *total*
% of EIGHT authors. SIX appear on the 'first-page' (for formatting
% reasons) and the remaining two appear in the \additionalauthors section.

\author{
% You can go ahead and credit any number of authors here,
% e.g. one 'row of three' or two rows (consisting of one row of three
% and a second row of one, two or three).
%
% The command \alignauthor (no curly braces needed) should
% precede each author name, affiliation/snail-mail address and
% e-mail address. Additionally, tag each line of
% affiliation/address with \affaddr, and tag the
% e-mail address with \email.
%
% 1st. author
\alignauthor
Author Name\\
       \affaddr{Institute for Clarity in Documentation}\\
       \affaddr{1932 Wallamaloo Lane}\\
       \affaddr{Wallamaloo, New Zealand}\\
       \email{trovato@corporation.com}
}
% There's nothing stopping you putting the seventh, eighth, etc.
% author on the opening page (as the 'third row') but we ask,
% for aesthetic reasons that you place these 'additional authors'
% in the \additional authors block, viz.
\additionalauthors{Additional authors: John Smith (The Th{\o}rv\"{a}ld Group, {\texttt{jsmith@affiliation.org}}), Julius P.~Kumquat
(The \raggedright{Kumquat} Consortium, {\small \texttt{jpkumquat@consortium.net}}), and Ahmet Sacan (Drexel University, {\small \texttt{ahmetdevel@gmail.com}})}
\date{30 July 1999}
% Just remember to make sure that the TOTAL number of authors
% is the number that will appear on the first page PLUS the
% number that will appear in the \additionalauthors section.


\maketitle

\begin{abstract}
Abstract content goes here.
\end{abstract}




\section{Introduction}
The DataFrame has become a staple component of modern data science. 
It is often used to clean or filter datasets, gather summary
statistics, and to query data. The success of the DataFrame can seem
somewhat counter-intuitive because many DataFrame systems violate
fundamental database principles in their implementation and offer
additional functionality and features that traditional database
systems do not. However, DataFrame systems are popular primarily
because of the deviations from conventional wisdom in database
systems. The primary reason DataFrame systems are so popular is
because the data has an order, and an order that is preserved through
transformations, similar to the spreadsheet model. Another important
design of the DataFrame is that queries can be built one small
component at a time, and intermediate results can be checked for
validity. In a traditional DBMS using SQL, intermediate results can
only be checked by independently executing a subquery, however DataFrame
technologies allow users to check intermediate results and build queries
one statement at a time. Depending on the use-case, other features may be
important to users, e.g. interoperability between linear and relational
algebra, indexing, and virtually unbounded user defined functions. Users
who prefer DataFrame systems typically use it in an interactive
environment. 

Because of these design deviations, DataFrame systems are difficult to
optimize with the best practices from traditional database query
optimization and have generated a large body of work studying how to
bridge the gap between traditional database systems and DataFrame
technologies [CITE SOME]. Unfortunately, many of the systems that attempt
to bridge this gap do not take advantage of all the work done by the
Database community in query optimization. They additionally push a
large portion of the optimization
burden onto the user, often resulting in a system that is both harder to use
and under-optimized. For example, many DataFrame systems use lazy execution to
construct a DAG of operations and only compute an answer when it is
needed. From the system’s perspective, this seems like the best way to
conduct query optimization: the system will optimize the number of CPU
cycles it takes to get to an answer. However, from the user’s
perspective, lazy evaluation removes two components of the DataFrame
system that make it more useful than a DBMS: incremental query building
and checking intermediate results. When the user checks the result of every
statement, it limits the amount of query planning possible in a system using 
lazy execution. Users in the
interactive environment also spend a large amount of time thinking in a
typical workflow. When this happens, the CPU ends up waste cycles being
idle while the user is also idle or thinking.

Instead of focusing on minimizing the CPU cycles it takes to arrive at an answer, a more useful
metric would be to minimize the overall wall clock time for an interactive
setting. In this way, we prioritize the user’s time over the CPU’s time and
provide a more productive environment for users. In order to be useful in a
general setting, a system that prioritizes a user’s time in an interactive
environment should also be able to perform as well as the state-of-the-art
systems that prioritize a CPU’s time when running in a batch environment or
in the worst case for interactive workflows. 

DataFrames are not SQL systems, but this does not mean that we should
completely throw out all of the research that has been done into optimizing
SQL when designing and building DataFrame systems. We should be borrowing
from and using SQL techniques to optimize queries in DataFrame systems. To
realize this vision, we built a system called Modin as a launchpad for
research into how to bridge the gap between DataFrame and Database systems.


\section{The origins of the DataFrame}
This section will contain the origins of the DataFrame text.

\section{Use cases and usage}
This section will contain the Use cases and usage text.

\section{Modin: Bridging DataFrames and Databases}
This section will contain the Modin research plan text.

\subsection{Current improvements over Pandas}
For example, multiprocessing.

\subsection{Query optimization}
Our plans for Query Optimization

\subsection{System level optimization}
Partitioning, Serverless, etc.

\subsection{API and other HCI}
Smaller API based on IR

\section{Conclusion}
This is the Conclusion section text.
%\end{document}  % This is where a 'short' article might terminate

% ensure same length columns on last page (might need two sub-sequent latex runs)
\balance

%ACKNOWLEDGMENTS are optional
\section{Acknowledgments}
I would like to thank the Emperor for squashing the rebellion.


% The following two commands are all you need in the
% initial runs of your .tex file to
% produce the bibliography for the citations in your paper.
\bibliographystyle{abbrv}
\bibliography{old_intro}  % old_intro.bib is the name of the Bibliography in this case
% You must have a proper ".bib" file
%  and remember to run:
% latex bibtex latex latex
% to resolve all references

\subsection{References}
Generated by bibtex from your ~.bib file.  Run latex,
then bibtex, then latex twice (to resolve references).

%APPENDIX is optional.
% ****************** APPENDIX **************************************
% Example of an appendix; typically would start on a new page
%pagebreak

\begin{appendix}
You can use an appendix for optional proofs or details of your evaluation which are not absolutely necessary to the core understanding of your paper. 

\section{Final Thoughts on Good Layout}
Please use readable font sizes in the figures and graphs. Avoid tempering with the correct border values, and the spacing (and format) of both text and captions of the PVLDB format (e.g. captions are bold).

At the end, please check for an overall pleasant layout, e.g. by ensuring a readable and logical positioning of any floating figures and tables. Please also check for any line overflows, which are only allowed in extraordinary circumstances (such as wide formulas or URLs where a line wrap would be counterintuitive).

Use the \texttt{balance} package together with a \texttt{\char'134 balance} command at the end of your document to ensure that the last page has balanced (i.e. same length) columns.

\end{appendix}



\end{document}


==> single_statement.tex <==
\section{Single Statement Acceleration}\label{sec:singlestatement}
\devin{Renormalize to focus on the unique features of the data model that make research interesting}

Based on users' common behaviors, there are two common database optimizations we can use to accelerate the execution of individual statements in dataframes: computing partial results
(\ref{sec:pre-suffix}) and approximate computation (\ref{sec:approx}).

\subsection{Prefix or Suffix Computation}\label{sec:pre-suffix}

Dataframe users often build their query incrementally through trial-and-error. As illustrated in Section~\ref{sec:usecase},
the trial and error style typically involves printing some subset
of the rows and columns through the 
\code{head}, \code{tail}, or \code{print} operation.
The \code{head} and \code{tail} commands print the first
or last \code{n} rows (5 by default), respectively. 
Printing a dataframe
shows both the first and last 5 rows. 
This is also another case where the user relies heavily on the
order of the data in their mental model. When a user prints
the first \code{n} rows, they expect to see the first
\code{n} rows from the actual data that was ingested,
and they expect that the system will print the same
\code{n} rows each time. The performance of displaying these first and last
\code{n} rows is important as users rely on these operations to verify the correctness of their data and query and subsequently make decisions about what to do next.

While it is possible to use strategies similar to those that optimize for the \code{LIMIT} clause in RDBMSs \cite{kim2018optimally}, additional
consideration must be made for the \code{ORDER BY} clause to ensure that the order is the same every time
time the user prints the dataframe. To avoid computing the \code{ORDER BY}
on every computation,
the first and
last \code{n} rows can be logically removed as separate tables, 
and perform computation on those
tables to print the results faster. The remaining data can 
computed separately following the lazy evaluation paradigm,
enabling query planning on the remaining data. In the case
that the query modifies the order of the data, the
printed rows will have to wait until the \code{ORDER BY} to 
ensure that the user sees the data in the order they have
specified. In these cases, there is a limit to the amount of
query planning that can be applied because the print forces
the \code{ORDER BY}. We will discuss ways that query planning
can be used and improved for dataframes in
Section \ref{sec:acrossstatement}.

\subsection{Approximate Computation}\label{sec:approx}

Approximate computation is another way to provide users with faster query responses to facilitate interactive workflows. In some cases, the user may be content to see an approximation
rather than needing to wait for the full result. Existing RDBMS approximation
techniques for online aggregation~\cite{Fekete2018,raman2002partial,lang2014partial,viglas2002rate,rahman2017ve},
barchart, histogram, scatterplot, and map plot generation~\cite{kim2015rapid,ding2016sample+,park2016visualization},
histogram matching~\cite{macke2018adaptive}, stratified sampling~\cite{agarwal2013blinkdb}, and
error estimation~\cite{zeng2014analytical,park2018verdictdb} are directly applicable
toward accelerating individual dataframe operations. However, dataframe semantics
offer some unique opportunities for further speedups via approximation.


\dorx{We don't need to make the next two points about top/bottom $K$. 
They're still applicable outside of the prefix/suffix setting.}

\devin{I think in this context the top/bottom $K$ present unique challenges
for dataframes over SQL, which is why that is the focus.}

\dlee{I agree with dorx and its also confusing since 4.1 talks about prefix/suffix issues already. The focus for this subparagraph should be the point about aggregation.}

\smacke{Agree with Dores that it's confusing in light of 4.1 (and it's my fault).
There is a fundamental difference though,
prefix / suffix section discusses accelerating exact computation of top / bottom $K$
while moving remainder to background, this section focuses on the case that
remainder cannot be moved to background for exact computation, and can only be
moved to background if we approximate top / bottom $K$. I'll work on contrasting
so that it's clear why this is a separate issue.}

\stitle{Cumulative Aggregates.}
Existing dataframe libraries like \pandas display the top and bottom $K$
rows whenever an evaluation is triggered. In a typical relational model
with no notion of order, any $2K$ rows could be chosen for display, but
dataframes, which have an inherent order, must be precise in order to
satisfy the expected semantics. This can create bottlenecks when the
computation required to display the bottom $K$ rows depends on the
result of the computation for all previous rows. For example,
a cumulative sum or cumulative max must be done in order from the
top of the dataframe to the bottom, causing significant latency
before the bottom $K$ rows can be displayed.

% placeholder until .bib is fixed
% @article{mozafari2015handbook,
%  title={A Handbook for Building an Approximate Query Engine.},
%  author={Mozafari, Barzan and Niu, Ning},
%  journal={IEEE Data Eng. Bull.},
%  volume={38},
%  number={3},
%  pages={3--29},
%  year={2015}
% }

While it is well known that an aggregate like \code{MAX}
cannot be approximated~\cite{mozafari2015handbook},
the user may be satisfied to see approximations of cumulative sums or means
in the bottom $K$ rows that
either update progressively as more data is processed, or that satisfy a
probabilistic accuracy requirement.

\stitle{Estimating Counts on Filtered Dataframes.}
Along with the top and bottom $K$ rows, dataframe libraries
like \pandas typically show summary statistics like \code{COUNT}
after each operation.
If a user applies a filter on a dataframe, without prior knowledge
it is impossible to know the exact number of rows passing the filter 
until the full computation has completed. One strategy is to
automatically identify such cases and adaptively estimate the
selectivity of the filter on-the-fly, again progressively updating the estimate as more tuples passes through the filter.

\stitle{Approximating Expensive Filters.}
For a filter that is both selective and expensive
(e.g., one that performs classification on
a dataframe where one of the columns contains videos), there might not be any row in the top or bottom
$K$ that satisfies the filter. As such, determining the top and bottom
$K$ rows that pass the filter can itself be a high-latency
operation, even without a complete filter application.
In this case, dataframes present a perfect use case for
{\em exploiting correlations}~\cite{joglekar2015exploiting}
between the filtering attribute
and other attributes in order to quickly approximate
the top and bottom $K$ rows that might pass the filter and
quickly display them to the user, refining as
additional filter evaluations are performed.

%\stitle{Partial Results Semantics: Preserving Shape.}
%Another unique aspect of dataframes is the ability to
%programmatically operate over many columns at the same time
%without explicitly naming them, due to the symmetry present
%between dataframe rows and columns.


\stitle{Approximation and Asynchrony.}
When used in conjunction with \modin's
inherent asynchronous background execution,
exact results may be scheduled in the background for
later verification (as in~\cite{moritz2017trust}).
This may result in many exact queries getting queued in the
background as the user rapidly issues statements and achieves
immediate approximate feedback. To increase throughput of
these statements that build up in the execution queue,
we can apply {\em multiquery optimization techniques}
and to take advantage of opportunities for shared computation,
to be described in detail in Section~\ref{sec:mqo}.

Overall, we envision that the unique semantics of dataframe
operations open up a rich design space of approximation
techniques made all the more relevant by the interactive nature of dataframe usage.

